Auto-Validate: Unsupervised Data Validation Using Data-Domain Patterns Inferred from Data Lakes

Complex data pipelines are increasingly common in diverse applications such as BI reporting and ML modeling. These pipelines often recur regularly (e.g., daily or weekly), as BI reports need to be refreshed, and ML models need to be retrained. However, it is widely reported that in complex production pipelines, upstream data feeds can change in unexpected ways, causing downstream applications to break silently that are expensive to resolve. Data validation has thus become an important topic, as evidenced by notable recent efforts from Google and Amazon, where the objective is to catch data quality issues early as they arise in the pipelines. Our experience on production data suggests, however, that on string-valued data, these existing approaches yield high false-positive rates and frequently require human intervention. In this work, we develop a corpus-driven approach to auto-validate \emph{machine-generated data} by inferring suitable data-validation "patterns" that accurately describe the underlying data domain, which minimizes false positives while maximizing data quality issues caught. Evaluations using production data from real data lakes suggest that Auto-Validate is substantially more effective than existing methods. Part of this technology ships as an Auto-Tag feature in Microsoft Azure Purview.

==> architecture.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{System Architecture}

TBD



==> auto-validate.bib.2 <==
% Encoding: windows-1252

@ARTICLE{abedjan2016,
  author = {Abedjan, Ziawasch and Chu, Xu and Deng, Dong and Fernandez, Raul
	Castro and Ilyas, Ihab F and Ouzzani, Mourad and Papotti, Paolo and
	Stonebraker, Michael and Tang, Nan},
  title = {Detecting Data Errors: Where are we and what needs to be done?},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@inproceedings{bogatu2020dataset,
  title={Dataset Discovery in Data Lakes},
  author={Bogatu, Alex and Fernandes, Alvaro AA and Paton, Norman W and Konstantinou, Nikolaos},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={709--720},
  year={2020},
  organization={IEEE}
}

@article{qahtan13pattern,
  title={Pattern Functional Dependencies for Data Cleaning},
  author={Qahtan, Abdulhakim and Tang, Nan and Ouzzani, Mourad and Cao, Yang and Stonebraker, Michael},
  journal={Proceedings of the VLDB Endowment},
  volume={13},
  number={5}
}

@article{padhi2018flashprofile,
  title={FlashProfile: a framework for synthesizing data profiles},
  author={Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov, Oleksandr and Gulwani, Sumit and Millstein, Todd},
  journal={Proceedings of the ACM on Programming Languages},
  volume={2},
  number={OOPSLA},
  pages={1--28},
  year={2018},
  publisher={ACM New York, NY, USA}
}



@inproceedings{qahtan2018fahes,
  title={FAHES: A robust disguised missing values detector},
  author={Qahtan, Abdulhakim A and Elmagarmid, Ahmed and Castro Fernandez, Raul and Ouzzani, Mourad and Tang, Nan},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2100--2109},
  year={2018}
}


@INPROCEEDINGS{abedjan2016dataxformer,
  author = {Abedjan, Ziawasch and Morcos, John and Ilyas, Ihab F and Ouzzani,
	Mourad and Papotti, Paolo and Stonebraker, Michael},
  title = {DataXFormer: A robust transformation discovery system},
  booktitle = {2016 IEEE 32nd International Conference on Data Engineering (ICDE)},
  year = {2016},
  pages = {1134--1145},
  organization = {IEEE}
}

@INPROCEEDINGS{abreu2014smelling,
  author = {Abreu, Rui and Cunha, J{\'a}come and Fernandes, Jo{\~a}o Paulo and
	Martins, Pedro and Perez, Alexandre and Saraiva, Jo{\~a}o},
  title = {Smelling faults in spreadsheets},
  booktitle = {Software Maintenance and Evolution (ICSME), 2014 IEEE International
	Conference on},
  year = {2014},
  organization = {IEEE}
}

@INPROCEEDINGS{afrati2009repair,
  author = {Afrati, Foto N and Kolaitis, Phokion G},
  title = {Repair checking in inconsistent databases: algorithms and complexity},
  booktitle = {Proceedings of the 12th International Conference on Database Theory},
  year = {2009},
  organization = {ACM}
}

@INPROCEEDINGS{arning1996linear,
  author = {Arning, Andreas and Agrawal, Rakesh and Raghavan, Prabhakar},
  title = {A Linear Method for Deviation Detection in Large Databases.},
  booktitle = {KDD},
  year = {1996}
}

@ARTICLE{arulselvan2014note,
  author = {Arulselvan, Ashwin},
  title = {A note on the set union knapsack problem},
  journal = {Discrete Applied Mathematics},
  year = {2014},
  volume = {169},
  publisher = {Elsevier}
}

@ARTICLE{asahiro2002complexity,
  author = {Asahiro, Yuichi and Hassin, Refael and Iwama, Kazuo},
  title = {Complexity of finding dense subgraphs},
  journal = {Discrete Applied Mathematics},
  year = {2002},
  volume = {121},
  pages = {15--26},
  number = {1-3},
  publisher = {Elsevier}
}

@ARTICLE{barron1998,
  author = {Barron, Andrew and Rissanen, Jorma and Yu, Bin},
  title = {The minimum description length principle in coding and modeling},
  journal = {IEEE Transactions on Information Theory},
  year = {1998},
  volume = {44},
  number = {6},
  publisher = {IEEE}
}

@INCOLLECTION{ben2005outlier,
  author = {Ben-Gal, Irad},
  title = {Outlier detection},
  booktitle = {Data mining and knowledge discovery handbook},
  publisher = {Springer},
  year = {2005}
}

@ARTICLE{bengio2003neural,
  author = {Bengio, Yoshua and Ducharme, R{\'e}jean and Vincent, Pascal and Jauvin,
	Christian},
  title = {A neural probabilistic language model},
  journal = {Journal of machine learning research},
  year = {2003},
  volume = {3},
  pages = {1137--1155},
  number = {Feb}
}

@ARTICLE{benjamini1995controlling,
  author = {Benjamini, Yoav and Hochberg, Yosef},
  title = {Controlling the false discovery rate: a practical and powerful approach
	to multiple testing},
  journal = {Journal of the Royal statistical society: series B (Methodological)},
  year = {1995}
}

@ARTICLE{berti2018discovery,
  author = {Berti-Equille, Laure and Harmouch, Hazar and Naumann, Felix and Novelli,
	No{\"e}l and Thirumuruganathan, Saravanan},
  title = {Discovery of genuine functional dependencies from relational data
	with missing values},
  journal = {VLDB},
  year = {2018}
}

@INPROCEEDINGS{bex2006,
  author = {Bex, Geert Jan and Neven, Frank and Schwentick, Thomas and Tuyls,
	Karl},
  title = {Inference of concise DTDs from XML data},
  booktitle = {VLDB},
  year = {2006}
}

@BOOK{biemann2011structure,
  title = {Structure discovery in natural language},
  publisher = {Springer Science \& Business Media},
  year = {2011},
  author = {Biemann, Chris and van den Bosch, Antal}
}

@INPROCEEDINGS{bohannon2005cost,
  author = {Bohannon, Philip and Fan, Wenfei and Flaster, Michael and Rastogi,
	Rajeev},
  title = {A cost-based model and effective heuristic for repairing constraints
	by value modification},
  booktitle = {Proceedings of the 2005 ACM SIGMOD international conference on Management
	of data},
  year = {2005},
  pages = {143--154},
  organization = {ACM}
}

@INPROCEEDINGS{bohannon2007,
  author = {Bohannon, Philip and Fan, Wenfei and Geerts, Floris and Jia, Xibei
	and Kementsietsidis, Anastasios},
  title = {Conditional functional dependencies for data cleaning},
  booktitle = {ICDE},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{breck2019data,
  author = {Breck, Eric and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven
	and Zinkevich, Martin},
  title = {Data Validation for Machine Learning},
  booktitle = {Conference on Systems and Machine Learning (SysML). https://www.
	sysml. cc/doc/2019/167. pdf},
  year = {2019}
}

@ARTICLE{brewer2012cap,
  author = {Brewer, Eric},
  title = {CAP Twelve years Later: how the},
  journal = {Computer},
  year = {2012},
  number = {2},
  publisher = {IEEE}
}

@ARTICLE{bruglieri2004cardinality,
  author = {Bruglieri, Maurizio and Maffioli, Francesco and Ehrgott, Matthias},
  title = {Cardinality constrained minimum cut problems: complexity and algorithms},
  journal = {Discrete Applied Mathematics},
  year = {2004},
  volume = {137},
  pages = {311--341},
  number = {3},
  publisher = {Elsevier}
}

@ARTICLE{cafarella2008,
  author = {Cafarella, Michael J and Halevy, Alon and Wang, Daisy Zhe and Wu,
	Eugene and Zhang, Yang},
  title = {Webtables: exploring the power of tables on the web},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{casellar,
  author = {Casella, George and Berger, Roger},
  title = {R. 2001, Statistical Inference},
  journal = {Duxbury Press}
}

@BOOK{casella2002statistical,
  title = {Statistical inference},
  publisher = {Duxbury Pacific Grove, CA},
  year = {2002},
  author = {Casella, George and Berger, Roger L},
  volume = {2}
}

@ARTICLE{webtables,
  author = {Chakrabarti, Kaushik and Chaudhuri, Surajit and Chen, Zhimin and
	Ganjam, Kris and He, Yeye and Redmond, WA},
  title = {Data services leveraging Bing's data assets.},
  journal = {IEEE Data Eng. Bull.},
  year = {2016},
  volume = {39},
  number = {3}
}

@ARTICLE{chandola2009anomaly,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Anomaly detection: A survey},
  journal = {ACM computing surveys (CSUR)},
  year = {2009},
  volume = {41},
  number = {3},
  publisher = {ACM}
}

@ARTICLE{chandola2007,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Outlier detection: A survey},
  journal = {ACM Computing Surveys},
  year = {2007}
}

@INPROCEEDINGS{chen1996empirical,
  author = {Chen, Stanley F and Goodman, Joshua},
  title = {An empirical study of smoothing techniques for language modeling},
  booktitle = {Proceedings of the 34th annual meeting on Association for Computational
	Linguistics},
  year = {1996},
  organization = {ACL}
}

@ARTICLE{chen2014fast,
  author = {Chen, Zhimin and Narasayya, Vivek and Chaudhuri, Surajit},
  title = {Fast foreign-key detection in Microsoft SQL server PowerPivot for
	Excel},
  journal = {Proceedings of the VLDB Endowment},
  year = {2014},
  volume = {7},
  pages = {1417--1428},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{cheung2016,
  author = {Cheung, Shing-Chi and Chen, Wanjun and Liu, Yepang and Xu, Chang},
  title = {CUSTODES: automatic spreadsheet cell clustering and smell detection
	using strong and weak features},
  booktitle = {Proceedings of the 38th International Conference on Software Engineering},
  year = {2016}
}

@ARTICLE{Chiang2008,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {Proceedings of the VLDB Endowment},
  year = {2008},
  volume = {1},
  pages = {1166--1177},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{chiang2008discovering,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2015tegra,
  author = {Chu, Xu and He, Yeye and Chakrabarti, Kaushik and Ganjam, Kris},
  title = {Tegra: Table extraction by global record alignment},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{chu2013,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{chu2013discovering,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2013holistic,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Holistic data cleaning: Putting violations into context},
  booktitle = {ICDE},
  year = {2013},
  organization = {IEEE}
}

@INPROCEEDINGS{chu2015,
  author = {Chu, Xu and Morcos, John and Ilyas, Ihab F and Ouzzani, Mourad and
	Papotti, Paolo and Tang, Nan and Ye, Yin},
  title = {Katara: A data cleaning system powered by knowledge bases and crowdsourcing},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{church1990word,
  author = {Church, Kenneth Ward and Hanks, Patrick},
  title = {Word association norms, mutual information, and lexicography},
  journal = {Computational linguistics},
  year = {1990},
  volume = {16},
  number = {1},
  publisher = {MIT Press}
}

@ARTICLE{clauset2009power,
  author = {Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, Mark EJ},
  title = {Power-law distributions in empirical data},
  journal = {SIAM review},
  year = {2009},
  volume = {51},
  number = {4},
  publisher = {SIAM}
}

@INPROCEEDINGS{collobert2008unified,
  author = {Collobert, Ronan and Weston, Jason},
  title = {A unified architecture for natural language processing: Deep neural
	networks with multitask learning},
  booktitle = {Proceedings of the 25th international conference on Machine learning},
  year = {2008},
  pages = {160--167},
  organization = {ACM}
}

@INPROCEEDINGS{cong2007,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {VLDB},
  year = {2007}
}

@INPROCEEDINGS{cong2007improving,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {Proceedings of the 33rd international conference on Very large data
	bases},
  year = {2007},
  pages = {315--326},
  organization = {VLDB Endowment}
}

@ARTICLE{cormode2005improved,
  author = {Cormode, Graham and Muthukrishnan, Shan},
  title = {An improved data stream summary: the count-min sketch and its applications},
  journal = {Journal of Algorithms},
  year = {2005},
  volume = {55},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{cormode2005summarizing,
  author = {Cormode, Graham and Muthukrishnan, S},
  title = {Summarizing and mining skewed data streams},
  booktitle = {Proceedings of the 2005 SIAM International Conference on Data Mining},
  year = {2005},
  organization = {SIAM}
}

@INPROCEEDINGS{dasu2002mining,
  author = {Dasu, Tamraparni and Johnson, Theodore and Muthukrishnan, Shanmugauelayut
	and Shkapenyuk, Vladislav},
  title = {Mining database structure; or, how to build a data quality browser},
  booktitle = {SIGMOD},
  year = {2002}
}

@INPROCEEDINGS{dayal2009data,
  author = {Dayal, Umeshwar and Castellanos, Malu and Simitsis, Alkis and Wilkinson,
	Kevin},
  title = {Data integration flows for business intelligence},
  booktitle = {Proceedings of the 12th International Conference on Extending Database
	Technology: Advances in Database Technology},
  year = {2009},
  pages = {1--11}
}

@INPROCEEDINGS{deng2017data,
  author = {Deng, Dong and Fernandez, Raul Castro and Abedjan, Ziawasch and Wang,
	Sibo and Stonebraker, Michael and Elmagarmid, Ahmed K and Ilyas,
	Ihab F and Madden, Samuel and Ouzzani, Mourad and Tang, Nan},
  title = {The Data Civilizer System.},
  booktitle = {Cidr},
  year = {2017}
}

@Misc{Enterprise2016,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@INPROCEEDINGS{fan2014,
  author = {Fan, Grace and Fan, Wenfei and Geerts, Floris},
  title = {Detecting errors in numeric attributes},
  booktitle = {International Conference on Web-Age Information Management},
  year = {2014},
  organization = {Springer}
}

@ARTICLE{fan2009reasoning,
  author = {Fan, Wenfei and Jia, Xibei and Li, Jianzhong and Ma, Shuai},
  title = {Reasoning about record matching rules},
  journal = {VLDB},
  year = {2009},
  volume = {2},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{fisher2005pads,
  author = {Fisher, Kathleen and Gruber, Robert},
  title = {PADS: a domain-specific language for processing ad hoc data},
  journal = {ACM Sigplan Notices},
  year = {2005},
  volume = {40},
  pages = {295--304},
  number = {6},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{fisher2008dirt,
  author = {Fisher, Kathleen and Walker, David and Zhu, Kenny Q and White, Peter},
  title = {From dirt to shovels: fully automatic tool generation from ad hoc
	data},
  journal = {ACM SIGPLAN Notices},
  year = {2008},
  volume = {43},
  pages = {421--434},
  number = {1},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{freeman1996make,
  author = {Freeman, David},
  title = {How to make spreadsheets error-proof},
  journal = {Journal of Accountancy},
  year = {1996},
  volume = {181},
  number = {5},
  publisher = {American Institute of Certified Public Accountants}
}

@INPROCEEDINGS{ganjisaffar2011qspell,
  author = {Ganjisaffar, Yasser and Zilio, Andrea and Javanmardi, Sara and Cetindil,
	Inci and Sikka, Manik and Katumalla, Sandeep and Khatib, Narges and
	Li, Chen and Lopes, Cristina},
  title = {qspell: Spelling correction of web search queries using ranking models
	and iterative correction},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{geerts2013llunatic,
  author = {Geerts, Floris and Mecca, Giansalvatore and Papotti, Paolo and Santoro,
	Donatello},
  title = {The LLUNATIC data-cleaning framework},
  journal = {Proceedings of the VLDB Endowment},
  year = {2013},
  volume = {6},
  pages = {625--636},
  number = {9},
  publisher = {VLDB Endowment}
}

@BOOK{gennick2010sql,
  title = {SQL Pocket Guide: A Guide to SQL Usage},
  publisher = {" O'Reilly Media, Inc."},
  year = {2010},
  author = {Gennick, Jonathan}
}

@ARTICLE{go2009twitter,
  author = {Go, Alec and Bhayani, Richa and Huang, Lei},
  title = {Twitter sentiment classification using distant supervision},
  journal = {CS224N Project Report, Stanford},
  year = {2009},
  volume = {1},
  number = {2009}
}

@ARTICLE{golab2010data,
  author = {Golab, Lukasz and Karloff, Howard and Korn, Flip and Srivastava,
	Divesh},
  title = {Data auditor: Exploring data quality and semantics using pattern
	tableaux},
  journal = {VLDB},
  year = {2010},
  volume = {3},
  number = {1-2},
  publisher = {VLDB Endowment}
}

@ARTICLE{goldschmidt1994polynomial,
  author = {Goldschmidt, Olivier and Hochbaum, Dorit S},
  title = {A polynomial algorithm for the k-cut problem for fixed k},
  journal = {Mathematics of operations research},
  year = {1994},
  volume = {19},
  pages = {24--37},
  number = {1},
  publisher = {INFORMS}
}

@ARTICLE{gulwani2012,
  author = {Gulwani, Sumit and Harris, William R and Singh, Rishabh},
  title = {Spreadsheet data manipulation using examples},
  journal = {Communications of the ACM},
  year = {2012},
  volume = {55},
  number = {8},
  publisher = {ACM}
}

@ARTICLE{gupta2014outlier,
  author = {Gupta, Manish and Gao, Jing and Aggarwal, Charu C and Han, Jiawei},
  title = {Outlier detection for temporal data: A survey},
  journal = {TKDE},
  year = {2014},
  volume = {26},
  number = {9},
  publisher = {IEEE}
}

@INPROCEEDINGS{halevy2016goods,
  author = {Halevy, Alon and Korn, Flip and Noy, Natalya F and Olston, Christopher
	and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong},
  title = {Goods: Organizing google's datasets},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{hall1992smoothed,
  author = {Hall, Peter and Marron, JS and Park, Byeong U},
  title = {Smoothed cross-validation},
  journal = {Probability theory and related fields},
  year = {1992},
  volume = {92},
  number = {1},
  publisher = {Springer}
}

@INPROCEEDINGS{harris2011spreadsheet,
  author = {Harris, William R and Gulwani, Sumit},
  title = {Spreadsheet table transformations from examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2011},
  volume = {46},
  number = {6},
  organization = {ACM}
}

@INPROCEEDINGS{he2016interactive,
  author = {He, Jian and Veltri, Enzo and Santoro, Donatello and Li, Guoliang
	and Mecca, Giansalvatore and Papotti, Paolo and Tang, Nan},
  title = {Interactive and deterministic data cleaning},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{he2018transform,
  author = {He, Yeye and Chu, Xu and Ganjam, Kris and Zheng, Yudian and Narasayya,
	Vivek and Chaudhuri, Surajit},
  title = {{Transform-data-by-example (TDE): an extensible search engine for
	data transformations}},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {10},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015sema,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2005,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  journal = {Advances in Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{he2005optimization,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  booktitle = {International Conference on Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{heer2015predictive,
  author = {Heer, Jeffrey and Hellerstein, Joseph M and Kandel, Sean},
  title = {Predictive Interaction for Data Transformation.},
  booktitle = {CIDR},
  year = {2015}
}

@ARTICLE{hellerstein2008,
  author = {Hellerstein, Joseph M},
  title = {Quantitative data cleaning for large databases},
  journal = {United Nations Economic Commission for Europe (UNECE)},
  year = {2008}
}

@INPROCEEDINGS{hochbaum,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@INPROCEEDINGS{hochbaum1996approximating,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@ARTICLE{hodge2004survey,
  author = {Hodge, Victoria and Austin, Jim},
  title = {A survey of outlier detection methodologies},
  journal = {Artificial intelligence review},
  year = {2004}
}

@INPROCEEDINGS{huang2018auto,
  author = {Huang, Zhipeng and He, Yeye},
  title = {{Auto-Detect: Data-Driven Error Detection in Tables}},
  booktitle = {SIGMOD},
  year = {2018}
}

@ARTICLE{huhtala1999tane,
  author = {Huhtala, Yka and K{\"a}rkk{\"a}inen, Juha and Porkka, Pasi and Toivonen,
	Hannu},
  title = {TANE: An efficient algorithm for discovering functional and approximate
	dependencies},
  journal = {The computer journal},
  year = {1999},
  volume = {42},
  number = {2},
  publisher = {OUP}
}

@BOOK{Ben-Gal05,
  title = {Data Mining and Knowledge Discovery Handbook: A Complete Guide for
	Practitioners and Researchers},
  publisher = {Kluwer Academic Publishers},
  year = {2005},
  author = {Ben-Gal I.},
  owner = {yeyehe},
  timestamp = {2018.10.02}
}

@INPROCEEDINGS{ilyas2018extracting,
  author = {Ilyas, Andrew and da Trindade, Joana MF and Fernandez, Raul Castro
	and Madden, Samuel},
  title = {Extracting syntactical patterns from databases},
  booktitle = {2018 IEEE 34th International Conference on Data Engineering (ICDE)},
  year = {2018},
  pages = {41--52},
  organization = {IEEE}
}

@INPROCEEDINGS{ilyas2004,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{ilyas2004cords,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{jin2017foofah,
  author = {Jin, Zhongjun and Anderson, Michael R and Cafarella, Michael and
	Jagadish, HV},
  title = {Foofah: Transforming data by example},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {683--698},
  organization = {ACM}
}

@INPROCEEDINGS{kandel2011wrangler,
  author = {Kandel, Sean and Paepcke, Andreas and Hellerstein, Joseph and Heer,
	Jeffrey},
  title = {Wrangler: Interactive visual specification of data transformation
	scripts},
  booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing
	Systems},
  year = {2011},
  pages = {3363--3372},
  organization = {ACM}
}

@ARTICLE{kazai2013analysis,
  author = {Kazai, Gabriella and Kamps, Jaap and Milic-Frayling, Natasa},
  title = {An analysis of human factors and label accuracy in crowdsourcing
	relevance judgments},
  journal = {Information retrieval},
  year = {2013},
  volume = {16},
  number = {2},
  publisher = {Springer}
}

@INPROCEEDINGS{keogh2004towards,
  author = {Keogh, Eamonn and Lonardi, Stefano and Ratanamahatana, Chotirat Ann},
  title = {Towards parameter-free data mining},
  booktitle = {SIGKDD},
  year = {2004}
}

@ARTICLE{khuller1999budgeted,
  author = {Khuller, Samir and Moss, Anna and Naor, Joseph Seffi},
  title = {The budgeted maximum coverage problem},
  journal = {Information Processing Letters},
  year = {1999},
  volume = {70},
  number = {1},
  publisher = {Elsevier}
}

@ARTICLE{kivinen1995approximate,
  author = {Kivinen, Jyrki and Mannila, Heikki},
  title = {Approximate inference of functional dependencies from relations},
  journal = {Theoretical Computer Science},
  year = {1995},
  volume = {149},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{knox1998algorithms,
  author = {Knox, Edwin M and Ng, Raymond T},
  title = {Algorithms for mining distance based outliers in large datasets},
  booktitle = {VLDB},
  year = {1998}
}

@TECHREPORT{BoostClean,
  author = {Sanjay Krishnan and Michael J. Franklin and Ken Goldberg and Eugene
	Wu},
  title = {BoostClean: Automated Error Detection and Repair for Machine Learning},
  year = {2017},
  owner = {yeye},
  timestamp = {2018.02.15}
}

@ARTICLE{krishnan2016activeclean,
  author = {Krishnan, Sanjay and Wang, Jiannan and Wu, Eugene and Franklin, Michael
	J and Goldberg, Ken},
  title = {ActiveClean: interactive data cleaning for statistical modeling},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{imagenet,
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  title = {Imagenet classification with deep convolutional neural networks},
  booktitle = {Advances in neural information processing systems},
  year = {2012}
}

@INPROCEEDINGS{Le2014,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  pages = {542--553},
  organization = {ACM}
}

@INPROCEEDINGS{le2014flashextract,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  organization = {ACM}
}

@BOOK{lee1997bayesian,
  title = {Bayesian statistics},
  publisher = {Arnold Publication},
  year = {1997},
  author = {Lee, Peter M}
}

@BOOK{lehmann2006testing,
  title = {Testing statistical hypotheses},
  publisher = {Springer Science \& Business Media},
  year = {2006},
  author = {Lehmann, Erich L and Romano, Joseph P}
}

@ARTICLE{leys2013detecting,
  author = {Leys, Christophe and Ley, Christophe and Klein, Olivier and Bernard,
	Philippe and Licata, Laurent},
  title = {Detecting outliers: Do not use standard deviation around the mean,
	use absolute deviation around the median},
  journal = {Journal of Experimental Social Psychology},
  year = {2013},
  volume = {49},
  number = {4},
  publisher = {Elsevier}
}

@INPROCEEDINGS{li2006exploring,
  author = {Li, Mu and Zhang, Yang and Zhu, Muhua and Zhou, Ming},
  title = {Exploring distributional similarity based models for query spelling
	correction},
  booktitle = {Proceedings of the 21st International Conference on Computational
	Linguistics and the 44th annual meeting of the Association for Computational
	Linguistics},
  year = {2006},
  organization = {ACL}
}

@INPROCEEDINGS{li2008regular,
  author = {Li, Yunyao and Krishnamurthy, Rajasekar and Raghavan, Sriram and
	Vaithyanathan, Shivakumar and Jagadish, HV},
  title = {Regular expression learning for information extraction},
  booktitle = {Proceedings of the Conference on Empirical Methods in Natural Language
	Processing},
  year = {2008},
  organization = {ACL}
}

@BOOK{lieberman2001your,
  title = {Your wish is my command: Programming by example},
  publisher = {Morgan Kaufmann},
  year = {2001},
  author = {Lieberman, Henry}
}

@ARTICLE{Forrester,
  author = {Cinny Little},
  title = {The Forrester Wave: Data Preparation Solutions, Q4 2018},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@ARTICLE{liu2009learning,
  author = {Liu, Tie-Yan and others},
  title = {Learning to rank for information retrieval},
  journal = {Foundations and Trends{\textregistered} in Information Retrieval},
  year = {2009},
  volume = {3},
  pages = {225--331},
  number = {3},
  publisher = {Now Publishers, Inc.}
}

@ARTICLE{lopes2002,
  author = {Lopes, St{\'e}phane and Petit, Jean-Marc and Lakhal, Lotfi},
  title = {Functional and approximate dependency mining: database and FCA points
	of view},
  journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
  year = {2002}
}

@INPROCEEDINGS{luec2011data,
  author = {Luec, Gord},
  title = {A data-driven approach for correcting search quaries},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{manning2008scoring,
  author = {Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  title = {Scoring, term weighting and the vector space model},
  journal = {Introduction to information retrieval},
  year = {2008},
  volume = {100},
  publisher = {Cambridge University Press}
}

@BOOK{pooling,
  title = {Evaluation in information retrieval, Stanford NLP Group, \url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparaGroup}},
  publisher = {Cambridge University Press},
  author = {Christopher D. Manning and Prabhakar Raghavan and Hinrich Schutze},
  owner = {yeyehe},
  timestamp = {2019.02.14},
  url = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}}
}

@ARTICLE{mariet2016outlier,
  author = {Mariet, Zelda and Harding, Rachael and Madden, Sam and others},
  title = {Outlier Detection in Heterogeneous Datasets using Automatic Tuple
	Expansion},
  journal = {MIT Technical Report},
  year = {2016}
}

@ARTICLE{Ziemann16,
  author = {Mark Ziemann, Yotam Eren and Assam El-Osta},
  title = {Gene name errors are widespread in the scientific literature},
  journal = {Genome Biology},
  year = {2016},
  owner = {yeyehe},
  timestamp = {2018.10.01}
}

@ARTICLE{maronna1976robust,
  author = {Maronna, Ricardo Antonio},
  title = {Robust M-estimators of multivariate location and scatter},
  journal = {The annals of statistics},
  year = {1976},
  publisher = {JSTOR}
}

@BOOK{maronna2018robust,
  title = {Robust Statistics: Theory and Methods (with R)},
  publisher = {Wiley},
  year = {2018},
  author = {Maronna, Ricardo A and Martin, R Douglas and Yohai, Victor J and
	Salibi{\'a}n-Barrera, Mat{\'\i}as}
}

@INPROCEEDINGS{differential-privacy,
  author = {McSherry, Frank and Talwar, Kunal},
  title = {Mechanism design via differential privacy},
  booktitle = {Foundations of Computer Science, 2007. FOCS'07. 48th Annual IEEE
	Symposium on},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{mikolov2010recurrent,
  author = {Mikolov, Tom{\'a}{\v{s}} and Karafi{\'a}t, Martin and Burget, Luk{\'a}{\v{s}}
	and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  title = {Recurrent neural network based language model},
  booktitle = {Eleventh annual conference of the international speech communication
	association},
  year = {2010}
}

@INPROCEEDINGS{word2vec,
  author = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg
	S and Dean, Jeff},
  title = {Distributed representations of words and phrases and their compositionality},
  booktitle = {Advances in neural information processing systems},
  year = {2013}
}

@INPROCEEDINGS{mintz2009distant,
  author = {Mintz, Mike and Bills, Steven and Snow, Rion and Jurafsky, Dan},
  title = {Distant supervision for relation extraction without labeled data},
  booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of
	the ACL and the 4th International Joint Conference on Natural Language
	Processing of the AFNLP: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@BOOK{neter1996applied,
  title = {Applied linear statistical models},
  publisher = {Irwin Chicago},
  year = {1996},
  author = {Neter, John and Kutner, Michael H and Nachtsheim, Christopher J and
	Wasserman, William},
  volume = {4}
}

@ARTICLE{Neyman33,
  author = {Neyman, J. and Pearson, E. S.},
  title = {On the problem of the most efficient tests of statistical hypotheses},
  journal = {Phil. Trans. R. Soc. Lond. A.},
  year = {1933}
}

@ARTICLE{padhi2017flashprofile,
  author = {Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov,
	Oleksandr and Gulwani, Sumit and Millstein, Todd D},
  title = {FlashProfile: Interactive Synthesis of Syntactic Profiles.},
  year = {2017}
}

@INPROCEEDINGS{pande2017effective,
  author = {Pande, Harshit},
  title = {Effective search space reduction for spell correction using character
	neural embeddings},
  booktitle = {Proceedings of the 15th Conference of the European Chapter of the
	ACL: Volume 2, Short Papers},
  year = {2017},
  volume = {2}
}

@INPROCEEDINGS{panko2008,
  author = {Panko, Raymond R},
  title = {Spreadsheet errors: What we know. what we think we can do},
  year = {2008},
  journal = {Symposium on Risk of Spreadsheets}
}

@ARTICLE{panko1998,
  author = {Panko, Raymond R},
  title = {What we know about spreadsheet errors},
  journal = {Journal of Organizational and End User Computing (JOEUC)},
  year = {1998}
}

@ARTICLE{papenbrock2015data,
  author = {Papenbrock, Thorsten and Bergmann, Tanja and Finke, Moritz and Zwiener,
	Jakob and Naumann, Felix},
  title = {Data profiling with metanome},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{parzen1962estimation,
  author = {Parzen, Emanuel},
  title = {On estimation of a probability density function and mode},
  journal = {The annals of mathematical statistics},
  year = {1962},
  volume = {33},
  number = {3},
  publisher = {JSTOR}
}

@INPROCEEDINGS{patel2019big,
  author = {Patel, Hiren and Jindal, Alekh and Szyperski, Clemens},
  title = {Big Data Processing at Microsoft: Hyper Scale, Massive Complexity,
	and Minimal Cost},
  booktitle = {Proceedings of the ACM Symposium on Cloud Computing},
  year = {2019},
  pages = {490--490}
}

@INPROCEEDINGS{polyzotis2017data,
  author = {Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong and Zinkevich,
	Martin},
  title = {Data management challenges in production machine learning},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {1723--1726}
}

@INPROCEEDINGS{powell2009,
  author = {Powell, Stephen G and Baker, Kenneth R and Lawson, Barry},
  title = {Errors in operational spreadsheets: A review of the state of the
	art},
  booktitle = {System Sciences, 2009. HICSS'09},
  year = {2009}
}

@INPROCEEDINGS{priedhorsky2007creating,
  author = {Priedhorsky, Reid and Chen, Jilin and Lam, Shyong Tony K and Panciera,
	Katherine and Terveen, Loren and Riedl, John},
  title = {Creating, destroying, and restoring value in Wikipedia},
  booktitle = {Proceedings of the 2007 international ACM conference on Supporting
	group work},
  year = {2007},
  organization = {ACM}
}

@INPROCEEDINGS{qahtan2018fahes,
  author = {Qahtan, Abdulhakim and Elmagarmid, Ahmed and Ouzzani, Mourad and
	Tang, Nan},
  title = {FAHES: Detecting disguised missing values},
  booktitle = {ICDE},
  year = {2018},
  organization = {IEEE}
}

@ARTICLE{rahman2018icarus,
  author = {Rahman, Protiva and Hebert, Courtney and Nandi, Arnab},
  title = {ICARUS: minimizing human effort in iterative data completion},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{squad,
  author = {Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang,
	Percy},
  title = {Squad: 100,000+ questions for machine comprehension of text},
  journal = {arXiv preprint arXiv:1606.05250},
  year = {2016}
}

@INPROCEEDINGS{raman2001potter,
  author = {Raman, Vijayshankar and Hellerstein, Joseph M},
  title = {Potter's wheel: An interactive data cleaning system},
  booktitle = {VLDB},
  year = {2001},
  volume = {1}
}

@ARTICLE{holoclean,
  author = {Rekatsinas, Theodoros and Chu, Xu and Ilyas, Ihab F and R{\'e}, Christopher},
  title = {Holoclean: Holistic data repairs with probabilistic inference},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {11},
  publisher = {VLDB Endowment}
}

@ARTICLE{rousseeuw1993alternatives,
  author = {Rousseeuw, Peter J and Croux, Christophe},
  title = {Alternatives to the median absolute deviation},
  journal = {Journal of the American Statistical association},
  year = {1993},
  volume = {88},
  number = {424},
  publisher = {Taylor \& Francis}
}

@BOOK{rozenberg2012handbook,
  title = {Handbook of Formal Languages: Volume 3 Beyond Words},
  publisher = {Springer Science \& Business Media},
  year = {2012},
  author = {Rozenberg, Grzegorz and Salomaa, Arto}
}

@BOOK{Schutze2008,
  title = {Introduction to information retrieval},
  publisher = {Cambridge University Press},
  year = {2008},
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  volume = {39}
}

@INPROCEEDINGS{schutze2008introduction,
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  title = {Introduction to information retrieval},
  booktitle = {Proceedings of the international communication of association for
	computing machinery conference},
  year = {2008},
  pages = {260}
}

@INPROCEEDINGS{schelter2019unit,
  author = {Schelter, Sebastian and Biessmann, Felix and Lange, Dustin and Rukat,
	Tammo and Schmidt, Phillipp and Seufert, Stephan and Brunelle, Pierre
	and Taptunov, Andrey},
  title = {Unit Testing Data with Deequ},
  booktitle = {Proceedings of the 2019 International Conference on Management of
	Data},
  year = {2019},
  pages = {1993--1996}
}

@INPROCEEDINGS{schelter2019differential,
  author = {Schelter, Sebastian and Grafberger, Stefan and Schmidt, Philipp and
	Rukat, Tammo and Kiessling, Mario and Taptunov, Andrey and Biessmann,
	Felix and Lange, Dustin},
  title = {Differential Data Quality Verification on Partitioned Data},
  booktitle = {2019 IEEE 35th International Conference on Data Engineering (ICDE)},
  year = {2019},
  pages = {1940--1945},
  organization = {IEEE}
}

@ARTICLE{schelter2018automating,
  author = {Schelter, Sebastian and Lange, Dustin and Schmidt, Philipp and Celikel,
	Meltem and Biessmann, Felix and Grafberger, Andreas},
  title = {Automating large-scale data quality verification},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {1781--1794},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{shachaf2010beyond,
  author = {Shachaf, Pnina and Hara, Noriko},
  title = {Beyond vandalism: Wikipedia trolls},
  journal = {Journal of Information Science},
  year = {2010},
  volume = {36},
  number = {3},
  publisher = {Sage Publications Sage UK: London, England}
}

@inproceedings{swami2020data,
  title={Data Sentinel: A Declarative Production-Scale Data Validation Platform},
  author={Swami, Arun and Vasudevan, Sriram and Huyn, Joojay},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={1579--1590},
  year={2020},
  organization={IEEE}
}


@ARTICLE{singh2016blinkfill,
  author = {Singh, Rishabh},
  title = {Blinkfill: Semi-supervised programming by example for syntactic string
	transformations},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {10},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{singh2016transforming,
  author = {Singh, Rishabh and Gulwani, Sumit},
  title = {Transforming spreadsheet data types using examples},
  booktitle = {Acm Sigplan Notices},
  year = {2016}
}

@ARTICLE{singhmelford,
  author = {Singh, Rishabh and Livshits, Benjamin and Zorn, Benjamin},
  title = {Melford: Using Neural Networks to Find Spreadsheet Errors},
  journal = {MSR technical report}
}

@ARTICLE{stoer1997simple,
  author = {Stoer, Mechthild and Wagner, Frank},
  title = {A simple min-cut algorithm},
  journal = {Journal of the ACM (JACM)},
  year = {1997},
  volume = {44},
  pages = {585--591},
  number = {4},
  publisher = {ACM}
}

@INPROCEEDINGS{surdeanu2010simple,
  author = {Surdeanu, Mihai and McClosky, David and Tibshirani, Julie and Bauer,
	John and Chang, Angel X and Spitkovsky, Valentin I and Manning, Christopher
	D},
  title = {A Simple Distant Supervision Approach for the TAC-KBP Slot Filling
	Task.},
  booktitle = {TAC},
  year = {2010}
}

@ARTICLE{tax2004support,
  author = {Tax, David MJ and Duin, Robert PW},
  title = {Support vector data description},
  journal = {Machine learning},
  year = {2004},
  volume = {54},
  number = {1},
  publisher = {Springer}
}

@BOOK{voorhees2005trec,
  title = {TREC: Experiment and evaluation in information retrieval},
  publisher = {MIT press Cambridge},
  year = {2005},
  author = {Voorhees, Ellen M and Harman, Donna K and others},
  volume = {1}
}

@INPROCEEDINGS{wang2017,
  author = {Wang, Yue and He, Yeye},
  title = {Synthesizing mapping relationships using table corpus},
  booktitle = {SIGMOD},
  year = {2017}
}

@INPROCEEDINGS{whitelaw2009using,
  author = {Whitelaw, Casey and Hutchinson, Ben and Chung, Grace Y and Ellis,
	Gerard},
  title = {Using the web for language independent spellchecking and autocorrection},
  booktitle = {Proceedings of the 2009 Conference on Empirical Methods in Natural
	Language Processing: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@ARTICLE{yaghmazadeh2018automated,
  author = {Yaghmazadeh, Navid and Wang, Xinyu and Dillig, Isil},
  title = {Automated migration of hierarchical data to relational tables using
	programming-by-example},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {580--593},
  number = {5},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{yakout2013don,
  author = {Yakout, Mohamed and Berti-{\'E}quille, Laure and Elmagarmid, Ahmed
	K},
  title = {Don't be SCAREd: use SCalable Automatic REpairing with maximal likelihood
	and bounded changes},
  booktitle = {SIGMOD},
  year = {2013}
}

@INPROCEEDINGS{yan18,
  author = {Cong Yan and Yeye He},
  title = {Synthesizing Type-Detection Logic using Open-source Code},
  booktitle = {SIGMOD},
  year = {2018},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@INPROCEEDINGS{yan2018synthesizing,
  author = {Yan, Cong and He, Yeye},
  title = {{Auto-Type: Synthesizing type-detection logic for rich semantic data
	types using open-source code}},
  booktitle = {Proceedings of the 2018 International Conference on Management of
	Data},
  year = {2018},
  organization = {ACM}
}

@INPROCEEDINGS{yu2011,
  author = {Yu, Yang and Heflin, Jeff},
  title = {Extending functional dependency to detect abnormal data in RDF graphs},
  booktitle = {International Semantic Web Conference},
  year = {2011},
  organization = {Springer}
}

@INPROCEEDINGS{zhai2017study,
  author = {Zhai, Chengxiang and Lafferty, John},
  title = {A study of smoothing methods for language models applied to ad hoc
	information retrieval},
  booktitle = {ACM SIGIR Forum},
  year = {2017},
  organization = {ACM}
}

@INPROCEEDINGS{auto-em,
  author = {Chen Zhao and Yeye He},
  title = {{Auto-EM: End-to-end Fuzzy Entity-Matching using Pre-trained Deep
	Models and Transfer Learning}},
  booktitle = {WWW},
  year = {2019}
}

@INPROCEEDINGS{zhao2017controlling,
  author = {Zhao, Zheguang and De Stefani, Lorenzo and Zgraggen, Emanuel and
	Binnig, Carsten and Upfal, Eli and Kraska, Tim},
  title = {Controlling false discoveries during interactive data exploration},
  booktitle = {SIGMOD},
  year = {2017}
}

@ARTICLE{zhou2012scope,
  author = {Zhou, Jingren and Bruno, Nicolas and Wu, Ming-Chuan and Larson, Per-Ake
	and Chaiken, Ronnie and Shakib, Darren},
  title = {SCOPE: parallel databases meet MapReduce},
  journal = {The VLDB Journal},
  year = {2012},
  volume = {21},
  pages = {611--636},
  number = {5},
  publisher = {Springer}
}

@ARTICLE{zhu2017auto,
  author = {Zhu, Erkang and He, Yeye and Chaudhuri, Surajit},
  title = {Auto-join: Joining tables by leveraging transformations},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {10},
  publisher = {VLDB Endowment}
}



@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://www.nuget.org/packages/Microsoft.ProgramSynthesis.Extraction.Text/}}
}


@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/transform-model/service-dataflows-create-use}}
}

@MISC{tableau-flow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://help.tableau.com/current/prep/en-us/prep_build_flow.htm}}
}

@MISC{amazon-workflow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://aws.amazon.com/blogs/big-data/simplify-data-pipelines-with-aws-glue-automatic-code-generation-and-workflows/}}
}

@MISC{azureml-pipelines,
  title = {{Azure ML: Data Pipelines}},
  howpublished = {\url{https://docs.microsoft.com/en-us/azure/machine-learning/concept-ml-pipelines}}
}

@MISC{ataccama,
  title = {{ataccama: Data Profiling}},
  howpublished = {\url{https://www.ataccama.com/product/data-discovery-and-profiling}}
}

@MISC{Kaggle-Dropbox,
  title = {{Kaggle Expeirment, Shared via Dropbox}},
  howpublished = {\url{https://www.dropbox.com/sh/cfyv5lhzcpiv1xk/AAC5SIKCjuZZL5n5_RKHzMBwa?dl=0}}
}

@article{chaiken2008scope,
  title={SCOPE: easy and efficient parallel processing of massive data sets},
  author={Chaiken, Ronnie and Jenkins, Bob and Larson, Per-{\AA}ke and Ramsey, Bill and Shakib, Darren and Weaver, Simon and Zhou, Jingren},
  journal={Proceedings of the VLDB Endowment},
  volume={1},
  number={2},
  pages={1265--1276},
  year={2008},
  publisher={VLDB Endowment}
}


@incollection{vassiliadis2009near,
  title={Near real time ETL},
  author={Vassiliadis, Panos and Simitsis, Alkis},
  booktitle={New trends in data warehousing and data analysis},
  pages={1--31},
  year={2009},
  publisher={Springer}
}



@MISC{xgboost,
  title = {{XGBoost}},
  howpublished = {\url{https://xgboost.readthedocs.io/en/latest/}}
}



@MISC{BingEntity,
  title = {Bing Entity Search},
  howpublished = {\url{https://azure.microsoft.com/en-us/services/cognitive-services/bing-entity-search-api/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Deequ,
  title = {{Amazon Deequ Library for Data Validation}},
  howpublished = {\url{https://github.com/awslabs/deequ}}
}

@MISC{DresdenTables,
  title = {{Dresden Web Table Corpus}},
  howpublished = {\url{https://wwwdb.inf.tu-dresden.de/misc/dwtc/}}
}

@MISC{eusprig,
  title = {Spreadsheet mistakes - news stories, compiled by European Spreadsheet
	Risk Interest Group {EuSpRiG}},
  howpublished = {\url{http://www.eusprig.org/horror-stories.htm}},
  owner = {yeyehe},
  timestamp = {2017.09.26}
}

@MISC{frameapi,
  title = {Pandas Data Frame List of APIs},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/frame.html}}
}

@MISC{gartner,
  title = {Self-Service Data Preparation, Worldwide, 2016},
  howpublished = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}},
  owner = {yeyehe},
  timestamp = {2017.03.07}
}

@ARTICLE{gartner17,
  title = {Market Guide for Data Preparation - Gartner, 2017},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@MISC{GitHubv3,
  title = {GitHub API},
  howpublished = {\url{https://developer.github.com/v3/}},
  owner = {yeyehe},
  timestamp = {2019.10.21}
}

@MISC{googlewebtables,
  title = {{Google Web Tables}},
  howpublished = {\url{http://research.google.com/tables}}
}

@MISC{groupbyapi,
  title = {Pandas Groupby Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.groupby.html}}
}

@MISC{Informatica,
  title = {{Informatica Rev}},
  howpublished = {\url{https://www.informatica.com/products/data-quality/rev.html}},
  owner = {yeyehe},
  timestamp = {2016.10.21}
}

@Misc{Informatica-DQ-rules,
  title        = {{Informatica Data Quality Rules (Retrieved in 2020-02)}},
  howpublished = {\url{https://www.informatica.com/content/dam/informatica-com/en/collateral/data-sheet/en_informatica-data-quality_data-sheet_6710.pdf}},
}

@MISC{jsonapi,
  title = {Pandas Json Normalize Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.io.json.json_normalize.html}}
}

@MISC{Jupyter,
  title = {Jupyter Notebooks},
  howpublished = {\url{https://jupyter.org/}}
}

@MISC{kaggle,
  title = {Kaggle},
  howpublished = {\url{https://www.kaggle.com/}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{kaggle-dataset,
  title = {Kaggle Dataset API},
  howpublished = {\url{https://www.kaggle.com/docs/api}{interacting-with-datasets}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{meltapi,
  title = {Pandas Melt Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.melt.html}}
}

@MISC{mergeapi,
  title = {Pandas Merge Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.merge.html}}
}

@MISC{OpenRefine,
  title = {{OpenRefine (formerly Google Refine)}},
  howpublished = {\url{http://openrefine.org/}}
}

@MISC{paxata,
  title = {Paxata data preparation},
  howpublished = {\url{https://www.paxata.com/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{pivotapi,
  title = {Pandas Pivot Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.pivot_table.html}}
}

@MISC{PowerBI,
  title = {Power BI},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/desktop-data-types}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{python-trace,
  title = {{python tracing library}},
  howpublished = {\url{https://pymotw.com/2/trace/}}
}

@MISC{ssis-profiling,
  title = {{SSIS: Data Profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}}
}

@MISC{TableauPrep,
  title = {Tableau Prep},
  howpublished = {\url{https://www.tableau.com/products/prep}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Talend,
  title = {Talend data validation},
  howpublished = {\url{https://www.talendbyexample.com/talend-data-validation.html}},
  owner = {yeyehe},
  timestamp = {2017.09.28}
}

@MISC{TalendSemantic,
  title = {Talend Data Services Platform Studio User Guide: Semantic Discovery},
  howpublished = {\url{https://help.talend.com/reader/nAXiZW0j0H~2~YApZIsRFw/_u0D0oqWxesgBDSihDgbYA}},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@MISC{TFDV,
  title = {{Google TensorFlow Data Validation}},
  howpublished = {\url{https://www.tensorflow.org/tfx/guide/tfdv}}
}

@MISC{Trifacta,
  title = {Trifacta},
  howpublished = {\url{https://www.trifacta.com/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{trifacta-profiling,
  title = {{Trifacta: Data Profiling}},
  howpublished = {\url{https://www.trifacta.com/data-profiling/}}
}

@MISC{WebDataCommonsTables,
  title = {{Web Table Corpora from Web Data Commons}},
  howpublished = {\url{http://webdatacommons.org/webtables/}}
}

@MISC{wiktionary,
  title = {Excel error checking rules},
  howpublished = {\url{https://www.wiktionary.org/}},
  owner = {yeyehe},
  timestamp = {2017.09.27}
}

@MISC{word2vec-demo,
  title = {Word embedding demo},
  howpublished = {\url{http://bionlp-www.utu.fi/wv_demo/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{word2vec-for-misspellings,
  title = {{Google's trained Word2Vec model }},
  howpublished = {\url{http://mccormickml.com/2016/04/12/googles-pretrained-word2vec-model-in-python/}}
}

@OTHER{,
  owner = {yeyehe},
  timestamp = {2020.03.02}
}

@Article{karp1985fast,
  author    = {Karp, Richard M and Wigderson, Avi},
  title     = {A fast parallel algorithm for the maximal independent set problem},
  journal   = {Journal of the ACM (JACM)},
  year      = {1985},
  volume    = {32},
  number    = {4},
  pages     = {762--773},
  publisher = {ACM New York, NY, USA},
}

@Article{wang1994complexity,
  author  = {Wang, Lusheng and Jiang, Tao},
  title   = {On the complexity of multiple sequence alignment},
  journal = {Journal of computational biology},
  year    = {1994},
  volume  = {1},
  number  = {4},
  pages   = {337--348},
}

@Article{carrillo1988multiple,
  author    = {Carrillo, Humberto and Lipman, David},
  title     = {The multiple sequence alignment problem in biology},
  journal   = {SIAM journal on applied mathematics},
  year      = {1988},
  volume    = {48},
  number    = {5},
  pages     = {1073--1082},
  publisher = {SIAM},
}

@Article{just2001computational,
  author    = {Just, Winfried},
  title     = {Computational complexity of multiple sequence alignment with SP-score},
  journal   = {Journal of computational biology},
  year      = {2001},
  volume    = {8},
  number    = {6},
  pages     = {615--623},
  publisher = {Mary Ann Liebert, Inc.},
}

@Book{cormen2009introduction,
  title     = {Introduction to algorithms},
  publisher = {MIT press},
  year      = {2009},
  author    = {Cormen, Thomas H and Leiserson, Charles E and Rivest, Ronald L and Stein, Clifford},
}

@Misc{enterprise2016trifacta,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@Misc{grok,
  title        = {{Grok Patterns}},
  howpublished = {\url{https://github.com/elastic/elasticsearch/blob/master/libs/grok/src/main/resources/patterns/grok-patterns}},
}

@Misc{,
  title        = {{SQL Server SSIS profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}},
}

@Misc{Glue,
  title        = {{AWS Glue custom classifers}},
  howpublished = {\url{https://docs.aws.amazon.com/glue/latest/dg/custom-classifier.html}},
}

@Misc{xsystem-code,
  title        = {{XSystem Code}},
  howpublished = {\url{https://bitbucket.org/andrewiilyas/xsystem-old/src/outlier-detection/}},
}

@Article{stonebraker2018data,
  author  = {Stonebraker, Michael and Ilyas, Ihab F},
  title   = {Data Integration: The Current Status and the Way Forward.},
  journal = {IEEE Data Eng. Bull.},
  year    = {2018},
  volume  = {41},
  number  = {2},
  pages   = {3--9},
}

@Book{kanji2006,
  title     = {100 statistical tests},
  publisher = {Sage},
  year      = {2006},
  author    = {Kanji, Gopal K},
}

@Article{agresti1992survey,
  author    = {Agresti, Alan and others},
  title     = {A survey of exact inference for contingency tables},
  journal   = {Statistical science},
  year      = {1992},
  volume    = {7},
  number    = {1},
  pages     = {131--153},
  publisher = {Institute of Mathematical Statistics},
}

@InProceedings{hynes2017data,
  author    = {Hynes, Nick and Sculley, D and Terry, Michael},
  title     = {The data linter: Lightweight, automated sanity checking for ml data sets},
  booktitle = {NIPS MLSys Workshop},
  year      = {2017},
}

@Article{naumann2014data,
  author    = {Naumann, Felix},
  title     = {Data profiling revisited},
  journal   = {ACM SIGMOD Record},
  year      = {2014},
  volume    = {42},
  number    = {4},
  pages     = {40--49},
  publisher = {ACM New York, NY, USA},
}

@Misc{msft-ml,
  title        = {{Microsoft ML pipelines}},
  howpublished = {\url{https://www.slideshare.net/KarthikMurugesan2/microsoft-ai-platform-aether-introduction}},
}

@Comment{jabref-meta: databaseType:bibtex;}


==> paper - arxiv-full-version/architecture.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{System Architecture}

TBD



==> paper - arxiv-full-version/auto-validate-horizontal.tex <==
%!TEX root = main.tex
%\vspace{-2mm}
\section{Auto-Validate (Horizontal Cuts)}
\label{sec:horizontal-cuts}
So far we assumed the query column $C$
to be ``clean'' with homogeneous
values drawn from the same domain 
(since they are generated by the same underlying program).
While this is generally true, we observe that some
columns can have ad-hoc special values  
(e.g., denoting null/empty-values) that do
not follow the domain-pattern of $C$,
as shown in Figure~\ref{fig:example-nulls}.

\begin{figure}
        \centering
        \includegraphics[width=0.5\textwidth]{figures/example-nulls.png}
\caption{Example ad-hoc special values (in red boxes)
not observing patterns of other values in the column.}
\label{fig:example-nulls}
\end{figure}



We note that examples like these are not uncommon -- even for
machine-generated data, there can be a 
branch of logic (think of \val{try-except}) that
 handles special cases (e.g., nulls),
and produces ad-hoc values 
not following the pattern of ``normal'' values.
We henceforth refer to these as \textit{non-conforming values}.

Recall that in FMDV, by assuming that the query column $C$ has
homogeneous values, we select patterns
from $\mathbf{H}(C) = \cap_{v \in C}{\mathbf{P}(v)}$, 
or the intersection of patterns for all values  $v \in C$.
Such an assumption does not hold 
for columns in Figure~\ref{fig:example-nulls},
yielding an empty $\mathbf{H}(C)$ and
no feasible solution to FMDV.


We thus consider a variant of \sj with ``horizontal
cuts'', meaning that we can ``cut off'' a small fraction
of non-conforming values in 
$C$ (which is identical to making patterns tolerate
a small fraction of non-conforming values). 
We use a \textit{tolerance parameter}
$\theta$ to control the maximum allowed fraction of 
non-conforming values that can be cut (e.g., 1\%, 5\%, etc.), 
which allows for a conscious trade-off between 
precision and recall.

This optimization problem, termed
FMDV-H, is defined as

\begin{align}
\hspace{-1cm} \text{(FMDV-H)}~~\min_{h}~& \text{FPR}_\mathbf{T}(h)   \label{eqn:fmdvh_obj} \\ 
 \mbox{s.t.} ~~ & h \in \cup_{v\in C}{\mathbf{P}(v) \setminus \text{``.*''}} \label{eqn:fmdvh_h} \\
&  \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:fmdvh_fpr} \\
 & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:fmdvh_cov} \\
 & |\{ v | v \in C, h \in \mathbf{P}(v) \}| \geq (1-\theta) |C| \label{eqn:fmdvh_tolerance}
\end{align}

Like before, our objective function is to 
minimize FPR in Equation~\eqref{eqn:fmdvh_obj}.
Equation~\eqref{eqn:fmdvh_h} shows that the 
hypothesis pattern $h$ is drawn from
the union of possible patterns for all $v \in C$.
%(as opposed to $\mathbf{H}(C)$ in FMDV that uses intersection).
The FPR and Coverage requirements in
Equation~\eqref{eqn:fmdvh_fpr} and
Equation~\eqref{eqn:fmdvh_cov} are 
the same as the basic FMDV.
Finally, Equation~\eqref{eqn:fmdvh_tolerance} requires
that the selected $h$ has to match at least 
$(1-\theta)$ fraction of values in $C$, where $\theta$ 
is the tolerance parameter above (the remaining
 $\theta$ fraction are non-conforming values).


\begin{example}
\label{ex:fmdvh}
Consider the leftmost column $C$ in Figure~\ref{fig:example-nulls}.
Using FMDV-H, we determine the pattern $h=$
``\val{<digit>+,<digit>+,<digit>+,} \val{<digit>+,<digit>+}''
to be a valid solution, as it meets the FPR and coverage
requirements based on $\mathbf{T}$.
Furthermore $h$ is consistent with 99\% of values in $C$
(the remaining 1\% non-conforming value
is the ``\val{-}'' marked in a red box), thus also 
satisfying Equation~\eqref{eqn:fmdvh_tolerance}.
\end{example}


For arbitrary $\theta$ and generalization hierarchy,
we can show that deciding whether there is a feasible 
solution to FMDV-H is NP-hard (let alone minimizing FPR), using a reduction
from independent set~\cite{karp1985fast}.
% (e.g., by
%modeling each $v \in C$ as a vertex in a graph,
%and connecting two vertices if their corresponding
%values have no common generalized patterns
%except the trivial pattern \val{.*}).

\begin{theorem}
\label{thm:fmdvh}
The decision version of FMDV-H is NP-hard.
\end{theorem}
\begin{comment} %remove after revision
{
\begin{proof}
We show this result using a reduction from
maximum independent set~\cite{karp1985fast}. Recall that 
given a graph $G = (V, E)$ and an integer $k$, the decision version of 
independent set is to determine if there exists an independent
set $I \subseteq V$ of size $|I| \geq k$. 

Given any instance of the independent set problem, we construct
an FMDV-H problem as follows. We build a bijection
$\phi: V \rightarrow C$, so that every vertex $v_i \in V$ corresponds
to a value $c_i \in C$. Each value $c_i$ is constructed to have exactly 
$n = {|V| \choose 2}$ consecutive
tokens, where each token $t_{ij}, i < j$ maps to 
a pair of vertices $(v_i, v_j)$ in $G$. 
For each pair of vertices  $(v_i, v_j), i<j$ that
are connected in $G$, we assign the corresponding token $t_{ij}$ in
$c_i, c_j$ to values that
generalize into different branches of a constructed $H$
(e.g., one to letters and one to symbols, which would only overlap
at the root level of $H$). This ensures that whatever pattern $h$
is chosen for the entire column $C$ in FMDV-H, $c_i$ and $c_j$ 
cannot be simultaneously ``covered'' by $h$ (as in independent set). 
We assign remaining
tokens of each value $c$ to a special leaf node string that can 
generalize to all intermediate nodes of $H$ (note that $H$
can have overlapping generalizations, like in the case of Digit and Num
in Figure~\ref{fig:hierarchy}), to ensure that these tokens in $c$
are ``compatible'' with any other tokens at the same position 
in a different $c'$. It can be seen that an decision-version of 
the independent set problem with a given $k$ now directly correspond
to a decision version of FMDV-H
with $\theta = 1- \frac{k}{|V|}$ ($m$ and $r$ are set to 1 and 1,
to make them trivially satisfiable). If we could find a feasible solution to
FMDV-H with $\theta = 1- \frac{k}{|V|}$,
then we would have found a feasible solution to the independent set with $k$
using the bijection, thus completing the proof.
\end{proof}
}
\end{comment}


While FMDV-H is hard in general, in practice because
the patterns of non-conforming values often
do not intersect with those of ``normal'' values
(as in Example~\ref{ex:fmdvh}),
they create 
easier instances of FMDV-H.
Leveraging this observation, in this work 
we optimize FMDV-H greedily, by discarding
values whose patterns do not intersect
with most others in $C$.
We can then find the optimal pattern for the
remaining conforming values in FMDV-H 
using FMDV.


\textbf{Distributional test of non-conforming values.}
Given a pattern $h$ inferred from the
``training data'' $C$ using FMDV-H, and given the
data $C'$ arriving in the future, our last task is 
to determine whether the fraction of non-conforming
values in $C'$ has changed significantly from $C$.

Specifically, at ``training'' time,
we can calculate the fraction of values in $C$ not 
conforming to $h$, denoted as $\theta_{C}(h) 
= \frac{|\{ v | v \in C, h \notin \mathbf{P}(v) \}|}{|C|}$.
At ``testing'' time, we also compute the fraction of 
values in $C'$ not 
matching $h$, denoted as $\theta_{C'}(h)$.


%\revised
%\iftoggle{fullversion}{
A naive approach to validate $C'$ is to trigger alarms
if $\theta_{C'}(h)$ is greater than $\theta_{C}(h)$.
This, however, is prone to false-positives.
Imagine a scenario where we compute the non-conforming ratio
$\theta_{C}(h)$ on training data $C$ to be 0.1\%. 
Suppose on $C'$ we find $\theta_{C'}(h)$ to be 0.11\%.
Raising alarms would likely be false-positives.
However, if $\theta_{C'}(h)$ is substantially higher, say at 
5\%, intuitively it becomes an issue
that we should report. (The special
case where no value in $C'$ matches $h$
has the extreme $\theta_{C'}(h)=$ 100\%).

To reason about it formally, we 
model the process of drawing a conforming value
vs. a non-conforming value in
$C$ and $C'$, as sampling from two binomial distributions.
We then perform a form of statistical hypothesis test called 
\textit{two-sample homogeneity test},
to determine whether the fraction of non-conforming values
has changed significantly,
using $\theta_{C}(h)$, $\theta_{C'}(h)$,
and their respective sample sizes $|C|$ and $|C'|$.

Here, the null-hypothesis $H_0$ states that the
two underlying binomial distributions are the same;
whereas $H_1$ states that the reverse is true. 
We use \textit{Fischer's exact test}~\cite{agresti1992survey}
and \textit{Pearson's Chi-Squared test}~\cite{kanji2006} with
Yates correction for this purpose, both of which are suitable tests
in this setting.
We report $C'$ as an issue if the divergence from $C$ 
is so strong such that the null hypothesis can be rejected
(e.g., $\theta_{C}(h) =$ 0.1\% and
$\theta_{C'}(h) =$ 5\%).



We omit details of these two
statistical tests in the interest of space. 
In practice we find both to perform well, with 
little difference in terms of validation quality.
%}%iftoggle
%{
\begin{comment}
We model the process of drawing a conforming value
vs. a non-conforming value in
$C$ and $C'$, as sampling from two binomial distributions.
We then perform a form of statistical hypothesis test called 
\textit{two-sample homogeneity test}, specifically using
\textit{Fischer's exact test}~\cite{agresti1992survey}
and \textit{Pearson's Chi-Squared test}~\cite{kanji2006} with
Yates correction. We report $C'$ as an issue if the divergence from $C$ 
is strong.
We omit details of these statistical tests in the interest of space. 
In practice we find both to perform well, with 
little difference in terms of quality in our experiments.
\end{comment}
%}% else iftoggle

\iftoggle{fullversion}{
\textbf{Time Complexity.}
Overall, the time complexity of the offline step is 
$\mathcal{O}(|\mathbf{T}| |\mathbf{P}(D)|)$,
which comes from scanning each column $D$ in
$\mathbf{T}$ and enumerating its possible patterns. 
Recall that because we use vertical-cuts to handle
composite domains, $\mathbf{P}(D)$ can be constrained 
by the chosen constant $\tau$ that is the upper-limit
of token-count considered in the indexing step (described
in Section~\ref{sec:architecture}), without affecting result
quality because at online inference time we compose domains
using vertical-cuts
(Section~\ref{sec:vertical-cuts}).
%effectively by limiting the max number of tokens in $D$ 
%(e.g., limiting max token size to 13 produces would upper-bound
%$|\mathbf{P}(D)|$ to 500),
%yet vertical-cuts can still handle the complex patterns
%without loss of precision/recall.


In the online step, the complexity of the most involved
FMDV-VH variant is $\mathcal{O}(|\mathbf{P}(v)| |C| t(C)^2)$,
where $t(C)$ is the max number of tokens in query column $C$.
Empirically we find the overall latency to be less than 100ms on average,
as we will report in our experiments.
}


%https://en.wikipedia.org/wiki/Binomial_proportion_confidence_interval
%Based on the Central Limit Theorem,
%we reject $H_0$ if 
%\begin{equation}
%\label{eqn:hypothesis-test}
%\theta_{C'}(h) > \theta_{C}(h) + z \sqrt{\frac{\theta_{C}(h) (1 - \theta_{C}(h)) }{|C|}}
%\end{equation}
%We use $z_{0.05}$ = 1.96  for a 95\% confidence interval,
%and consider the validation to fail if 
%the null-hypothesis is rejected. 

%Many statistical tests are possible here
%(e.g., Chi-Squared and Fisher's tests)










==> paper - arxiv-full-version/auto-validate-vertical.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Auto-Validate (Vertical Cuts)}
\label{sec:vertical-cuts}

So far we only discussed the basic-version of
\sj. We now describe formulations that handle
more complex and real situations: (1) \textit{composite} structures
in query columns (this section); 
and (2) ``dirty'' values in query columns that violate
the homogeneity assumption (Section~\ref{sec:horizontal-cuts}).



Figure~\ref{fig:example-split} shows a real
column with composite structures 
that are concatenated from \textit{atomic domains}. Intuitively, 
we can see that it consists of at least 4
``sub-domains'', a floating-number (``\val{0.1}''),
followed by two time-stamps, 
followed by a status message (``\val{OnBooking}'').
We observe that such columns are common
in machine-generated data, where 
many are complex with over 10 sub-domains.


Such complex columns pose both quality and
scalability challenges. In terms of quality,
if we were to directly test complex
patterns against $\mathbf{T}$ like in FMDV, we may not be
able to see many exact matches in $\mathbf{T}$, 
because the complex patterns in $C$ may be concatenated 
in ad-hoc ways and are
sparsely represented in $\mathbf{T}$.
As a result, we may fail to find a
feasible solution to FMDV, 
because of the coverage requirement in 
Equation~\eqref{eqn:fmdv_cov}.

The second challenge is scalability.
As column $C$ become ``wider'' with
more tokens/segments, the space of possible patterns $\mathbf{P}(C)$
 that we will have to enumerate
grows exponentially in the number of tokens.
This is an issue both at online query time
for query column $C$, as well as
at offline indexing time to enumerate 
$\mathbf{P}(D)$ for data column $D \in \mathbf{T}$ --
recall that the date-time example in 
Figure~\ref{fig:generalization} already produces
over 3 billion patterns;  for the column in
Figure~\ref{fig:example-split} the
space of patterns is simply impractically large to enumerate. 
In the offline indexing step in Section~\ref{sec:architecture},
we discussed that we intentionally omit wide columns with
more than $\tau$ tokens to make pattern enumeration
tractable. We will show here that our
horizontal-cut algorithm
can ``compensate'' such omission without affecting result quality.


A natural approach to complex query column $C$
is to vertically ``cut'' it into
sub-columns (like shown in  
Figure~\ref{fig:example-split}). Patterns for
each sub-column can then be generated in turn using FMDV.
The benefit of this divide-and-conquer
approach is that each sub-domain
is likely well-represented in $\mathbf{T}$,
allowing them to be reliably inferred from $\mathbf{T}$.
Furthermore, the cost of pattern-enumeration in offline-indexing 
becomes significantly smaller, as each sub-domain can be enumerated
separately.


Specifically, we first use a lexer to tokenize each $v \in C$
into coarse-grained token-class (\val{<symbol>}, 
\val{<num>}, \val{<letter>}), by scanning each $v$
from left to right and ``growing'' each token until 
a character of a different class is encountered. 
In the example of Figure~\ref{fig:example-split},
for each row, we would generate an identical token-sequence
``\val{[<num>|<num>/<num>/<num> <num>:<num>:<num>|} \ldots \val{|<letter>]}''.

We then perform multi-sequence alignment 
(MSA)~\cite{carrillo1988multiple}
for all token sequences, before actually performing vertical-cuts.
Recall that the goal of MSA is to find optimal 
alignment across all input sequences 
(using objective functions such as 
sum-of-pair scores~\cite{just2001computational}).
Since MSA is NP-hard in 
general~\cite{just2001computational}, we follow
a standard approach to greedily align one additional sequence at a time.
We note that for homogeneous machine-generated 
data, this often solves MSA optimally.


\begin{example}
\label{ex:align}
For the column in Figure~\ref{fig:example-split},
each value $v \in C$ has an identical token-sequence
with 29 tokens:
``\val{[<num>|<num>/<num>/<num> 
<num>:<num>:<num>|} \ldots \val{|<letter>]}'', and
the aligned sequence using MSA can be
produced trivially as just a sequence with these 29 tokens (no gaps).
\end{example}




After alignment, characters in each $v \in C$ would map to
the aligned sequence of length $n$
(e.g., ``\val{0.1}'' maps to the first \val{<num>} in the aligned
token sequence,
``\val{02}'' maps to the second \val{<num>}, etc.).
%we produce a sequence of tokens $S_i$ of same length $n$,
%written as $S_i = [t^i_1, t^i_2, \ldots, t^i_n]$, where each $t^i_j$ is
%a token at the $j$-th position of value $v_i$.
Recall that our goal is to vertically split the $n$ tokens 
into $m$ segments so that values mapped to
each segment would correspond to a sub-domain as determined by FMDV.
We define an $m$-segmentation of $C$ as follows.

\begin{definition}
\label{def:segmentation}
Given a column $C$ with $n$ aligned tokens,
define $C[s, e]$ as a segment of $C$ that starts from token position 
$s$ and ends at position $e$, with $s, e \in [n]$.
An $m$-segmentation of $C$, 
is a list of $m$ such segments that
collectively cover $C$, defined as:
$(C[s_1, e_1], C[s_2, e_2],$ $\ldots$ $C[s_m, e_m])$,
where $s_1 = 1, e_m = n$, and $s_{i+1} = e_i + 1~\forall i \in [m]$.
We write $C[s_i, e_i]$ as $C_i$ for short,
and an $m$-segmentation as 
$(C_i : i \in [m])$ for short. 
\end{definition}


Note that each $C_i$ can be seen just like a regular column
``cut'' from the original $C$, with which we can invoke 
the FMDV.
Our overall objective is to jointly find: (1) an $m$-segmentation 
$(C_i : i \in [m])$
from all possible segmentation, denoted by $\mathbf{S}(C)$;
and  (2) furthermore find appropriate patterns 
$h_i \in \mathbf{H}(C_i)$ for each segment
$C_i$, such that the entire $C$ can be validated with a low
expected FPR. Also note that because we limit pattern enumeration
in offline-indexing to columns of at most $\tau$ tokens,
we would not find candidate patterns longer than $\tau$ in offline-index,
and can thus naturally limit the span of each segment to at most $\tau$
($e_i - s_i < \tau$, $\forall i$).
We can write this as an optimization problem FMDV-V defined as follows:




%\small
\begin{align}
 \text{(FMDV-V)}~ \min_{\substack{ h_1 \dots h_m \\ h_i \in \mathbf{H}(C_i) \\ (C_i: i \in [m]) \in \mathbf{S}(C)}}~~~& \sum_{h_i} \text{FPR}_\mathbf{T}(h_i)   \label{eqn:fmdvv_obj} \\ 
 \mbox{s.t.} ~~
% & (h_1, h_2, \ldots, h_n) \in \mathbf{H}(C) \label{eqn:fmdvv_concat} \\
& \sum_{h_i} \text{FPR}_\mathbf{T}(h_i) \leq r \label{eqn:fmdvv_fpr} \\
 & \text{Cov}_\mathbf{T}(h_i) \geq m,~\forall h_i \label{eqn:fmdvv_cov}
\end{align}
%\normalsize

In FMDV-V, we are optimizing over all possible segmentation
$(C_i : i \in [m]) \in \mathbf{S}(C)$, and for each $C_i$
all possible hypothesis patterns $h_i \in \mathbf{H}(C_i)$.
Our objective in Equation~\eqref{eqn:fmdvv_obj} is 
to minimize the sum of 
$\text{FPR}_\mathbf{T}(h_i)$ for all $h_i$.
We should note that this corresponds to a ``pessimistic'' 
approach that assumes non-conforming rows 
of each $h_i$ are disjoint at a row-level, thus needing
to sum them up in the objective function.
(An alternative could ``optimistically'' assume
non-conforming values in different segments 
to overlap at a row-level, in which case
we can use \textit{max} in place of the \textit{sum}.
We find this to be less effective and omit details in the interest of space).

%The FPR and coverage requirements in Equation~\eqref{eqn:fmdvv_fpr}
%and~\eqref{eqn:fmdvv_cov} are similar to their counterparts in FMDV.


We can show that the minimum FRP scores of 
$m$-segmentation optimized in Equation~\eqref{eqn:fmdvv_obj} have 
\textit{optimal substructure}~\cite{cormen2009introduction}, which makes
it amenable to dynamic programming (without exhaustive
enumeration). Specifically, 
we can show that the following holds:

%\scriptsize
\begin{equation}
%\vspace{-2mm}
\label{eqn:substructure}
\begin{split}
\text{minFRP}&(C[s, e])  = \\ \min \bigg(&  \min_{h \in \mathbf{P}(C[s, e])} \text{FPR}_{\mathbf{T}}(h), \\ 
&  \min_{t \in[s, e-1]}{\Big( \text{minFPR}(C[s, t]) + \text{minFPR}(C[t+1, e]) \Big)}\bigg)
\end{split}
\end{equation}
%\normalsize

Here, minFRP$(C[s, e])$ is the minimum FRP score with
vertical splits as optimized in 
Equation~\eqref{eqn:fmdvv_obj}, for a sub-column
corresponding to the segment
$C[s, e]$ from token-position $s$ to $e$.
Note that $C[1, n]$ corresponds to the original query column $C$,
and minFRP$(C[1, n])$ is the score we want to optimize.
Equation~\eqref{eqn:substructure} shows how this
can be computed incrementally.
Specifically, minFRP$(C[s, e])$ is the minimum of
(1) $\min_{h \in \mathbf{P}(C[s, e])}\text{FPR}_{\mathbf{T}}(h)$,
which is the FRP score 
of treating $C[s, e]$ as one column (with no splits), solvable
using FMDV;
and (2) $\min_{ t \in [s, e-1]}{\big( \text{minFPR}(C[s, t]) + \text{minFPR}(C[t+1, e]) \big)}$, which is the best minFRP scores from 
all possible two-way splits that
can be solved optimally in polynomial time using bottom-up 
dynamic-programming.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.45\textwidth]{figures/example-split.png}
\caption{Example columns with composite domains.}
\label{fig:example-split}
\end{figure}

%\rev made into full version in revision, bring back after
%\iftoggle{fullversion}{
\begin{example}
\label{ex:fmdv-v}
Continue with Example~\ref{ex:align}.
The aligned sequence of column $C$ in Figure~\ref{fig:example-split}
has 29 tokens, corresponding to $C[1, 29]$. 
The sub-sequence $C[4, 14]$ maps to identical
values ``\val{02/18/2015 00:00:00}'' for all rows, 
which can be seen as a ``sub-column'' split from $C$.

Using Equation~\eqref{eqn:substructure}, 
\text{minFRP}$(C[4, 14])$ of this sub-column 
can be computed as 
the minimum of:
(1) Not splitting of $C[4, 14]$, or
$\min_{h \in \mathbf{P}(C[4, 14])}\text{FPR}_{\mathbf{T}}(h)$,
computed using FMDV; and
(2) Further splitting $C[4, 14]$ into two parts, 
where the best score is computed as
$\min_{t \in[4, 13]}{\Big( \text{minFPR}(C[4, t]) + \text{minFPR}(C[t+1, 14]) \Big)}$, which can in turn be recursively computed.
Suppose we compute (1) to have FPR of 0.004\%, 
and the best of (2) to have FPR of 0.01\% (say, splitting 
into ``\val{02/18/2015}'' and ``\val{00:00:00}'').
Overall, not splitting $C[4, 14]$ is the best option.

Each such $C[s, e]$ can be computed bottom-up, until reaching
the top-level. %Specifically, the top-level
%\text{minFRP}(C[1, 29]) can be computed as 
%the minimum of:
%(1) Not splitting $C[1, 29]$: 
%or $\min_{h \in \mathbf{P}(C[1, 29])}\text{FPR}_{\mathbf{T}}(h)$
% computed from FMDV. 
%Because $C[1, 29]$ is sparsely represented in $\mathbf{T}$,
%in FMDV we could not find feasible solutions 
%meeting the coverage requirement. And
%(2) Splitting $C[1, 29]$: we find splitting along
%$C[1, 14]$ and $C[15, 29]$ to have the minimum FPR
%(which are in turn recursively split). 
The resulting split
minimizes the overall FPR and is the solution to FMDV-V.
\end{example}
%}%iftoggle


We would like to highlight that by using vertical-cuts, we can safely
ignore wide columns with more than $\tau$ tokens during offline
indexing (Section~\ref{sec:architecture}), without
affecting result quality. As a concrete example, 
when we encounter a column like
in Figure~\ref{fig:example-split}, brute-force enumeration would
generate at least $4^{29}$ patterns, which is impractically large
and thus omitted given a smaller token-length limit $\tau$ (e.g., 13) 
in offline indexing. However, when we encounter 
this column Figure~\ref{fig:example-split}
as a query column, we can still generate valid domain patterns
with the help of vertical-cuts (like shown in
Example~\ref{ex:fmdv-v}),
as long as each segment has at most
$\tau$ tokens. Vertical-cuts thus
greatly speed up offline-indexing as
well as online-inference, without affecting result quality.










==> paper - arxiv-full-version/auto-validate.bib.2 <==
% Encoding: windows-1252

@ARTICLE{abedjan2016,
  author = {Abedjan, Ziawasch and Chu, Xu and Deng, Dong and Fernandez, Raul
	Castro and Ilyas, Ihab F and Ouzzani, Mourad and Papotti, Paolo and
	Stonebraker, Michael and Tang, Nan},
  title = {Detecting Data Errors: Where are we and what needs to be done?},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@inproceedings{bogatu2020dataset,
  title={Dataset Discovery in Data Lakes},
  author={Bogatu, Alex and Fernandes, Alvaro AA and Paton, Norman W and Konstantinou, Nikolaos},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={709--720},
  year={2020},
  organization={IEEE}
}

@article{qahtan13pattern,
  title={Pattern Functional Dependencies for Data Cleaning},
  author={Qahtan, Abdulhakim and Tang, Nan and Ouzzani, Mourad and Cao, Yang and Stonebraker, Michael},
  journal={Proceedings of the VLDB Endowment},
  volume={13},
  number={5}
}

@article{padhi2018flashprofile,
  title={FlashProfile: a framework for synthesizing data profiles},
  author={Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov, Oleksandr and Gulwani, Sumit and Millstein, Todd},
  journal={Proceedings of the ACM on Programming Languages},
  volume={2},
  number={OOPSLA},
  pages={1--28},
  year={2018},
  publisher={ACM New York, NY, USA}
}



@inproceedings{qahtan2018fahes,
  title={FAHES: A robust disguised missing values detector},
  author={Qahtan, Abdulhakim A and Elmagarmid, Ahmed and Castro Fernandez, Raul and Ouzzani, Mourad and Tang, Nan},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2100--2109},
  year={2018}
}


@INPROCEEDINGS{abedjan2016dataxformer,
  author = {Abedjan, Ziawasch and Morcos, John and Ilyas, Ihab F and Ouzzani,
	Mourad and Papotti, Paolo and Stonebraker, Michael},
  title = {DataXFormer: A robust transformation discovery system},
  booktitle = {2016 IEEE 32nd International Conference on Data Engineering (ICDE)},
  year = {2016},
  pages = {1134--1145},
  organization = {IEEE}
}

@INPROCEEDINGS{abreu2014smelling,
  author = {Abreu, Rui and Cunha, J{\'a}come and Fernandes, Jo{\~a}o Paulo and
	Martins, Pedro and Perez, Alexandre and Saraiva, Jo{\~a}o},
  title = {Smelling faults in spreadsheets},
  booktitle = {Software Maintenance and Evolution (ICSME), 2014 IEEE International
	Conference on},
  year = {2014},
  organization = {IEEE}
}

@INPROCEEDINGS{afrati2009repair,
  author = {Afrati, Foto N and Kolaitis, Phokion G},
  title = {Repair checking in inconsistent databases: algorithms and complexity},
  booktitle = {Proceedings of the 12th International Conference on Database Theory},
  year = {2009},
  organization = {ACM}
}

@INPROCEEDINGS{arning1996linear,
  author = {Arning, Andreas and Agrawal, Rakesh and Raghavan, Prabhakar},
  title = {A Linear Method for Deviation Detection in Large Databases.},
  booktitle = {KDD},
  year = {1996}
}

@ARTICLE{arulselvan2014note,
  author = {Arulselvan, Ashwin},
  title = {A note on the set union knapsack problem},
  journal = {Discrete Applied Mathematics},
  year = {2014},
  volume = {169},
  publisher = {Elsevier}
}

@ARTICLE{asahiro2002complexity,
  author = {Asahiro, Yuichi and Hassin, Refael and Iwama, Kazuo},
  title = {Complexity of finding dense subgraphs},
  journal = {Discrete Applied Mathematics},
  year = {2002},
  volume = {121},
  pages = {15--26},
  number = {1-3},
  publisher = {Elsevier}
}

@ARTICLE{barron1998,
  author = {Barron, Andrew and Rissanen, Jorma and Yu, Bin},
  title = {The minimum description length principle in coding and modeling},
  journal = {IEEE Transactions on Information Theory},
  year = {1998},
  volume = {44},
  number = {6},
  publisher = {IEEE}
}

@INCOLLECTION{ben2005outlier,
  author = {Ben-Gal, Irad},
  title = {Outlier detection},
  booktitle = {Data mining and knowledge discovery handbook},
  publisher = {Springer},
  year = {2005}
}

@ARTICLE{bengio2003neural,
  author = {Bengio, Yoshua and Ducharme, R{\'e}jean and Vincent, Pascal and Jauvin,
	Christian},
  title = {A neural probabilistic language model},
  journal = {Journal of machine learning research},
  year = {2003},
  volume = {3},
  pages = {1137--1155},
  number = {Feb}
}

@ARTICLE{benjamini1995controlling,
  author = {Benjamini, Yoav and Hochberg, Yosef},
  title = {Controlling the false discovery rate: a practical and powerful approach
	to multiple testing},
  journal = {Journal of the Royal statistical society: series B (Methodological)},
  year = {1995}
}

@ARTICLE{berti2018discovery,
  author = {Berti-Equille, Laure and Harmouch, Hazar and Naumann, Felix and Novelli,
	No{\"e}l and Thirumuruganathan, Saravanan},
  title = {Discovery of genuine functional dependencies from relational data
	with missing values},
  journal = {VLDB},
  year = {2018}
}

@INPROCEEDINGS{bex2006,
  author = {Bex, Geert Jan and Neven, Frank and Schwentick, Thomas and Tuyls,
	Karl},
  title = {Inference of concise DTDs from XML data},
  booktitle = {VLDB},
  year = {2006}
}

@BOOK{biemann2011structure,
  title = {Structure discovery in natural language},
  publisher = {Springer Science \& Business Media},
  year = {2011},
  author = {Biemann, Chris and van den Bosch, Antal}
}

@INPROCEEDINGS{bohannon2005cost,
  author = {Bohannon, Philip and Fan, Wenfei and Flaster, Michael and Rastogi,
	Rajeev},
  title = {A cost-based model and effective heuristic for repairing constraints
	by value modification},
  booktitle = {Proceedings of the 2005 ACM SIGMOD international conference on Management
	of data},
  year = {2005},
  pages = {143--154},
  organization = {ACM}
}

@INPROCEEDINGS{bohannon2007,
  author = {Bohannon, Philip and Fan, Wenfei and Geerts, Floris and Jia, Xibei
	and Kementsietsidis, Anastasios},
  title = {Conditional functional dependencies for data cleaning},
  booktitle = {ICDE},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{breck2019data,
  author = {Breck, Eric and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven
	and Zinkevich, Martin},
  title = {Data Validation for Machine Learning},
  booktitle = {Conference on Systems and Machine Learning (SysML). https://www.
	sysml. cc/doc/2019/167. pdf},
  year = {2019}
}

@ARTICLE{brewer2012cap,
  author = {Brewer, Eric},
  title = {CAP Twelve years Later: how the},
  journal = {Computer},
  year = {2012},
  number = {2},
  publisher = {IEEE}
}

@ARTICLE{bruglieri2004cardinality,
  author = {Bruglieri, Maurizio and Maffioli, Francesco and Ehrgott, Matthias},
  title = {Cardinality constrained minimum cut problems: complexity and algorithms},
  journal = {Discrete Applied Mathematics},
  year = {2004},
  volume = {137},
  pages = {311--341},
  number = {3},
  publisher = {Elsevier}
}

@ARTICLE{cafarella2008,
  author = {Cafarella, Michael J and Halevy, Alon and Wang, Daisy Zhe and Wu,
	Eugene and Zhang, Yang},
  title = {Webtables: exploring the power of tables on the web},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{casellar,
  author = {Casella, George and Berger, Roger},
  title = {R. 2001, Statistical Inference},
  journal = {Duxbury Press}
}

@BOOK{casella2002statistical,
  title = {Statistical inference},
  publisher = {Duxbury Pacific Grove, CA},
  year = {2002},
  author = {Casella, George and Berger, Roger L},
  volume = {2}
}

@ARTICLE{webtables,
  author = {Chakrabarti, Kaushik and Chaudhuri, Surajit and Chen, Zhimin and
	Ganjam, Kris and He, Yeye and Redmond, WA},
  title = {Data services leveraging Bing's data assets.},
  journal = {IEEE Data Eng. Bull.},
  year = {2016},
  volume = {39},
  number = {3}
}

@ARTICLE{chandola2009anomaly,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Anomaly detection: A survey},
  journal = {ACM computing surveys (CSUR)},
  year = {2009},
  volume = {41},
  number = {3},
  publisher = {ACM}
}

@ARTICLE{chandola2007,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Outlier detection: A survey},
  journal = {ACM Computing Surveys},
  year = {2007}
}

@INPROCEEDINGS{chen1996empirical,
  author = {Chen, Stanley F and Goodman, Joshua},
  title = {An empirical study of smoothing techniques for language modeling},
  booktitle = {Proceedings of the 34th annual meeting on Association for Computational
	Linguistics},
  year = {1996},
  organization = {ACL}
}

@ARTICLE{chen2014fast,
  author = {Chen, Zhimin and Narasayya, Vivek and Chaudhuri, Surajit},
  title = {Fast foreign-key detection in Microsoft SQL server PowerPivot for
	Excel},
  journal = {Proceedings of the VLDB Endowment},
  year = {2014},
  volume = {7},
  pages = {1417--1428},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{cheung2016,
  author = {Cheung, Shing-Chi and Chen, Wanjun and Liu, Yepang and Xu, Chang},
  title = {CUSTODES: automatic spreadsheet cell clustering and smell detection
	using strong and weak features},
  booktitle = {Proceedings of the 38th International Conference on Software Engineering},
  year = {2016}
}

@ARTICLE{Chiang2008,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {Proceedings of the VLDB Endowment},
  year = {2008},
  volume = {1},
  pages = {1166--1177},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{chiang2008discovering,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2015tegra,
  author = {Chu, Xu and He, Yeye and Chakrabarti, Kaushik and Ganjam, Kris},
  title = {Tegra: Table extraction by global record alignment},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{chu2013,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{chu2013discovering,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2013holistic,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Holistic data cleaning: Putting violations into context},
  booktitle = {ICDE},
  year = {2013},
  organization = {IEEE}
}

@INPROCEEDINGS{chu2015,
  author = {Chu, Xu and Morcos, John and Ilyas, Ihab F and Ouzzani, Mourad and
	Papotti, Paolo and Tang, Nan and Ye, Yin},
  title = {Katara: A data cleaning system powered by knowledge bases and crowdsourcing},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{church1990word,
  author = {Church, Kenneth Ward and Hanks, Patrick},
  title = {Word association norms, mutual information, and lexicography},
  journal = {Computational linguistics},
  year = {1990},
  volume = {16},
  number = {1},
  publisher = {MIT Press}
}

@ARTICLE{clauset2009power,
  author = {Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, Mark EJ},
  title = {Power-law distributions in empirical data},
  journal = {SIAM review},
  year = {2009},
  volume = {51},
  number = {4},
  publisher = {SIAM}
}

@INPROCEEDINGS{collobert2008unified,
  author = {Collobert, Ronan and Weston, Jason},
  title = {A unified architecture for natural language processing: Deep neural
	networks with multitask learning},
  booktitle = {Proceedings of the 25th international conference on Machine learning},
  year = {2008},
  pages = {160--167},
  organization = {ACM}
}

@INPROCEEDINGS{cong2007,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {VLDB},
  year = {2007}
}

@INPROCEEDINGS{cong2007improving,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {Proceedings of the 33rd international conference on Very large data
	bases},
  year = {2007},
  pages = {315--326},
  organization = {VLDB Endowment}
}

@ARTICLE{cormode2005improved,
  author = {Cormode, Graham and Muthukrishnan, Shan},
  title = {An improved data stream summary: the count-min sketch and its applications},
  journal = {Journal of Algorithms},
  year = {2005},
  volume = {55},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{cormode2005summarizing,
  author = {Cormode, Graham and Muthukrishnan, S},
  title = {Summarizing and mining skewed data streams},
  booktitle = {Proceedings of the 2005 SIAM International Conference on Data Mining},
  year = {2005},
  organization = {SIAM}
}

@INPROCEEDINGS{dasu2002mining,
  author = {Dasu, Tamraparni and Johnson, Theodore and Muthukrishnan, Shanmugauelayut
	and Shkapenyuk, Vladislav},
  title = {Mining database structure; or, how to build a data quality browser},
  booktitle = {SIGMOD},
  year = {2002}
}

@INPROCEEDINGS{dayal2009data,
  author = {Dayal, Umeshwar and Castellanos, Malu and Simitsis, Alkis and Wilkinson,
	Kevin},
  title = {Data integration flows for business intelligence},
  booktitle = {Proceedings of the 12th International Conference on Extending Database
	Technology: Advances in Database Technology},
  year = {2009},
  pages = {1--11}
}

@INPROCEEDINGS{deng2017data,
  author = {Deng, Dong and Fernandez, Raul Castro and Abedjan, Ziawasch and Wang,
	Sibo and Stonebraker, Michael and Elmagarmid, Ahmed K and Ilyas,
	Ihab F and Madden, Samuel and Ouzzani, Mourad and Tang, Nan},
  title = {The Data Civilizer System.},
  booktitle = {Cidr},
  year = {2017}
}

@Misc{Enterprise2016,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@INPROCEEDINGS{fan2014,
  author = {Fan, Grace and Fan, Wenfei and Geerts, Floris},
  title = {Detecting errors in numeric attributes},
  booktitle = {International Conference on Web-Age Information Management},
  year = {2014},
  organization = {Springer}
}

@ARTICLE{fan2009reasoning,
  author = {Fan, Wenfei and Jia, Xibei and Li, Jianzhong and Ma, Shuai},
  title = {Reasoning about record matching rules},
  journal = {VLDB},
  year = {2009},
  volume = {2},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{fisher2005pads,
  author = {Fisher, Kathleen and Gruber, Robert},
  title = {PADS: a domain-specific language for processing ad hoc data},
  journal = {ACM Sigplan Notices},
  year = {2005},
  volume = {40},
  pages = {295--304},
  number = {6},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{fisher2008dirt,
  author = {Fisher, Kathleen and Walker, David and Zhu, Kenny Q and White, Peter},
  title = {From dirt to shovels: fully automatic tool generation from ad hoc
	data},
  journal = {ACM SIGPLAN Notices},
  year = {2008},
  volume = {43},
  pages = {421--434},
  number = {1},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{freeman1996make,
  author = {Freeman, David},
  title = {How to make spreadsheets error-proof},
  journal = {Journal of Accountancy},
  year = {1996},
  volume = {181},
  number = {5},
  publisher = {American Institute of Certified Public Accountants}
}

@INPROCEEDINGS{ganjisaffar2011qspell,
  author = {Ganjisaffar, Yasser and Zilio, Andrea and Javanmardi, Sara and Cetindil,
	Inci and Sikka, Manik and Katumalla, Sandeep and Khatib, Narges and
	Li, Chen and Lopes, Cristina},
  title = {qspell: Spelling correction of web search queries using ranking models
	and iterative correction},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{geerts2013llunatic,
  author = {Geerts, Floris and Mecca, Giansalvatore and Papotti, Paolo and Santoro,
	Donatello},
  title = {The LLUNATIC data-cleaning framework},
  journal = {Proceedings of the VLDB Endowment},
  year = {2013},
  volume = {6},
  pages = {625--636},
  number = {9},
  publisher = {VLDB Endowment}
}

@BOOK{gennick2010sql,
  title = {SQL Pocket Guide: A Guide to SQL Usage},
  publisher = {" O'Reilly Media, Inc."},
  year = {2010},
  author = {Gennick, Jonathan}
}

@ARTICLE{go2009twitter,
  author = {Go, Alec and Bhayani, Richa and Huang, Lei},
  title = {Twitter sentiment classification using distant supervision},
  journal = {CS224N Project Report, Stanford},
  year = {2009},
  volume = {1},
  number = {2009}
}

@ARTICLE{golab2010data,
  author = {Golab, Lukasz and Karloff, Howard and Korn, Flip and Srivastava,
	Divesh},
  title = {Data auditor: Exploring data quality and semantics using pattern
	tableaux},
  journal = {VLDB},
  year = {2010},
  volume = {3},
  number = {1-2},
  publisher = {VLDB Endowment}
}

@ARTICLE{goldschmidt1994polynomial,
  author = {Goldschmidt, Olivier and Hochbaum, Dorit S},
  title = {A polynomial algorithm for the k-cut problem for fixed k},
  journal = {Mathematics of operations research},
  year = {1994},
  volume = {19},
  pages = {24--37},
  number = {1},
  publisher = {INFORMS}
}

@ARTICLE{gulwani2012,
  author = {Gulwani, Sumit and Harris, William R and Singh, Rishabh},
  title = {Spreadsheet data manipulation using examples},
  journal = {Communications of the ACM},
  year = {2012},
  volume = {55},
  number = {8},
  publisher = {ACM}
}

@ARTICLE{gupta2014outlier,
  author = {Gupta, Manish and Gao, Jing and Aggarwal, Charu C and Han, Jiawei},
  title = {Outlier detection for temporal data: A survey},
  journal = {TKDE},
  year = {2014},
  volume = {26},
  number = {9},
  publisher = {IEEE}
}

@INPROCEEDINGS{halevy2016goods,
  author = {Halevy, Alon and Korn, Flip and Noy, Natalya F and Olston, Christopher
	and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong},
  title = {Goods: Organizing google's datasets},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{hall1992smoothed,
  author = {Hall, Peter and Marron, JS and Park, Byeong U},
  title = {Smoothed cross-validation},
  journal = {Probability theory and related fields},
  year = {1992},
  volume = {92},
  number = {1},
  publisher = {Springer}
}

@INPROCEEDINGS{harris2011spreadsheet,
  author = {Harris, William R and Gulwani, Sumit},
  title = {Spreadsheet table transformations from examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2011},
  volume = {46},
  number = {6},
  organization = {ACM}
}

@INPROCEEDINGS{he2016interactive,
  author = {He, Jian and Veltri, Enzo and Santoro, Donatello and Li, Guoliang
	and Mecca, Giansalvatore and Papotti, Paolo and Tang, Nan},
  title = {Interactive and deterministic data cleaning},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{he2018transform,
  author = {He, Yeye and Chu, Xu and Ganjam, Kris and Zheng, Yudian and Narasayya,
	Vivek and Chaudhuri, Surajit},
  title = {{Transform-data-by-example (TDE): an extensible search engine for
	data transformations}},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {10},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015sema,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2005,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  journal = {Advances in Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{he2005optimization,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  booktitle = {International Conference on Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{heer2015predictive,
  author = {Heer, Jeffrey and Hellerstein, Joseph M and Kandel, Sean},
  title = {Predictive Interaction for Data Transformation.},
  booktitle = {CIDR},
  year = {2015}
}

@ARTICLE{hellerstein2008,
  author = {Hellerstein, Joseph M},
  title = {Quantitative data cleaning for large databases},
  journal = {United Nations Economic Commission for Europe (UNECE)},
  year = {2008}
}

@INPROCEEDINGS{hochbaum,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@INPROCEEDINGS{hochbaum1996approximating,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@ARTICLE{hodge2004survey,
  author = {Hodge, Victoria and Austin, Jim},
  title = {A survey of outlier detection methodologies},
  journal = {Artificial intelligence review},
  year = {2004}
}

@INPROCEEDINGS{huang2018auto,
  author = {Huang, Zhipeng and He, Yeye},
  title = {{Auto-Detect: Data-Driven Error Detection in Tables}},
  booktitle = {SIGMOD},
  year = {2018}
}

@ARTICLE{huhtala1999tane,
  author = {Huhtala, Yka and K{\"a}rkk{\"a}inen, Juha and Porkka, Pasi and Toivonen,
	Hannu},
  title = {TANE: An efficient algorithm for discovering functional and approximate
	dependencies},
  journal = {The computer journal},
  year = {1999},
  volume = {42},
  number = {2},
  publisher = {OUP}
}

@BOOK{Ben-Gal05,
  title = {Data Mining and Knowledge Discovery Handbook: A Complete Guide for
	Practitioners and Researchers},
  publisher = {Kluwer Academic Publishers},
  year = {2005},
  author = {Ben-Gal I.},
  owner = {yeyehe},
  timestamp = {2018.10.02}
}

@INPROCEEDINGS{ilyas2018extracting,
  author = {Ilyas, Andrew and da Trindade, Joana MF and Fernandez, Raul Castro
	and Madden, Samuel},
  title = {Extracting syntactical patterns from databases},
  booktitle = {2018 IEEE 34th International Conference on Data Engineering (ICDE)},
  year = {2018},
  pages = {41--52},
  organization = {IEEE}
}

@INPROCEEDINGS{ilyas2004,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{ilyas2004cords,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{jin2017foofah,
  author = {Jin, Zhongjun and Anderson, Michael R and Cafarella, Michael and
	Jagadish, HV},
  title = {Foofah: Transforming data by example},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {683--698},
  organization = {ACM}
}

@INPROCEEDINGS{kandel2011wrangler,
  author = {Kandel, Sean and Paepcke, Andreas and Hellerstein, Joseph and Heer,
	Jeffrey},
  title = {Wrangler: Interactive visual specification of data transformation
	scripts},
  booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing
	Systems},
  year = {2011},
  pages = {3363--3372},
  organization = {ACM}
}

@ARTICLE{kazai2013analysis,
  author = {Kazai, Gabriella and Kamps, Jaap and Milic-Frayling, Natasa},
  title = {An analysis of human factors and label accuracy in crowdsourcing
	relevance judgments},
  journal = {Information retrieval},
  year = {2013},
  volume = {16},
  number = {2},
  publisher = {Springer}
}

@INPROCEEDINGS{keogh2004towards,
  author = {Keogh, Eamonn and Lonardi, Stefano and Ratanamahatana, Chotirat Ann},
  title = {Towards parameter-free data mining},
  booktitle = {SIGKDD},
  year = {2004}
}

@ARTICLE{khuller1999budgeted,
  author = {Khuller, Samir and Moss, Anna and Naor, Joseph Seffi},
  title = {The budgeted maximum coverage problem},
  journal = {Information Processing Letters},
  year = {1999},
  volume = {70},
  number = {1},
  publisher = {Elsevier}
}

@ARTICLE{kivinen1995approximate,
  author = {Kivinen, Jyrki and Mannila, Heikki},
  title = {Approximate inference of functional dependencies from relations},
  journal = {Theoretical Computer Science},
  year = {1995},
  volume = {149},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{knox1998algorithms,
  author = {Knox, Edwin M and Ng, Raymond T},
  title = {Algorithms for mining distance based outliers in large datasets},
  booktitle = {VLDB},
  year = {1998}
}

@TECHREPORT{BoostClean,
  author = {Sanjay Krishnan and Michael J. Franklin and Ken Goldberg and Eugene
	Wu},
  title = {BoostClean: Automated Error Detection and Repair for Machine Learning},
  year = {2017},
  owner = {yeye},
  timestamp = {2018.02.15}
}

@ARTICLE{krishnan2016activeclean,
  author = {Krishnan, Sanjay and Wang, Jiannan and Wu, Eugene and Franklin, Michael
	J and Goldberg, Ken},
  title = {ActiveClean: interactive data cleaning for statistical modeling},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{imagenet,
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  title = {Imagenet classification with deep convolutional neural networks},
  booktitle = {Advances in neural information processing systems},
  year = {2012}
}

@INPROCEEDINGS{Le2014,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  pages = {542--553},
  organization = {ACM}
}

@INPROCEEDINGS{le2014flashextract,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  organization = {ACM}
}

@BOOK{lee1997bayesian,
  title = {Bayesian statistics},
  publisher = {Arnold Publication},
  year = {1997},
  author = {Lee, Peter M}
}

@BOOK{lehmann2006testing,
  title = {Testing statistical hypotheses},
  publisher = {Springer Science \& Business Media},
  year = {2006},
  author = {Lehmann, Erich L and Romano, Joseph P}
}

@ARTICLE{leys2013detecting,
  author = {Leys, Christophe and Ley, Christophe and Klein, Olivier and Bernard,
	Philippe and Licata, Laurent},
  title = {Detecting outliers: Do not use standard deviation around the mean,
	use absolute deviation around the median},
  journal = {Journal of Experimental Social Psychology},
  year = {2013},
  volume = {49},
  number = {4},
  publisher = {Elsevier}
}

@INPROCEEDINGS{li2006exploring,
  author = {Li, Mu and Zhang, Yang and Zhu, Muhua and Zhou, Ming},
  title = {Exploring distributional similarity based models for query spelling
	correction},
  booktitle = {Proceedings of the 21st International Conference on Computational
	Linguistics and the 44th annual meeting of the Association for Computational
	Linguistics},
  year = {2006},
  organization = {ACL}
}

@INPROCEEDINGS{li2008regular,
  author = {Li, Yunyao and Krishnamurthy, Rajasekar and Raghavan, Sriram and
	Vaithyanathan, Shivakumar and Jagadish, HV},
  title = {Regular expression learning for information extraction},
  booktitle = {Proceedings of the Conference on Empirical Methods in Natural Language
	Processing},
  year = {2008},
  organization = {ACL}
}

@BOOK{lieberman2001your,
  title = {Your wish is my command: Programming by example},
  publisher = {Morgan Kaufmann},
  year = {2001},
  author = {Lieberman, Henry}
}

@ARTICLE{Forrester,
  author = {Cinny Little},
  title = {The Forrester Wave: Data Preparation Solutions, Q4 2018},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@ARTICLE{liu2009learning,
  author = {Liu, Tie-Yan and others},
  title = {Learning to rank for information retrieval},
  journal = {Foundations and Trends{\textregistered} in Information Retrieval},
  year = {2009},
  volume = {3},
  pages = {225--331},
  number = {3},
  publisher = {Now Publishers, Inc.}
}

@ARTICLE{lopes2002,
  author = {Lopes, St{\'e}phane and Petit, Jean-Marc and Lakhal, Lotfi},
  title = {Functional and approximate dependency mining: database and FCA points
	of view},
  journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
  year = {2002}
}

@INPROCEEDINGS{luec2011data,
  author = {Luec, Gord},
  title = {A data-driven approach for correcting search quaries},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{manning2008scoring,
  author = {Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  title = {Scoring, term weighting and the vector space model},
  journal = {Introduction to information retrieval},
  year = {2008},
  volume = {100},
  publisher = {Cambridge University Press}
}

@BOOK{pooling,
  title = {Evaluation in information retrieval, Stanford NLP Group, \url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparaGroup}},
  publisher = {Cambridge University Press},
  author = {Christopher D. Manning and Prabhakar Raghavan and Hinrich Schutze},
  owner = {yeyehe},
  timestamp = {2019.02.14},
  url = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}}
}

@ARTICLE{mariet2016outlier,
  author = {Mariet, Zelda and Harding, Rachael and Madden, Sam and others},
  title = {Outlier Detection in Heterogeneous Datasets using Automatic Tuple
	Expansion},
  journal = {MIT Technical Report},
  year = {2016}
}

@ARTICLE{Ziemann16,
  author = {Mark Ziemann, Yotam Eren and Assam El-Osta},
  title = {Gene name errors are widespread in the scientific literature},
  journal = {Genome Biology},
  year = {2016},
  owner = {yeyehe},
  timestamp = {2018.10.01}
}

@ARTICLE{maronna1976robust,
  author = {Maronna, Ricardo Antonio},
  title = {Robust M-estimators of multivariate location and scatter},
  journal = {The annals of statistics},
  year = {1976},
  publisher = {JSTOR}
}

@BOOK{maronna2018robust,
  title = {Robust Statistics: Theory and Methods (with R)},
  publisher = {Wiley},
  year = {2018},
  author = {Maronna, Ricardo A and Martin, R Douglas and Yohai, Victor J and
	Salibi{\'a}n-Barrera, Mat{\'\i}as}
}

@INPROCEEDINGS{differential-privacy,
  author = {McSherry, Frank and Talwar, Kunal},
  title = {Mechanism design via differential privacy},
  booktitle = {Foundations of Computer Science, 2007. FOCS'07. 48th Annual IEEE
	Symposium on},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{mikolov2010recurrent,
  author = {Mikolov, Tom{\'a}{\v{s}} and Karafi{\'a}t, Martin and Burget, Luk{\'a}{\v{s}}
	and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  title = {Recurrent neural network based language model},
  booktitle = {Eleventh annual conference of the international speech communication
	association},
  year = {2010}
}

@INPROCEEDINGS{word2vec,
  author = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg
	S and Dean, Jeff},
  title = {Distributed representations of words and phrases and their compositionality},
  booktitle = {Advances in neural information processing systems},
  year = {2013}
}

@INPROCEEDINGS{mintz2009distant,
  author = {Mintz, Mike and Bills, Steven and Snow, Rion and Jurafsky, Dan},
  title = {Distant supervision for relation extraction without labeled data},
  booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of
	the ACL and the 4th International Joint Conference on Natural Language
	Processing of the AFNLP: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@BOOK{neter1996applied,
  title = {Applied linear statistical models},
  publisher = {Irwin Chicago},
  year = {1996},
  author = {Neter, John and Kutner, Michael H and Nachtsheim, Christopher J and
	Wasserman, William},
  volume = {4}
}

@ARTICLE{Neyman33,
  author = {Neyman, J. and Pearson, E. S.},
  title = {On the problem of the most efficient tests of statistical hypotheses},
  journal = {Phil. Trans. R. Soc. Lond. A.},
  year = {1933}
}

@ARTICLE{padhi2017flashprofile,
  author = {Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov,
	Oleksandr and Gulwani, Sumit and Millstein, Todd D},
  title = {FlashProfile: Interactive Synthesis of Syntactic Profiles.},
  year = {2017}
}

@INPROCEEDINGS{pande2017effective,
  author = {Pande, Harshit},
  title = {Effective search space reduction for spell correction using character
	neural embeddings},
  booktitle = {Proceedings of the 15th Conference of the European Chapter of the
	ACL: Volume 2, Short Papers},
  year = {2017},
  volume = {2}
}

@INPROCEEDINGS{panko2008,
  author = {Panko, Raymond R},
  title = {Spreadsheet errors: What we know. what we think we can do},
  year = {2008},
  journal = {Symposium on Risk of Spreadsheets}
}

@ARTICLE{panko1998,
  author = {Panko, Raymond R},
  title = {What we know about spreadsheet errors},
  journal = {Journal of Organizational and End User Computing (JOEUC)},
  year = {1998}
}

@ARTICLE{papenbrock2015data,
  author = {Papenbrock, Thorsten and Bergmann, Tanja and Finke, Moritz and Zwiener,
	Jakob and Naumann, Felix},
  title = {Data profiling with metanome},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{parzen1962estimation,
  author = {Parzen, Emanuel},
  title = {On estimation of a probability density function and mode},
  journal = {The annals of mathematical statistics},
  year = {1962},
  volume = {33},
  number = {3},
  publisher = {JSTOR}
}

@INPROCEEDINGS{patel2019big,
  author = {Patel, Hiren and Jindal, Alekh and Szyperski, Clemens},
  title = {Big Data Processing at Microsoft: Hyper Scale, Massive Complexity,
	and Minimal Cost},
  booktitle = {Proceedings of the ACM Symposium on Cloud Computing},
  year = {2019},
  pages = {490--490}
}

@INPROCEEDINGS{polyzotis2017data,
  author = {Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong and Zinkevich,
	Martin},
  title = {Data management challenges in production machine learning},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {1723--1726}
}

@INPROCEEDINGS{powell2009,
  author = {Powell, Stephen G and Baker, Kenneth R and Lawson, Barry},
  title = {Errors in operational spreadsheets: A review of the state of the
	art},
  booktitle = {System Sciences, 2009. HICSS'09},
  year = {2009}
}

@INPROCEEDINGS{priedhorsky2007creating,
  author = {Priedhorsky, Reid and Chen, Jilin and Lam, Shyong Tony K and Panciera,
	Katherine and Terveen, Loren and Riedl, John},
  title = {Creating, destroying, and restoring value in Wikipedia},
  booktitle = {Proceedings of the 2007 international ACM conference on Supporting
	group work},
  year = {2007},
  organization = {ACM}
}

@INPROCEEDINGS{qahtan2018fahes,
  author = {Qahtan, Abdulhakim and Elmagarmid, Ahmed and Ouzzani, Mourad and
	Tang, Nan},
  title = {FAHES: Detecting disguised missing values},
  booktitle = {ICDE},
  year = {2018},
  organization = {IEEE}
}

@ARTICLE{rahman2018icarus,
  author = {Rahman, Protiva and Hebert, Courtney and Nandi, Arnab},
  title = {ICARUS: minimizing human effort in iterative data completion},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{squad,
  author = {Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang,
	Percy},
  title = {Squad: 100,000+ questions for machine comprehension of text},
  journal = {arXiv preprint arXiv:1606.05250},
  year = {2016}
}

@INPROCEEDINGS{raman2001potter,
  author = {Raman, Vijayshankar and Hellerstein, Joseph M},
  title = {Potter's wheel: An interactive data cleaning system},
  booktitle = {VLDB},
  year = {2001},
  volume = {1}
}

@ARTICLE{holoclean,
  author = {Rekatsinas, Theodoros and Chu, Xu and Ilyas, Ihab F and R{\'e}, Christopher},
  title = {Holoclean: Holistic data repairs with probabilistic inference},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {11},
  publisher = {VLDB Endowment}
}

@ARTICLE{rousseeuw1993alternatives,
  author = {Rousseeuw, Peter J and Croux, Christophe},
  title = {Alternatives to the median absolute deviation},
  journal = {Journal of the American Statistical association},
  year = {1993},
  volume = {88},
  number = {424},
  publisher = {Taylor \& Francis}
}

@BOOK{rozenberg2012handbook,
  title = {Handbook of Formal Languages: Volume 3 Beyond Words},
  publisher = {Springer Science \& Business Media},
  year = {2012},
  author = {Rozenberg, Grzegorz and Salomaa, Arto}
}

@BOOK{Schutze2008,
  title = {Introduction to information retrieval},
  publisher = {Cambridge University Press},
  year = {2008},
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  volume = {39}
}

@INPROCEEDINGS{schutze2008introduction,
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  title = {Introduction to information retrieval},
  booktitle = {Proceedings of the international communication of association for
	computing machinery conference},
  year = {2008},
  pages = {260}
}

@INPROCEEDINGS{schelter2019unit,
  author = {Schelter, Sebastian and Biessmann, Felix and Lange, Dustin and Rukat,
	Tammo and Schmidt, Phillipp and Seufert, Stephan and Brunelle, Pierre
	and Taptunov, Andrey},
  title = {Unit Testing Data with Deequ},
  booktitle = {Proceedings of the 2019 International Conference on Management of
	Data},
  year = {2019},
  pages = {1993--1996}
}

@INPROCEEDINGS{schelter2019differential,
  author = {Schelter, Sebastian and Grafberger, Stefan and Schmidt, Philipp and
	Rukat, Tammo and Kiessling, Mario and Taptunov, Andrey and Biessmann,
	Felix and Lange, Dustin},
  title = {Differential Data Quality Verification on Partitioned Data},
  booktitle = {2019 IEEE 35th International Conference on Data Engineering (ICDE)},
  year = {2019},
  pages = {1940--1945},
  organization = {IEEE}
}

@ARTICLE{schelter2018automating,
  author = {Schelter, Sebastian and Lange, Dustin and Schmidt, Philipp and Celikel,
	Meltem and Biessmann, Felix and Grafberger, Andreas},
  title = {Automating large-scale data quality verification},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {1781--1794},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{shachaf2010beyond,
  author = {Shachaf, Pnina and Hara, Noriko},
  title = {Beyond vandalism: Wikipedia trolls},
  journal = {Journal of Information Science},
  year = {2010},
  volume = {36},
  number = {3},
  publisher = {Sage Publications Sage UK: London, England}
}

@inproceedings{swami2020data,
  title={Data Sentinel: A Declarative Production-Scale Data Validation Platform},
  author={Swami, Arun and Vasudevan, Sriram and Huyn, Joojay},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={1579--1590},
  year={2020},
  organization={IEEE}
}


@ARTICLE{singh2016blinkfill,
  author = {Singh, Rishabh},
  title = {Blinkfill: Semi-supervised programming by example for syntactic string
	transformations},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {10},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{singh2016transforming,
  author = {Singh, Rishabh and Gulwani, Sumit},
  title = {Transforming spreadsheet data types using examples},
  booktitle = {Acm Sigplan Notices},
  year = {2016}
}

@ARTICLE{singhmelford,
  author = {Singh, Rishabh and Livshits, Benjamin and Zorn, Benjamin},
  title = {Melford: Using Neural Networks to Find Spreadsheet Errors},
  journal = {MSR technical report}
}

@ARTICLE{stoer1997simple,
  author = {Stoer, Mechthild and Wagner, Frank},
  title = {A simple min-cut algorithm},
  journal = {Journal of the ACM (JACM)},
  year = {1997},
  volume = {44},
  pages = {585--591},
  number = {4},
  publisher = {ACM}
}

@INPROCEEDINGS{surdeanu2010simple,
  author = {Surdeanu, Mihai and McClosky, David and Tibshirani, Julie and Bauer,
	John and Chang, Angel X and Spitkovsky, Valentin I and Manning, Christopher
	D},
  title = {A Simple Distant Supervision Approach for the TAC-KBP Slot Filling
	Task.},
  booktitle = {TAC},
  year = {2010}
}

@ARTICLE{tax2004support,
  author = {Tax, David MJ and Duin, Robert PW},
  title = {Support vector data description},
  journal = {Machine learning},
  year = {2004},
  volume = {54},
  number = {1},
  publisher = {Springer}
}

@BOOK{voorhees2005trec,
  title = {TREC: Experiment and evaluation in information retrieval},
  publisher = {MIT press Cambridge},
  year = {2005},
  author = {Voorhees, Ellen M and Harman, Donna K and others},
  volume = {1}
}

@INPROCEEDINGS{wang2017,
  author = {Wang, Yue and He, Yeye},
  title = {Synthesizing mapping relationships using table corpus},
  booktitle = {SIGMOD},
  year = {2017}
}

@INPROCEEDINGS{whitelaw2009using,
  author = {Whitelaw, Casey and Hutchinson, Ben and Chung, Grace Y and Ellis,
	Gerard},
  title = {Using the web for language independent spellchecking and autocorrection},
  booktitle = {Proceedings of the 2009 Conference on Empirical Methods in Natural
	Language Processing: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@ARTICLE{yaghmazadeh2018automated,
  author = {Yaghmazadeh, Navid and Wang, Xinyu and Dillig, Isil},
  title = {Automated migration of hierarchical data to relational tables using
	programming-by-example},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {580--593},
  number = {5},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{yakout2013don,
  author = {Yakout, Mohamed and Berti-{\'E}quille, Laure and Elmagarmid, Ahmed
	K},
  title = {Don't be SCAREd: use SCalable Automatic REpairing with maximal likelihood
	and bounded changes},
  booktitle = {SIGMOD},
  year = {2013}
}

@INPROCEEDINGS{yan18,
  author = {Cong Yan and Yeye He},
  title = {Synthesizing Type-Detection Logic using Open-source Code},
  booktitle = {SIGMOD},
  year = {2018},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@INPROCEEDINGS{yan2018synthesizing,
  author = {Yan, Cong and He, Yeye},
  title = {{Auto-Type: Synthesizing type-detection logic for rich semantic data
	types using open-source code}},
  booktitle = {Proceedings of the 2018 International Conference on Management of
	Data},
  year = {2018},
  organization = {ACM}
}

@INPROCEEDINGS{yu2011,
  author = {Yu, Yang and Heflin, Jeff},
  title = {Extending functional dependency to detect abnormal data in RDF graphs},
  booktitle = {International Semantic Web Conference},
  year = {2011},
  organization = {Springer}
}

@INPROCEEDINGS{zhai2017study,
  author = {Zhai, Chengxiang and Lafferty, John},
  title = {A study of smoothing methods for language models applied to ad hoc
	information retrieval},
  booktitle = {ACM SIGIR Forum},
  year = {2017},
  organization = {ACM}
}

@INPROCEEDINGS{auto-em,
  author = {Chen Zhao and Yeye He},
  title = {{Auto-EM: End-to-end Fuzzy Entity-Matching using Pre-trained Deep
	Models and Transfer Learning}},
  booktitle = {WWW},
  year = {2019}
}

@INPROCEEDINGS{zhao2017controlling,
  author = {Zhao, Zheguang and De Stefani, Lorenzo and Zgraggen, Emanuel and
	Binnig, Carsten and Upfal, Eli and Kraska, Tim},
  title = {Controlling false discoveries during interactive data exploration},
  booktitle = {SIGMOD},
  year = {2017}
}

@ARTICLE{zhou2012scope,
  author = {Zhou, Jingren and Bruno, Nicolas and Wu, Ming-Chuan and Larson, Per-Ake
	and Chaiken, Ronnie and Shakib, Darren},
  title = {SCOPE: parallel databases meet MapReduce},
  journal = {The VLDB Journal},
  year = {2012},
  volume = {21},
  pages = {611--636},
  number = {5},
  publisher = {Springer}
}

@ARTICLE{zhu2017auto,
  author = {Zhu, Erkang and He, Yeye and Chaudhuri, Surajit},
  title = {Auto-join: Joining tables by leveraging transformations},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {10},
  publisher = {VLDB Endowment}
}



@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://www.nuget.org/packages/Microsoft.ProgramSynthesis.Extraction.Text/}}
}


@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/transform-model/service-dataflows-create-use}}
}

@MISC{tableau-flow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://help.tableau.com/current/prep/en-us/prep_build_flow.htm}}
}

@MISC{amazon-workflow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://aws.amazon.com/blogs/big-data/simplify-data-pipelines-with-aws-glue-automatic-code-generation-and-workflows/}}
}

@MISC{azureml-pipelines,
  title = {{Azure ML: Data Pipelines}},
  howpublished = {\url{https://docs.microsoft.com/en-us/azure/machine-learning/concept-ml-pipelines}}
}

@MISC{ataccama,
  title = {{ataccama: Data Profiling}},
  howpublished = {\url{https://www.ataccama.com/product/data-discovery-and-profiling}}
}

@MISC{Kaggle-Dropbox,
  title = {{Kaggle Expeirment, Shared via Dropbox}},
  howpublished = {\url{https://www.dropbox.com/sh/cfyv5lhzcpiv1xk/AAC5SIKCjuZZL5n5_RKHzMBwa?dl=0}}
}

@article{chaiken2008scope,
  title={SCOPE: easy and efficient parallel processing of massive data sets},
  author={Chaiken, Ronnie and Jenkins, Bob and Larson, Per-{\AA}ke and Ramsey, Bill and Shakib, Darren and Weaver, Simon and Zhou, Jingren},
  journal={Proceedings of the VLDB Endowment},
  volume={1},
  number={2},
  pages={1265--1276},
  year={2008},
  publisher={VLDB Endowment}
}


@incollection{vassiliadis2009near,
  title={Near real time ETL},
  author={Vassiliadis, Panos and Simitsis, Alkis},
  booktitle={New trends in data warehousing and data analysis},
  pages={1--31},
  year={2009},
  publisher={Springer}
}



@MISC{xgboost,
  title = {{XGBoost}},
  howpublished = {\url{https://xgboost.readthedocs.io/en/latest/}}
}



@MISC{BingEntity,
  title = {Bing Entity Search},
  howpublished = {\url{https://azure.microsoft.com/en-us/services/cognitive-services/bing-entity-search-api/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Deequ,
  title = {{Amazon Deequ Library for Data Validation}},
  howpublished = {\url{https://github.com/awslabs/deequ}}
}

@MISC{DresdenTables,
  title = {{Dresden Web Table Corpus}},
  howpublished = {\url{https://wwwdb.inf.tu-dresden.de/misc/dwtc/}}
}

@MISC{eusprig,
  title = {Spreadsheet mistakes - news stories, compiled by European Spreadsheet
	Risk Interest Group {EuSpRiG}},
  howpublished = {\url{http://www.eusprig.org/horror-stories.htm}},
  owner = {yeyehe},
  timestamp = {2017.09.26}
}

@MISC{frameapi,
  title = {Pandas Data Frame List of APIs},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/frame.html}}
}

@MISC{gartner,
  title = {Self-Service Data Preparation, Worldwide, 2016},
  howpublished = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}},
  owner = {yeyehe},
  timestamp = {2017.03.07}
}

@ARTICLE{gartner17,
  title = {Market Guide for Data Preparation - Gartner, 2017},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@MISC{GitHubv3,
  title = {GitHub API},
  howpublished = {\url{https://developer.github.com/v3/}},
  owner = {yeyehe},
  timestamp = {2019.10.21}
}

@MISC{googlewebtables,
  title = {{Google Web Tables}},
  howpublished = {\url{http://research.google.com/tables}}
}

@MISC{groupbyapi,
  title = {Pandas Groupby Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.groupby.html}}
}

@MISC{Informatica,
  title = {{Informatica Rev}},
  howpublished = {\url{https://www.informatica.com/products/data-quality/rev.html}},
  owner = {yeyehe},
  timestamp = {2016.10.21}
}

@Misc{Informatica-DQ-rules,
  title        = {{Informatica Data Quality Rules (Retrieved in 2020-02)}},
  howpublished = {\url{https://www.informatica.com/content/dam/informatica-com/en/collateral/data-sheet/en_informatica-data-quality_data-sheet_6710.pdf}},
}

@MISC{jsonapi,
  title = {Pandas Json Normalize Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.io.json.json_normalize.html}}
}

@MISC{Jupyter,
  title = {Jupyter Notebooks},
  howpublished = {\url{https://jupyter.org/}}
}

@MISC{kaggle,
  title = {Kaggle},
  howpublished = {\url{https://www.kaggle.com/}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{kaggle-dataset,
  title = {Kaggle Dataset API},
  howpublished = {\url{https://www.kaggle.com/docs/api}{interacting-with-datasets}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{meltapi,
  title = {Pandas Melt Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.melt.html}}
}

@MISC{mergeapi,
  title = {Pandas Merge Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.merge.html}}
}

@MISC{OpenRefine,
  title = {{OpenRefine (formerly Google Refine)}},
  howpublished = {\url{http://openrefine.org/}}
}

@MISC{paxata,
  title = {Paxata data preparation},
  howpublished = {\url{https://www.paxata.com/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{pivotapi,
  title = {Pandas Pivot Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.pivot_table.html}}
}

@MISC{PowerBI,
  title = {Power BI},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/desktop-data-types}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{python-trace,
  title = {{python tracing library}},
  howpublished = {\url{https://pymotw.com/2/trace/}}
}

@MISC{ssis-profiling,
  title = {{SSIS: Data Profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}}
}

@MISC{TableauPrep,
  title = {Tableau Prep},
  howpublished = {\url{https://www.tableau.com/products/prep}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Talend,
  title = {Talend data validation},
  howpublished = {\url{https://www.talendbyexample.com/talend-data-validation.html}},
  owner = {yeyehe},
  timestamp = {2017.09.28}
}

@MISC{TalendSemantic,
  title = {Talend Data Services Platform Studio User Guide: Semantic Discovery},
  howpublished = {\url{https://help.talend.com/reader/nAXiZW0j0H~2~YApZIsRFw/_u0D0oqWxesgBDSihDgbYA}},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@MISC{TFDV,
  title = {{Google TensorFlow Data Validation}},
  howpublished = {\url{https://www.tensorflow.org/tfx/guide/tfdv}}
}

@MISC{Trifacta,
  title = {Trifacta},
  howpublished = {\url{https://www.trifacta.com/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{trifacta-profiling,
  title = {{Trifacta: Data Profiling}},
  howpublished = {\url{https://www.trifacta.com/data-profiling/}}
}

@MISC{WebDataCommonsTables,
  title = {{Web Table Corpora from Web Data Commons}},
  howpublished = {\url{http://webdatacommons.org/webtables/}}
}

@MISC{wiktionary,
  title = {Excel error checking rules},
  howpublished = {\url{https://www.wiktionary.org/}},
  owner = {yeyehe},
  timestamp = {2017.09.27}
}

@MISC{word2vec-demo,
  title = {Word embedding demo},
  howpublished = {\url{http://bionlp-www.utu.fi/wv_demo/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{word2vec-for-misspellings,
  title = {{Google's trained Word2Vec model }},
  howpublished = {\url{http://mccormickml.com/2016/04/12/googles-pretrained-word2vec-model-in-python/}}
}

@OTHER{,
  owner = {yeyehe},
  timestamp = {2020.03.02}
}

@Article{karp1985fast,
  author    = {Karp, Richard M and Wigderson, Avi},
  title     = {A fast parallel algorithm for the maximal independent set problem},
  journal   = {Journal of the ACM (JACM)},
  year      = {1985},
  volume    = {32},
  number    = {4},
  pages     = {762--773},
  publisher = {ACM New York, NY, USA},
}

@Article{wang1994complexity,
  author  = {Wang, Lusheng and Jiang, Tao},
  title   = {On the complexity of multiple sequence alignment},
  journal = {Journal of computational biology},
  year    = {1994},
  volume  = {1},
  number  = {4},
  pages   = {337--348},
}

@Article{carrillo1988multiple,
  author    = {Carrillo, Humberto and Lipman, David},
  title     = {The multiple sequence alignment problem in biology},
  journal   = {SIAM journal on applied mathematics},
  year      = {1988},
  volume    = {48},
  number    = {5},
  pages     = {1073--1082},
  publisher = {SIAM},
}

@Article{just2001computational,
  author    = {Just, Winfried},
  title     = {Computational complexity of multiple sequence alignment with SP-score},
  journal   = {Journal of computational biology},
  year      = {2001},
  volume    = {8},
  number    = {6},
  pages     = {615--623},
  publisher = {Mary Ann Liebert, Inc.},
}

@Book{cormen2009introduction,
  title     = {Introduction to algorithms},
  publisher = {MIT press},
  year      = {2009},
  author    = {Cormen, Thomas H and Leiserson, Charles E and Rivest, Ronald L and Stein, Clifford},
}

@Misc{enterprise2016trifacta,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@Misc{grok,
  title        = {{Grok Patterns}},
  howpublished = {\url{https://github.com/elastic/elasticsearch/blob/master/libs/grok/src/main/resources/patterns/grok-patterns}},
}

@Misc{,
  title        = {{SQL Server SSIS profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}},
}

@Misc{Glue,
  title        = {{AWS Glue custom classifers}},
  howpublished = {\url{https://docs.aws.amazon.com/glue/latest/dg/custom-classifier.html}},
}

@Misc{xsystem-code,
  title        = {{XSystem Code}},
  howpublished = {\url{https://bitbucket.org/andrewiilyas/xsystem-old/src/outlier-detection/}},
}

@Article{stonebraker2018data,
  author  = {Stonebraker, Michael and Ilyas, Ihab F},
  title   = {Data Integration: The Current Status and the Way Forward.},
  journal = {IEEE Data Eng. Bull.},
  year    = {2018},
  volume  = {41},
  number  = {2},
  pages   = {3--9},
}

@Book{kanji2006,
  title     = {100 statistical tests},
  publisher = {Sage},
  year      = {2006},
  author    = {Kanji, Gopal K},
}

@Article{agresti1992survey,
  author    = {Agresti, Alan and others},
  title     = {A survey of exact inference for contingency tables},
  journal   = {Statistical science},
  year      = {1992},
  volume    = {7},
  number    = {1},
  pages     = {131--153},
  publisher = {Institute of Mathematical Statistics},
}

@InProceedings{hynes2017data,
  author    = {Hynes, Nick and Sculley, D and Terry, Michael},
  title     = {The data linter: Lightweight, automated sanity checking for ml data sets},
  booktitle = {NIPS MLSys Workshop},
  year      = {2017},
}

@Article{naumann2014data,
  author    = {Naumann, Felix},
  title     = {Data profiling revisited},
  journal   = {ACM SIGMOD Record},
  year      = {2014},
  volume    = {42},
  number    = {4},
  pages     = {40--49},
  publisher = {ACM New York, NY, USA},
}

@Misc{msft-ml,
  title        = {{Microsoft ML pipelines}},
  howpublished = {\url{https://www.slideshare.net/KarthikMurugesan2/microsoft-ai-platform-aether-introduction}},
}

@Comment{jabref-meta: databaseType:bibtex;}


==> paper - arxiv-full-version/auto-validate.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Auto-Validate (Basic Version)}

We start by describing a basic-version of \sj{} for ease of illustration,
before going into more involved
algorithm variants that use vertical-cuts (Section~\ref{sec:vertical-cuts})
and horizontal-cuts  (Section~\ref{sec:horizontal-cuts}).

\vspace{-2mm}
\subsection{Preliminary: Pattern Language}
\label{sec:language}
Since we propose to validate data by patterns,
we first briefly describe the pattern language used. 
We note that this is fairly standard (e.g., similar to 
ones used in~\cite{raman2001potter}) 
and not the focus of this work.

Figure~\ref{fig:hierarchy} shows a generalization hierarchy 
used, where leaf-nodes represent the English alphabet, 
and intermediate nodes (e.g., 
\val{<digit>}, \val{<letter>}) represent \textit{tokens} that values
can generalize into. A pattern is simply a sequence 
of (leaf or intermediate) tokens,
and for a given value $v$, this hierarchy
induces a space of all patterns consistent with $v$, 
denoted by $\mathbf{P}(v)$.
For instance, for a value $v =$ ``\val{9:07}'', we can generate
$\mathbf{P}(v) = $ \{%\val{9:07}, 
%\val{<digit>:07}, 
%\val{9:<digit>\{2\}}, 
 ``\val{<digit>:<digit>\{2\}}'', 
 ``\val{<digit>+:<digit>\{2\}}'', 
 ``\val{<digit>:<digit>+}'', 
 ``\val{<num>:<digit>+}'',  ``\val{9:<digit>\{2\}}'', \ldots
\}, among many other options.


Given a column $C$ for which patterns need
to be generated, we define the 
space of \textit{hypothesis-patterns}, 
denoted by $\mathbf{H}(C)$, as the set of patterns 
consistent with all values  $v \in C$, or 
$\mathbf{H}(C) = \cap_{v \in C}{\mathbf{P}(v)} \setminus \text{``.*''}$ (note that we exclude the trivial ``.*'' pattern as it 
is trivially consistent with all $C$).
Here we make an implicit assumption that values in 
$C$ are homogeneous and drawn from the same domain, which is generally
true for \textit{machine-generated data} from production
pipelines (like shown in 
Figure~\ref{fig:domain-example})\footnote{Our empirical sample
in an enterprise data lake suggests that 87.9\% columns are 
homogeneous (defined as drawn from the same underlying
domain), and 67.6\% are homogeneous with
machine-generated patterns.}.
Note that the assumption is used to only simplify our discussion of 
the basic-version of \sj (this section), and will later be relaxed
in more advanced variants (Section~\ref{sec:horizontal-cuts}).




 We call $\mathbf{H}(C)$ hypothesis-patterns because as we will see, 
each $h(C) \in \mathbf{H}(C)$
will be tested like a ``hypothesis'' to determine if $h$ is a good
validation pattern.  
We use $h$ and $h(C)$
interchangeably when the context is clear. 
\begin{example}
\label{ex:patterns}
Given the column $C$ shown in Figure~\ref{fig:generalization},
and the hierarchy in Figure~\ref{fig:hierarchy}, the 
space of hypothesis patterns $\mathbf{H}(C)$ is shown 
at the top of  Figure~\ref{fig:generalization}.
\end{example}

We use an in-house implementation to produce patterns based
on the hierarchy, which can be considered
as a variant of well-known pattern-profiling
techniques like~\cite{raman2001potter}. Briefly,
our pattern-generation works in two steps. In the
first step, it scans each cell value and
emits \textit{coarse-grained} tokens 
(e.g., \val{<num>} and \val{<letter>+}), 
without specializing into 
\textit{fine-grained} tokens 
(e.g., \val{<digit>\{1\}} or \val{<letter>\{2\}}).
For each value in Figure~\ref{fig:generalization},
for instance, this produces the same 
\val{<num>/<num>/<num> <num>:<num>:<num> <letter>+}.
Each coarse-grained pattern is then checked for coverage
so that only patterns meeting a coverage threshold are retained. 
In the second step, each coarse-grained pattern is
specialized into fine-grained patterns (examples are shown in 
Figure~\ref{fig:generalization}), as long as the given
threshold is met. 
\iftoggle{fullversion}
{Pseudo-code of the procedure can be found in 
Algorithm~\ref{algo:pattern} below.}
{More details of this can be found in a 
full version of this paper~\cite{full}. %\todo{link}
}


\iftoggle{fullversion}
{
\begin{algorithm}
\SetAlgoLined
  \SetKwInOut{Input}{input}
  \SetKwInOut{Output}{output}
  \SetKwData{S}{$\mathcal{S}$}
  \SetKwData{P}{$\mathcal{P}$}
  \SetKwProg{GeneratePatterns}{GeneratePatterns}{}{}

  \GeneratePatterns{$(\S, H)$}{
  \Input{string values $\S = \{s_1, \dots, s_n\}$, generalization hierarchy $H$}
  \Output{patterns $\P_{fine}$ of $\S$ induced by $H$}
$\P_{coarse} \leftarrow \{\}$\;
\ForEach{$s \in \S$ }{
p $\leftarrow$ GenerateCoarsePatterns(s)\;
add p to $\P_{coarse}$
}
retain patterns in $\P_{coarse}$ with sufficient coverage\;
$\P_{fine} \leftarrow \{\}$\;
\ForEach{$p$ $\in$ $\P_{coarse}$}{
p' $\leftarrow$ drill-down each $p$ using $H$\;
add p' to $\P_{fine}$ if coverage is sufficient \;
}
   \KwRet{$\P_{fine}$}\;
}
\caption{Generate patterns from a column of values}\label{algo:pattern}
\end{algorithm}
}
{}

We emphasize that the
proposed \sj{} framework is not tied to specific 
choices of hierarchy/pattern-languages -- in fact, it is 
entirely orthogonal to such choices, as other variants of languages 
are equally applicable in this framework.


\vspace{-2mm}
\subsection{Intuition: Goodness of Patterns}
\label{sec:intuition}
The core challenge in  \sj{}, is to determine whether a pattern
$h(C) \in \mathbf{H}(C)$ is  suitable for data-validation.
Our idea here is to leverage a corpus of 
related tables $\mathbf{T}$ (e.g., drawn from the
same enterprise data lake, which stores input/output data
of all production pipelines). Intuitively, a pattern
$h(C) \in \mathbf{H}(C)$ is a ``good'' validation
pattern for $C$, if it accurately describes the underlying ``domain'' of $C$,
defined as the space of all valid data values.
Conversely, $h(C)$ is a ``bad'' validation pattern, if:
\begin{itemize}[leftmargin=*,topsep=0pt]
\item[](1) $h(C)$ does not capture all valid values in the underlying ``domain'' of $C$;
\item[](2) $h(C)$ does not produce sufficient matches in $\mathbf{T}$.
\end{itemize}

Both are intuitive requirements -- 
(1) is desirable, because as we discussed, the danger in data-validation is
to produce patterns 
that do not cover all valid values from the same domain, 
which leads to false alarms.
Requirement (2) is also sensible because we want to see sufficient
evidence in $\mathbf{T}$ 
before we can reliably 
declare a pattern $h(C)$ to be a common ``domain''
of interest (seeing a pattern once or twice is not sufficient).


We note that both of these two requirements can be reliably tested using 
$\mathbf{T}$ alone and without involving humans.
Testing (2) is straightforward using standard pattern-matches. 
Testing (1) is also feasible,
under the assumption that most data columns 
in $D \in \mathbf{T}$ contain homogeneous
values drawn from the same underlying 
domain, which is generally true for ``machine-generated'' data
from production pipelines.
(Homogeneity is less likely to hold on other types of data, e.g., data manually typed in by human operators).

We highlight the fact that
we are now dealing with two types of columns that
can be a bit confusing --
the first is the input column $C$ for which we need to
generate validation patterns $h$, and the second is 
columns $D \in \mathbf{T}$ from which we draw evidence 
to determine the goodness of $h$.
To avoid confusion,  we will follow the standard of referring
to the first as the \textit{query column}, denoted by $C$,
and the second as \textit{data columns}, denoted by $D$.


\begin{figure*}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/intuition.png}
\caption{Leverage corpus $\mathbf{T}$ to determine ``good'' vs. ``bad'' hypothesis patterns, for a given query column $C$.}
\vspace{-3mm}
\label{fig:intuition}
\end{figure*}


We now show how to test requirement (1) using $\mathbf{T}$ below.

\begin{example}
\label{ex:intuition} 
The left of
Figure~\ref{fig:intuition} shows a query column $C$ for which
validation patterns need to be generated. A few
hypothesis-patterns in $\mathbf{H}(C)$ are listed in
the middle. In this example, we intuitively know
that $h_1(C)$ and $h_2(C)$ are ``bad'' patterns
since they 
are too ``narrow'' and would lead to false-alarms,
while $h_5(C)$ is a ``good'' validation pattern
that suitably generalizes the underlying domain. 

We show that such determinations can 
be inferred using $\mathbf{T}$.
Specifically, $h_1(C)$ is a ``bad'' pattern based on $\mathbf{T}$,
because we can find many columns like $D \in \mathbf{T}$ 
shown on the right of Figure~\ref{fig:intuition}
that are ``impure'' -- these columns contain
values that match $h_1(C)$, as well as values that do not
(e.g., ``{\small \texttt{9/12/2019 12:01:32 PM}}'',
where the ``{\small \texttt{PM}}'' part does not match $h_1(C)$).
A large number of ``impure'' columns like this would
indicate that $h_1(C)$ is not a good pattern to describe 
the underlying domain because if it were, we should not see
many impure columns like $D \in \mathbf{T}$ given homogeneity.

Similarly, we can show that $h_2(C)$ is not a good validation pattern,
for using $h_2(C)$ to describe the 
domain would again make many columns like $D$ ``impure'' 
(values like ``\val{10:02:20 AM}'' are inconsistent
with $h_2(C)$ since they have two-digit hours, whereas
$h_2(C)$ uses a single \val{<digit>} for hours),
  suggesting $h_2(C)$ is also too narrow.

Using the ideal pattern $h_5(C)$ to describe the domain, 
on the other hand, would yield few
``impure'' columns in $\mathbf{T}$.
\end{example}



Intuitively, we can use the \textit{impurity} of pattern $h$ on
data columns $D \in \mathbf{T}$,
to infer whether $h$ is a good validation pattern
for the domain, defined as follows.
\begin{definition}
\label{def:impurity}
The \textit{impurity} of a data column 
$D \in \mathbf{T}$, relative to a given hypothesis pattern $h$,
is defined as:
\begin{equation}
\label{eqn:impurity}
\text{Imp}_{D}(h) = \frac{|\{v | v \in D, h \notin \mathbf{P}(v)\}|}{|\{ v | v \in D \}|}
\end{equation}
\end{definition}

This definition is intuitive -- we measure 
impurity as the fraction 
of values in $D$ not matching $h$.



\begin{example}
\label{ex:fpr}
In Figure~\ref{fig:intuition}, 
$\text{Imp}_D(h_1)$ can be calculated as $\frac{2}{12}$,
since the last 2 values (with ``\val{PM}'') 
out of 12 do not match $h_1$.

Similarly, $\text{Imp}_D(h_2)$ can be calculated as $\frac{8}{12}$,
since the last 8 values in $D$ (with two-digit hours) 
do not match $h_2$.

Finally, $\text{Imp}_D(h_5)$ is $\frac{0}{12}$,
since all values in $D$ match $h_5$.
\end{example}



We note that if $h(C)$ is used to validate
a data column $D$ (in the same domain as $C$)
arriving in the future, then 
Imp$_D(h)$ directly corresponds to
expected false-positive-rate (FPR):

\begin{definition}
\label{def:fpr}
The expected \textit{false-positive-rate} (FPR) of using pattern $h(C)$ 
to validate a data column $D$ drawn from the same domain as $C$,
denoted by $\text{FPR}_{D}(h)$, is defined as:
\begin{equation}
\label{f}
\text{FPR}_{D}(h) = \frac{\text{FP}_{D}(h)}{\text{TN}_{D}(h)+\text{FP}_{D}(h)}
\end{equation}
Where FP$_{D}(h)$ and TN$_{D}(h)$ are the numbers of 
false-positive detection and true-negative detection of $h$ on $D$,
respectively. 
\end{definition}
Note that since $D$ is from the same domain as $C$,
ensuring that TN$_{D}(h)$ + FP$_{D}(h)$ = $|D|$, 
$\text{FPR}_{D}(h)$ can be rewritten as:
\begin{equation}
\label{eqn:fpr}
\text{FPR}_{D}(h) = \frac{|\{v | v \in D, h \notin \mathbf{P}(v)\}|}{|\{v | v \in D \}|} = \text{Imp}_D(h)
\end{equation}
Thus allowing us to estimate $\text{FPR}_{D}(h)$ using $\text{Imp}_D(h)$.

\begin{example}
\label{ex:fpr-impurity}
Continue with Example~\ref{ex:fpr}, it can be
verified that the expected 
FPR of using $h$ as the validation pattern for $D$,
directly corresponds to the impurity $\text{Imp}_D(h)$ --
e.g., using $h_1$ to validate $D$ has $\text{FPR}_{D}(h_1)$
= $\text{Imp}_D(h_1)$ = $\frac{2}{12}$; while using 
$h_5$ to validate $D$ has $\text{FPR}_{D}(h_5) = \text{Imp}_D(h_5) = 0$, etc.
\end{example}

Based on FPR$_{D}(h)$ defined for one column $D \in \mathbf{T}$, 
we can in turn define the estimated FPR on the entire corpus $\mathbf{T}$,
using all column $D \in \mathbf{T}$ 
where some value $v \in D$ matches $h$:
\begin{definition}
\label{def:fpr_corpus}
Given a corpus $\mathbf{T}$, we estimate the 
FPR of pattern $h$ on  $\mathbf{T}$, 
denoted by FPR$_{\mathbf{T}}(h)$, as:
\begin{equation}
\label{eqn:fpr_agg}
\text{FPR}_{\mathbf{T}}(h) = \avg_{D \in \mathbf{T}, v \in D, h \in \mathbf{P}(v) }{\text{FPR}_{D}(h)}
\end{equation} 
\end{definition}
\vspace{-2mm}
%Note that $\text{FPR}_{\mathbf{T}}(h)$ uses
%all column $D \in \mathbf{T}$ where some value $v \in D$ 
%match $h$, or written as $h \in \mathbf{P}(v)$.

%This is consistent with our homogeneity assumption 
%of machine-generated data --
%because values in $D$ are generated by the same program
%and thus drawn from the same domain, 
%the fact that $v \in D$ matches a domain pattern $h$ 
%indicates that $D$ is from the same domain described by $h$,
%allowing us to use $\text{FPR}_{D}(h)$ as a piece of local evidence
%to estimate $h$.

\begin{example}
\label{ex:fpr_t}
Continue with the $h_5$ in Example~\ref{ex:fpr-impurity}. Suppose 
there are 5000 data columns $D \in \mathbf{T}$ 
where some value $v \in D$ matches $h_5$.
Suppose 4800 columns out of the 5000 have $\text{FPR}_{D}(h_5) = 0$, 
and the remaining 200 columns have $\text{FPR}_{D}(h_5) = 1\%$. 
The overall $\text{FPR}_{\mathbf{T}}(h_5)$ 
can be calculated as $\frac{200 * 1\%}{5000} = 0.04\%$,
using Equation~\eqref{eqn:fpr_agg}.
\end{example}



We emphasize that a low FPR is 
critical for data-validation, because given a large 
number of columns in production 
systems, even a 1\% FPR
translates into many false-alarms that require human
attention to resolve. FPR is thus a key objective we minimize.


\vspace{-2mm}
\subsection{Problem Statement}
We now describe the basic version 
of \sj{} as follows. 
Given an input query column $C$ and a background corpus $\mathbf{T}$,
we need to produce a validation pattern $h(C)$, 
such that $h(C)$ is expected to have a low FPR
but can still catch many quality issues.
We formulate this as an optimization problem.
Specifically, we introduce an FPR-Minimizing 
version of Data-Validation (FMDV), defined as:
\begin{align}
\hspace{-1cm} \text{(FMDV)} \qquad{} \min_{h \in \mathbf{H}(C)} & \text{FPR}_\mathbf{T}(h)   \label{eqn:fmdv_obj} \\ 
 \mbox{s.t.} ~~ & \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:fmdv_fpr} \\
 & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:fmdv_cov}
\end{align}
Where $\text{FPR}_\mathbf{T}(h)$ is the 
expected FPR of $h$ estimated using $\mathbf{T}$,
which has to be lower than a given target threshold $r$
(Equation~\eqref{eqn:fmdv_fpr}); and
$\text{Cov}_\mathbf{T}(h)$ is the coverage of $h$, or 
the number of columns in $\mathbf{T}$ that match $h$,
which has to be greater than a given threshold 
$m$ (Equation~\eqref{eqn:fmdv_cov}). Note that
these two constraints directly map to the 
two ``goodness'' criteria in Section~\ref{sec:intuition}.

The validation pattern $h$ we produce for $C$ is
then the minimizer
of FMDV from the hypothesis space 
$\mathbf{H}(C)$ (Equation~\eqref{eqn:fmdv_obj}).
We note that this can be interpreted as a conservative approach
that aims to find a ``safe'' pattern $h(C)$ with minimum FPR.

%ensures that the FPR is below
%a predefined target threshold $r$ (e.g., 1\% FPR would correspond
%to a target precision of 99\%), or otherwise we do not consider
%the solution to be feasible and do not produce a validation pattern.
%The second constraint in 
%ensures that the coverage of pattern $h(C)$ on $\mathbf{T}$
%is significant (e.g., $m$ = 1000, meaning that there are at least
%1000 columns in $\mathbf{T}$ matching this pattern), for otherwise
%this pattern $h(C)$ does not have sufficient representation in
%$\mathbf{T}$ for us to draw reliable conclusions, and furthermore
%if $h(C)$ only occurs once or twice it is unlikely to be a commonly
%used data-format for us to declare this to be a ``domain'' of data values.

%revised
%\iftoggle{fullversion}{
\begin{example}
\label{ex:fmdv}
Suppose we have FMDV with a target FPR rate $r$ no greater
than $0.1\%$, and a required coverage of at least $m = 100$.
Given the 3 example hypothesis patterns in Figure~\ref{fig:intuition},
we can see that patterns $h_1$ and $h_2$ are not feasible solutions
because of their high estimated FPR.
Pattern $h_5$ has an estimated FPR of 0.04\% and a coverage of 5000,
which is a feasible solution to FMDV.
\end{example}
%} %iftoggle


%\iftoggle{fullversion}{
\begin{lemma}
\label{lem:fmdv}
In a simplified scenario where each 
column in $\mathbf{T}$ has values drawn randomly from
exactly one underlying domain, and each domain in turn 
corresponds to one ground-truth
pattern. Then given a query column $C$ for which a validation pattern
needs to be generated,
and a corpus $\mathbf{T}$ with a large number ($n$) of 
columns generated from the same domain as $C$, 
with high probability (at least $1 - (\frac{1}{2})^n$), 
the optimal solution of FMDV 
for $C$ (with $r=0$) converges to the ground-truth pattern of $C$.
\end{lemma}



\iftoggle{fullversion}{
\begin{proofsketch}
We show that any candidate patterns 
that ``under-generalizes'' the
domain will with high probability 
be pruned away due to FPR violations (given $r=0$).
To see why this is the case, consider a pattern $p$ produced for $C$
that under-generalizes the ground-truth pattern $g$. Note
$p$ is picked over $g$ only when not a single value in all $n$ columns 
in the same domain as $C$
drawn from the space of values defined 
by $g$ are not in $p$ (since $r$ is set to 0). 
Because these $n$ columns are drawn randomly
from $g$ and each column has at least one value,
the probability of this happening is thus at most $(\frac{1}{2})^n$
($\frac{1}{2}$ is used because there is at least one branch
$p'$ in $g$ that is not in $p$), making the overall probability of success to be
$1 - (\frac{1}{2})^n$.
\end{proofsketch}
}
{
Intuitively, this result holds under the simplifying assumptions, 
because when given a sufficiently large number of $n$ columns in
$\mathbf{T}$ from the same domain as $C$, any candidate patterns 
that ``under-generalizes'' the
domain will be pruned away due to FPR violations, 
leaving the ground-truth pattern to be the optimal solution.
More details of the result can be found in~\cite{full}.
}


We also explored alternative formulations, such as 
coverage-minimizing data-validation (CMDV), where
we minimize coverage $\text{Cov}_\mathbf{T}(h)$
in the objective function in place of FPR$_\mathbf{T}(h)$ as in FMDV.
%The intuition here is that patterns with
%smaller coverage on $\mathbf{T}$ are more precise/restrictive
%and may catch more quality issues.
%\begin{align}
%\hspace{-1cm} \text{(CMDV)} \qquad{} \min_{h \in \mathbf{H}(C)} & \text{Cov}_\mathbf{T}(h)   \label{eqn:cmdv_obj} \\ 
% \mbox{s.t.} ~~ & \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:cmdv_fpr} \\
% & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:cmdv_cov}
%\end{align}
We omit details in the interest of space, 
but will report that the conservative FMDV is more
effective in practice. %(as CMDV tends to under-generalize).

A dual version of FMDV can be used for automated data-tagging, 
where we want to find the most restrictive 
(smallest coverage) pattern
to describe the underlying domain (which can be used to ``tag'' related
columns of the same type), under the constraint
of some target false-negative rate. We describe this dual version
in~\cite{auto-tag-tr}.


\subsection{System Architecture}
\label{sec:architecture}
While FMDV is simple overall, 
a naive implementation would
require a full scan of $\mathbf{T}$ to compute  
$\text{FPR}_\mathbf{T}(h)$ and $\text{Cov}_\mathbf{T}(h)$ for each
hypothesis $h$.
This is both costly and slow
considering the fact that  $\mathbf{T}$ is typically large 
in enterprise data lakes (e.g., in terabytes), 
where a full-scan can take hours. 
This is especially problematic for user-in-the-loop 
validation like in Google's TFDV, where users
are expected to review/modify suggested validation rules
and interactive response time is critical.

We thus introduce an offline index with summary
statistics of $\mathbf{T}$,  so that at online time and given a new 
query column $C$, 
we can evaluate hypothesis patterns $h$ efficiently using only the index, 
without needing to scan $\mathbf{T}$ again.

The architecture of our system can be
seen in Figure~\ref{fig:architecture}. 


\textbf{Offline stage.}
In the offline stage, we perform
one full scan of $\mathbf{T}$, enumerating all possible patterns for
each $D \in \mathbf{T}$ as 
$\mathbf{P}(D) = \cup_{v \in D} \mathbf{P}(v)$,
or the union of patterns for all $v \in D$
(where $\mathbf{P}$ is the generalization hierarchy 
in Section~\ref{sec:language}).
%that can ``cover'' a substantial fraction $\theta$ (e.g., 50\%) of values in 

Note that the space of $\mathbf{P}(D)$ 
can be quite large, especially for
``wide'' columns with many tokens as discussed in Figure~\ref{fig:generalization}. 
To limit $\mathbf{P}(D)$, in the basic version
we produce $\mathbf{P}(D)$ as 
$\cup_{v \in D, t(v)<\tau} \mathbf{P}(v)$, where $t(v)$ is the number
of tokens in $v$ (defined as the number of consecutive sequences
of letters, digits, or symbols in $v$), 
and $\tau$ is some fixed constant (e.g., 8 or 13) to make $\mathbf{P}(D)$
tractable.  We will describe how 
columns wider than $\tau$ can be safely skipped in offline 
indexing without affecting result quality, using 
a vertical-cut technique (in Section~\ref{sec:vertical-cuts}).
%(e.g., Figure~\ref{fig:generalization}
%can be decomposed into a date and a time-stamp).


For each pattern $p \in \mathbf{P}(D)$,
we pre-compute the local impurity score of $p$ on 
$D$ as $\text{Imp}_{D}(p)$,
since $p$ may be hypothesized 
as a domain pattern for some query column $C$ in the future,
for which this $D$ can provide a piece of local evidence.
%Recall that $\text{Imp}(D, p)$ directly corresponds to 
%$\text{FPR}_{D}(p)$ (Definition~\ref{def:fpr}), providing
%a piece of local evidence on the goodness of $p$.

Let $\mathbf{P}(\mathbf{T}) = \{p | p \in \mathbf{P}(D), D \in \mathbf{T}\}$
be the space of possible patterns in $\mathbf{T}$.
We pre-compute $\text{FPR}_{\mathbf{T}}(p)$ for
all possible $p \in \mathbf{P}(\mathbf{T})$
on the entire $\mathbf{T}$, 
by aggregating local $\text{Imp}_{D}(p)$ scores using
Equation~\eqref{eqn:fpr} and~\eqref{eqn:fpr_agg}.
The coverage scores $\text{Cov}_{\mathbf{T}}(p)$ of all $p$ can be 
pre-computed similarly as 
$\text{Cov}_{\mathbf{T}}(p) = |\{ D | D \in \mathbf{T}, v \in D, p \in \mathbf{P}(v) \}|$.

The result from the offline step is an index for lookup that maps
each possible $p \in \mathbf{P}(\mathbf{T})$, to its
pre-computed $\text{FPR}_{\mathbf{T}}(p)$ 
and $\text{Cov}_{\mathbf{T}}(p)$ values.
We note that this index is many
orders of magnitude smaller than the original
$\mathbf{T}$ -- e.g., a 1TB corpus $\mathbf{T}$ 
yields an index less than 1GB in our experiments.



\textbf{Online stage.}
At online query time, for a given
query column $C$, we enumerate $h \in \mathbf{H}(C)$,
and use the offline index to perform a lookup to retrieve 
$\text{FPR}_{\mathbf{T}}(p)$ and $\text{Cov}_{\mathbf{T}}(p)$
scores for FMDV, without needing to scan the full $\mathbf{T}$ again.
This indexing approach reduces our latency per 
query-column $C$ from hours to
tens of milliseconds, which makes it possible
to do interactive, human-in-the-loop
verification of suggested rules,
as we will report in experiments.



\begin{figure}[t]
        \centering
        \includegraphics[width=0.5\textwidth]{figures/architecture.png}
\caption{Architecture of the \sj{} System.}
\label{fig:architecture}
\end{figure}




















==> paper - arxiv-full-version/conclusions.tex <==
%!TEX root = main.tex

%\vspace{-3mm}
\section{Conclusions and Future Work}

Observing the need to automate data-validation 
in production pipelines, we propose a corpus-driven approach to
inferring single-column constraints that can be used to 
auto=validate string-valued data.
Possible directions of future work include extending beyond
``machine-generated data'' to consider
natural-language-like data, and extending the same validation 
principle also to numeric data.

\begin{comment}
Finally, although our current approach
exploits single-column constraints that are simple in structure 
and can be reliably learned from a corpus, extending this to 
multi-column constraints in an unsupervised manner 
(without requiring human verification like in typical FD-discovery)
would also be interesting direction of future work.
\end{comment}


==> paper - arxiv-full-version/experiments.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Experiments}
We implement our offline indexing algorithm in a Map-Reduce-like system
used internally at Microsoft~\cite{chaiken2008scope, zhou2012scope}. 
The offline job processes 7M columns with over 1TB data in under 3 hours. 
%Our online FMDV algorithms are implemented in C\#.


\vspace{-2mm}
\subsection{Benchmark Evaluation}
We build benchmarks using real data, to evaluate the quality of data-validation rules generated 
by different algorithms.

\textbf{Data set}. We evaluate algorithms using 
two real corpora:  

$\bullet$ \texttt{Enterprise:} We crawled data produced by
production pipelines from an enterprise data lake
at Microsoft. Over 100K daily production 
pipelines (for Bing, Office, etc.)-eps-converted-to.pdf
read/write data in the lake~\cite{zhou2012scope}.

$\bullet$ \texttt{Government}: We crawled data files
in the health domain from NationalArchives.gov.uk, following a procedure suggested in~\cite{bogatu2020dataset} 
(e.g., using queries like ``hospitals''). We used the crawler
from the authors of~\cite{bogatu2020dataset} (code is available from~\cite{crawler}).  These data files correspond to data in a different
domain (government).\footnote{This government benchmark is released at \url{https://github.com/jiesongk/auto-validate}.}



We refer to these two corpora as $\mathbf{T_{E}}$ and
$\mathbf{T_{G}}$, respectively.
The statistics of the two corpora can be found in f~\ref{tab:corpora}.

\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{|c | c | c | c | c | } 
 \hline
 Corpus & \begin{tabular}{@{}c@{}}total \# of \\ data files\end{tabular} & \begin{tabular}{@{}c@{}}total \# of \\ data cols\end{tabular} & \begin{tabular}{@{}c@{}} avg col value cnt \\ (standard deviation)\end{tabular}   & \begin{tabular}{@{}c@{}} avg col distinct value cnt \\ (standard deviation) \end{tabular}  \\  \hline
  \texttt{Enterprise} ($\mathbf{T_{E}}$) & 507K & 7.2M & 8945 (17778) & 1543 (7219) \\  \hline
 \texttt{Government} ($\mathbf{T_{G}}$) & 29K & 628K & 305 (331) &  46 (119) \\
 \hline
\end{tabular}
\caption{Characteristics of data corpora used.}
\label{tab:corpora}
\end{table}



\textbf{Evaluation methodology}.  
We randomly sample 1000 columns
from $\mathbf{T_{E}}$ and $\mathbf{T_{G}}$, respectively, 
to produce two benchmark sets of query-columns, denoted by
$\mathbf{B_{E}}$ and $\mathbf{B_{G}}$.\footnote{We use 
the first 1000 values of each column in $\mathbf{B_{E}}$
and the first 100 values of each column in 
$\mathbf{B_{G}}$ to control 
column size variations.}

Given a benchmark $\mathbf{B}$ with 1000 columns, 
$\mathbf{B} = \{C_i | i \in [1, 1000]\}$,
we programmatically 
evaluate the precision and
recall of data-validation rules generated on $\mathbf{B}$ 
as follows. For each column $C_i \in \mathbf{B}$, 
we use the first $10\%$ of values in $C_i$
as the ``training data'' that arrive first, 
denoted by $C_i^\text{train}$, from which
validation-rules need to be inferred. The remaining
$90\%$ of values are used as ``testing data''  $C_i^\text{test}$,
which arrive in the future but will be tested against the inferred
validation-rules.

Each algorithm $A$ can observe $C_i^\text{train}$ 
and ``learn'' data-validation 
rule $A(C_i^\text{train})$.
The inferred rule $A(C_i^\text{train})$ will be ``tested'' on two groups of
``testing data'': (1) $C_i^\text{test}$; and (2) $\{C_j | C_j \in \mathbf{B}, j \neq i\}$.

For (1), we know that when $A(C_i^\text{train})$ is used to 
validate against $C_i^\text{test}$, 
no errors should be detected
because $C_i^\text{test}$ and $C_i^\text{train}$ were 
drawn from the same column $C_i \in \mathbf{B}$.
If it so happens that $A(C_i^\text{train})$ incorrectly reports any error
on $C_i^\text{test}$, it is likely a false-positive.

For (2), when $A(C_i^\text{train})$ is used to validate 
$\{C_j | C_j \in \mathbf{B}, j \neq i\}$,
we know each $C_j$ ($j \neq i$) is likely from a different 
domain as $C_i$, and should be 
flagged by $A(C_i^\text{train})$. (This simulates schema-drift
and schema-alignment errors that are
common, because upstream data can add or remove
columns). This allows us to
evaluate the ``recall'' of each $A(C_i^\text{train})$.

More formally, we define the \textit{precision} of 
algorithm $A$ on test case $C_i$,
denoted by $P_A(C_i)$, as 1 if no value in $C_i^{test}$
 is incorrectly flagged
by $A(C_i^\text{train})$ as an error, and 0 otherwise.
The overall precision on benchmark $\mathbf{B}$ 
is the average across all cases:
%\begin{equation}
$P_{A}(\mathbf{B})  = \avg_{C_i \in \mathbf{B}} P_A(C_i)$.
%\end{equation}

The \textit{recall} of algorithm $A$ on case $C_i$, 
denoted by $R_A(C_i)$, is defined as the fraction of 
cases in $\{C_j | C_j \in \mathbf{B}, j \neq i\}$
that $A(C_i^\text{train})$
can correctly report as errors:
\begin{equation}
R_{A}(C_i)  = \frac{|\{C_j |\text{Validate}(C_j, A(C_i^\text{train})) = \text{fail}, C_j \in \mathbf{B}, j \neq i \}|}{|\{C_j | C_j \in \mathbf{B}, j \neq i \}|}
\end{equation}
Since high precision is critical for data-validation,
if algorithm $A$ produces false-alarms on case $C_i$,
we squash its recall $R_{A}(C_i)$  to 0. %(because 
%the false-alarms would likely have forced users
%to ignore/shut it).
The overall recall across all cases in $\mathbf{B}$ is then:
%\begin{equation}
$R_{A}(\mathbf{B})  = \avg_{C_i \in \mathbf{B}} R_A(C_i)$.
%\end{equation}

In addition to programmatic evaluation, we also
manually labeled each case in $\mathbf{B_{E}}$
with an ideal ground-truth validation-pattern. We use
these ground-truth labels, to both
accurately report precision/recall on $\mathbf{B_{E}}$,
and to confirm the validity of our programmatic evaluation
methodology.

\vspace{-2mm}
\subsection{Methods Compared}
\label{sec:methodsCompared}
We compare the following algorithms using each
benchmark $\mathbf{B}$, by reporting precision/recall numbers
$P_A(\mathbf{B})$ and $R_{A}(\mathbf{B})$.

\textbf{\sj}. This is our proposed approach. To understand the behavior of different variants of FMDV, we 
report FMDV, FMDV-V, FMDV-H, as well as a variant FMDV-VH
which combines vertical and horizontal cuts. For FMDV-H
and FMDV-VH, we report numbers using two-tailed
Fischer's exact test with a significance level of 0.01.
%(results using the Chi-squared test have no practical difference).


\textbf{Deequ}~\cite{schelter2019unit}. Deequ is a 
pioneering library from Amazon for declarative 
data validation. It is capable of suggesting data validation
rules based on  training data.
We compare with two relevant rules in Deequ for string-valued data
(version 1.0.2): the
CategoricalRangeRule (refer to as \texttt{Deequ-Cat}) and 
FractionalCategoricalRangeRule (referred to as 
\texttt{Deequ-Fra})~\cite{Deequ},
which learn fixed dictionaries
and require future test data to be in the dictionaries,
either completely (\texttt{Deequ-Cat}) or partially (\texttt{Deequ-Fra}).



\textbf{TensorFlow Data Validation (TFDV)}~\cite{TFDV}. 
TFDV is another pioneering data 
validation library for machine learning pipelines in TensorFlow. It can
also infer dictionary-based validation rules (similar to  \texttt{Deequ-Cat}).
We install TFDV via Python pip (version 0.15.0) and invoke it directly from Python.


\textbf{Potter's Wheel (PWheel)}~\cite{raman2001potter}. This is
an influential pattern-profiling method, which finds the best
pattern for a data column based on 
minimal description length (MDL). 

\textbf{SQL Server Integration Services 
(SSIS)}~\cite{ssis-profiling}. SQL Server 
has a data-profiling feature in SSIS. We invoke it programmatically
to produce regex patterns
for each column.

\textbf{XSystem}~\cite{ilyas2018extracting}. This recent
approach develops a flexible branch and
merges strategy to pattern profiling. We use the authors' implementation
on GitHub~\cite{xsystem-code} to produce patterns.

\textbf{FlashProfile}~\cite{padhi2018flashprofile}. FlashProfile
is a recent approach to pattern profiling, which clusters
similar values by a distance score. 
We use the authors' implementation
in NuGet~\cite{FlashProfileCode} to produce 
regex patterns for each column.


\textbf{Grok Patterns (Grok)}~\cite{grok}. Grok has a collection of
60+ manually-curated regex patterns, widely used in log parsing
and by vendors 
like AWS Glue ETL~\cite{Glue}, to
recognize common data-types
(e.g., time-stamp, ip-address, etc.). For data-validation,
we use all values in $C_i^\text{train}$ to determine whether there
is a match with a known Grok pattern (e.g., ip-address). This approach
is likely high-precision but low recall
because only common data-types are curated.


\textbf{Schema-Matching}~\cite{rahm2001survey}. Because \sj{}
leverages related tables in $\mathbf{T}$ as additional evidence to derive
validation patterns, we also compare with vanilla schema-matching  
that ``broaden'' the training examples using related
tables in $\mathbf{T}$. Specifically, we compare
with two instance-based techniques 
\val{Schema-Matching-Instance-1 (SM-I-1)} 
and \val{Schema-Matching-Instance-10 (SM-I-10)},
which use any column in $\mathbf{T}$ that overlaps with
more than 1 or 10 instances of $C_i^\text{train}$, respectively,
as additional training-examples.
We also compare with two pattern-based
\val{Schema-Matching-Pattern-Majority (SM-P-M)} 
and \val{Schema-Matching-Pattern-Plurality (SM-P-P)},
which use as training-data 
columns in $\mathbf{T}$ whose majority-pattern 
and plurality-patterns match those of 
$C_i^\text{train}$, respectively.  We invoke \val{PWheel}
on the resulting data, since it is the best-performing
pattern-profiling technique in our experiments.


\textbf{Functional-dependency-upper-bound (FD-UB)}. 
Functional dependency (FD) is an orthogonal approach that
leverages multi-column dependency for 
data quality~\cite{rahm2000data}. 
While FDs inferred from individual table instances
often may not hold in a semantic 
sense~\cite{berti2018discovery, papenbrock2016hybrid}, 
we nevertheless evaluate the
fraction of benchmark columns that are part of any FD
from their original tables,
which would be a recall upper-bound for FD-based approaches.
For simplicity, in this analysis, we 
assume a perfect precision for FD-based methods.



\textbf{Auto-Detect-upper-bound (AD-UB)}~\cite{huang2018auto}. 
Auto-detect is a recent approach that detects incompatibility 
through two common patterns that are rarely co-occurring.
For a pair of values $(v_1, v_2)$ to be recognized as incompatible
in Auto-detect, both of $v_1$ and $v_2$ need to correspond to
common patterns, which limits its coverage. 
%(In \sj only one pattern needs to be common). 
Like in \texttt{FD-UB}, we evaluate the recall 
upper-bound of Auto-detect (assuming a perfect precision).


%\rev{We should note that we compare all these methods on result 
%quality only (some of these existing methods are not known to be interactive
%and are omitted for latency comparisons).}

%\textbf{Missing-Val-upper-bound (MissingVal)}. 
%In order to evaluate what fraction of issues can be 
%Auto-detect is a recent approach that detects incompatibility 
%through two common patterns that are rarely co-occurring.
%For a pair of values $(v_1, v_2)$ to be recognized as incompatible
%in Auto-detect, both of $v_1$ and $v_2$ need to correspond to
%common patterns, which limits its coverage. 
%(In \sj only one pattern needs to correspond to 
%common). Like above, e evaluate the recall 
%upper-bound of Missing-Values (assuming a perfect precision).


\vspace{-2mm}
\subsection{Experimental Results}
\textbf{Accuracy.}
Figure~\ref{fig:result_pr_ent_scaled} 
shows average precision/recall of all 
methods using the enterprise benchmark $\mathbf{B_E}$ with 
1000 randomly sampled test cases.
Since no pattern-based methods (\val{FMDV}, \val{PWheel}, 
\val{SSIS}, \val{XSystem}, etc.) 
can generate meaningful patterns (except
the trivial ``\val{.*}'') 
on 429 out of the 1000 cases (because they have substantial 
natural language content for example), we report results
on the remaining 571  cases
in Figure~\ref{fig:result_pr_ent_scaled}, where pattern-based 
methods are applicable.% (additional analysis on the full result
%will be deferred to a full version of this paper in the interest of space).

It can be seen from Figure~\ref{fig:result_pr_ent_scaled}
that variants of FMDV are substantially better than other
methods in both precision and recall,
with FMDV-VH being the best at 0.96 precision and 0.88 recall on average.
FMDV-VH is better than FMDV-H,
which is in turn better than 
FMDV-V and FMDV, showing the benefit of using 
vertical-cuts and horizontal-cuts, respectively.



Among all the baselines, we find 
\val{PWheel} and \val{SM-I-1} (which uses schema-matching
with 1-instance overlap)
to be the most competitive, indicating that patterns
are indeed applicable to validating string-valued data, 
but need to be carefully selected to be effective.
%\texttt{XSystem} infers patterns using a sample 
%of data values, which tends to find narrow patterns 
%and thus low precision.

Our experiments on \texttt{FD-UB} confirm its orthogonal 
nature to single-column constraints considered by \sj --
the upper-bound recall of \texttt{FD-UB} only ``covers'' around 25\%
of cases handled by \sj 
(assuming discovered FDs have perfect precision).


The two data-validation
methods \texttt{TFDV} and \texttt{Deequ} do not 
perform well on string-valued data, 
partly because their current focus is
on numeric-data, and both use relatively simple 
logic for string data (e.g., dictionaries), which 
often leads to false-positives.
%\texttt{Deequ-Fra} implements a more sophisticated
%version of the dictionary-logic, which is still inadequate.
%}%iftoggle


Similar results can be observed on the government benchmark 
$\mathbf{B_G}$,
which is shown in 
Figure~\ref{fig:result_pr_gov_scaled}. (To avoid clutter, we omit 
methods that are not competitive in 
$\mathbf{B_E}$ in this figure).
This benchmark is more challenging because we 
have a smaller corpus and less clean data (e.g.,
many are manually-edited csv files), which leads to lower precision/recall
for all methods. Nevertheless, FMDV methods
still produce the best quality, showing the robustness of
the proposed approaches on challenging data corpus.
%\rev remove after revision
%\rev{The standard deviations of FMDV-VH are 0.277 for precision
%and 0.286 for recall, respectively.}




\begin{figure*}
\label{fig:result_pr}
    \centering
    \subfigure[\texttt{Enterprise} benchmark:
Numbers reported using a subset of 571 cases where syntactic patterns exist.]{\label{fig:result_pr_ent_scaled}\includegraphics[width=0.75\columnwidth]{figures/prec_vs_recall_scaled_corporate_C100_r0_1-eps-converted-to.pdf}}
    \qquad
    \subfigure[\texttt{Government} benchmark:
Numbers reported using a subset of 359 cases where syntactic patterns exist.
%(for which at least one profiling or validation method 
%can generate non-trivial patterns).
]{\label{fig:result_pr_gov_scaled}\includegraphics[width=0.75\columnwidth]{figures/data_gov_uk_scaled_corporate_C10_r0_1_5-3-eps-converted-to.pdf}}
    \caption[]{Recall vs. Precision comparisons of all methods, on \texttt{Enterprise} and \texttt{Government} benchmarks. 
}
    \label{fig:accuracy}
\vspace{-3mm}
\end{figure*}


\begin{table}[h!]
\vspace{-2mm}
\centering
\small
\begin{tabular}{|c | c| c|} 
 \hline
  Evaluation Method &  precision & recall  \\  \hline
  Programmatic evaluation  &   0.961  &  0.880 \\  \hline 
 Hand curated ground-truth &  0.963  & 0.915 \\  \hline
\end{tabular}
\caption{Quality results on $\mathbf{B_{E}}$, using programmatic evaluation vs. manually-cleaned ground-truth.}
\label{tab:compare-eval}
\end{table}


For all comparisons in Figure~\ref{fig:accuracy}
discussed above, we perform statistical tests using the F-scores
between FMDV-VH and all other methods on 1000 columns 
(where the null-hypothesis being the F-score of 
FMDV-VH is no better than a given baseline). We report
that the $p$-values of all comparisons range from 0.001 to 0.007
(substantially smaller than the $p<0.05$ level),
indicating that we should reject the null-hypothesis and the observed advantages are likely significant.


\textbf{Manually-labeled ground-truth.}
While our programmatic evaluation provides a good proxy of the ground-truth
without needing any labeling effort, we also perform a manual
evaluation to verify the validity of the programmatic evaluation.

Specifically, we manually label the ground-truth validation patterns
for 1000 test cases in $\mathbf{B_{E}}$, 
and perform two
types of adjustments: (1) To accurately report precision, 
we manually remove values in the test-set of each
column that should not belong to the column
(e.g., occasionally column-headers are parsed
incorrectly as data values), to ensure that we do not
unfairly punish methods that identify correct patterns; and 
(2) To accurately report recall, we identify
ground-truth patterns of each test query column, so that in recall
evaluation if another column is drawn from the same domain
with the identical pattern, 
we do not count it as a recall-loss.

We note that both adjustments \textit{improve}
the precision/recall, because our programmatic evaluation
\textit{under-estimates} the true precision/recall. 
Table~\ref{tab:compare-eval} compares the quality results
using programmatic evaluation and manual ground-truth,
which confirms the validity of the programmatic evaluation.


%revised
%\iftoggle{fullversion}{
%\textbf{Case-by-case analysis.}
Figure~\ref{fig:case_by_case} shows 
a case-by-case analysis of F1 results
on $\mathbf{B_E}$ with competitive
methods, using 100 randomly sampled
cases, sorted by their results on 
FMDV-VH to make comparison easy.
We can see that FMDV dominates other 
methods. An error-analysis on
the failed cases shows that these are mainly attributable
to advanced pattern-constructs such as 
flexibly-formatted URLs, and unions of distinct patterns, 
which are not supported by our current profiler. %-- it has
%close to perfect precision/recall
%on over 60\% cases.
%The rightmost of
%the figure shows 6 cases out of 100 for which FMDV produces an 
%F-score of 0. A detailed analysis shows that one case
%fails because of the capability of our profiling module --
%e.g., some columns require a \textit{union} of patterns,
%which is not supported by our current profiler (it is only
%supported by the commercial profiler \texttt{SSIS}).
%Two more cases fail because of hypothesis tests;
%and two other fail due to overly-narrow patterns
%resulting from a lax setting of $r = 0.1$. 
%The final case fails because the 
%test-data drawn from a column is ``dirty'' with
%mixed floating-numbers and date-time strings (rare in 
%machine-generated data), leading to validation failure
%(which however should not count against the algorithm). 



\begin{figure*}
\vspace{4mm}
  \includegraphics[width=0.9\textwidth]{figures/per_column_f1-eps-converted-to.pdf}
  \caption{Case-by-case results reported using F-1 scores, on 100 randomly sampled cases.}
  \label{fig:case_by_case}
\end{figure*}
%}%fullversion


\textbf{Sensitivity.}
Figure~\ref{fig:sensitivity} shows a detailed sensitivity analysis for
all FMDV variants using average precision/recall.
Figure~\ref{fig:sensitivity_r} shows the result with a
varying FRP target $r$, from the most strict 0 to a
more lax 0.1. As we can see, $r$ values directly translate
to a precision/recall trade-off and is an effective
knob for different precision targets. For the proposed
FMDV-VH variant, its performance is not sensitive for
$r \geq 0.02$. %, and setting $r$ to values like $0.05$ would be a safe
%choice in practice.

Figure~\ref{fig:sensitivity_C} shows the effect of
varying the coverage target $m$ from 0 to 100. 
We see that the precision/recall of
our algorithms is not sensitive to $m$ in most cases,
because the test columns we sample randomly are likely
to have popular patterns matching thousands of columns.
We recommend using a large $m$ (e.g., at least 100) to ensure
confident domain inference.


Figure~\ref{fig:sensitivity_to_index_tau} shows the
impact of varying $\tau$, which is the max
number of tokens in a column for it to be indexed (Section~\ref{sec:architecture}).
As can be seen from the figure, algorithms using vertical-cuts
(FMDV-V and FMDV-VH) are insensitive to smaller
$\tau$, while algorithms without vertical-cuts
(FMDV and FMDV-H) suffer substantial recall loss with a small
$\tau=8$, which shows the benefit of using vertical-cuts.
We recommend using FMDV-VH with a small $\tau$ (e.g., 8), 
which is efficient and inexpensive to run.

Figure~\ref{fig:sensitivity_to_theta} shows the sensitivity
to $\theta$. We can see that the algorithm is not sensitive to $\theta$,
as long as it is not too small.

\begin{comment}
Finally, we consider the sensitivity of our algorithm to 
time, by ``training'' using data tables that are at least 6-month old,
and ``testing'' using data created within the last 6-months.
Here, we are strictly training using ``past'' data and
predicting on ``future'' data, by essentially stop ``training'' for 6 months.

From Table~\ref{tab:sensitivity-time}, we 
observe a 5\% drop in precision and 11\% drop in recall. We should
highlight that these are still substantially better than all other 
methods compared (Figure~\ref{fig:result_pr_ent_scaled}).
This experiment underlines the importance of ``re-training'', but also
shows the robustness of our approach even with
very infrequent training. 


\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c |} 
 \hline
  Test data drawn from & \# of cols w/ patterns (tested) & precision & recall  \\  \hline
  $[0, T)$  & 558 (1000) &  0.960  &  0.901  \\  \hline %[0, $T$) 
 $[T, T$+6-months$)$ & 626 (1000) &  0.918  &  0.797\\ %[$T$, $T$+6 month) 
 \hline
\end{tabular}
\caption{Sensitivity to time, when ``trained'' using data
created in time $[0, T)$, ``tested'' using 1000 columns
sampled from data created in $[0, T)$ vs. $[T, T$+6-months$)$.}
\vspace{-2mm}
\label{tab:sensitivity-time}
\end{table}
\end{comment}


%\iftoggle{fullversion}
%{
\begin{figure*}
%\vspace{-10mm}
    \centering
    \subfigure[Sensitivity to FPR threshold ($r$)]{\label{fig:sensitivity_r}\includegraphics[height=5.7cm]{figures/sensitivity_to_r-eps-converted-to.pdf}}
    \qquad
    \subfigure[Sensitivity to Coverage ($m$)]{\label{fig:sensitivity_C}\includegraphics[height=5.7cm]{figures/sensitivity_to_C-eps-converted-to.pdf}}
    \qquad
    \subfigure[Sensitivity to token-limit ($\tau$)]{\label{fig:sensitivity_to_index_tau}\includegraphics[height=5.7cm]{figures/sensitivity_to_index_atom_num-eps-converted-to.pdf}}
    \qquad
    \subfigure[Sensitivity of FMDV-H to ($\theta$)]{\label{fig:sensitivity_to_theta}\includegraphics[height=5.7cm]{figures/sensitivity_to_theta-eps-converted-to.pdf}}
    
    \caption[]{Sensitivity analysis of FMDV algorithms on the Enterprise benchmark.}
    \label{fig:sensitivity}
\end{figure*}
%}%iftoggle



\iftoggle{fullversion}
{
\textbf{Pattern analysis.}
Because our offline index enumerates all possible patterns that can 
be generated from $\mathbf{T}$, it provides 
a unique opportunity to understand: (1) all common domains
in $\mathbf{T}$ independent of query-columns, defined as patterns
with high coverage and low FPR; and (2) the characteristics of all
candidate patterns generated from $\mathbf{T}$. 

For (1) we inspect the 
``head'' patterns in the index file, 
e.g. patterns matching over 10K columns and with low FPR.
This indeed reveals many
common ``domains'' of interest in this data lake, 
some examples of which are shown in 
Figure~\ref{fig:domain-example}. We note that
identifying data domains in proprietary 
formats have applications beyond 
data validation (e.g., in enterprise data search),
and is an interesting area for future research.

For (2), we show an
analysis of all patterns in $\mathbf{T}$
using the index
in Figure \ref{fig:pattern_analysis}.
Figure~\ref{fig:pattern_by_token} shows
the frequency of patterns by token-length
(each \val{<num>}, \val{<letter>}, etc.
is a token). We can see that
the patterns are fairly evenly distributed,
where patterns with 5-7 token are the most common.
Figure~\ref{fig:pattern_by_freq} shows
the frequency of all distinct candidate patterns.
We observe a power-law-like distribution -- while
the ``head'' patterns are likely useful domain patterns,
the vast majority have low coverage that are either
generalized too narrowly or are not common domains.


\begin{figure}
    \centering
    \subfigure[Pattern distr. by \#-of-tokens]{\label{fig:pattern_by_token}\includegraphics[width=0.45\columnwidth]{figures/indexByNumOfAtoms-eps-converted-to.pdf}}
    \qquad
    \subfigure[Pattern distr. by frequency]{\label{fig:pattern_by_freq}\includegraphics[width=0.45\columnwidth]{figures/indexByNumOfCols-eps-converted-to.pdf}}
    
    \caption[]{Distribution of patterns in the offline index.}
    \label{fig:pattern_analysis}
\end{figure}
}% \iftoggle full version



\textbf{Efficiency.}
Figure~\ref{fig:latency} shows the average latency
(in milliseconds) to process  one query column $C$ in our benchmark.
We emphasize that low latency is critical
for human-in-the-loop scenarios (e.g.,
TFDV), where users are expected to verify suggested constraints.

On the right of the figure, we can see the average latency 
for \val{PWheel}, \val{FalshProfile}, and \val{XSystem}, respectively
(we use authors' original implementations for the last two methods~\cite{FlashProfileCode, xsystem-code}).
It can be seen that these existing pattern-profiling techniques all require
on average 6-7 seconds per column. Given that tables often have tens of columns, the end-to-end latency can be slow.

In comparison, we observe that despite using a more
involved algorithm and a large corpus $\mathbf{T}$, 
all FMDV variants are two orders
of magnitude faster, 
where the most expensive FMDV-VH takes only 0.082 seconds
per column. This demonstrates the benefit of the offline indexing
step in Section~\ref{sec:architecture}, which 
distills $\mathbf{T}$ (in terabytes) down to a small index 
with summary statistics (with less than one gigabyte), 
and pushes expensive reasoning to offline, allowing 
for fast online response time.
As an additional reference point, if we do not 
use offline indexes, the ``FMDV (no-index)'' method
has to scan $\mathbf{T}$ for each query and is many orders of magnitude slower.



%Between the FMDV variants, we can see that the average 
%latency for FMDV is 48ms and is
%the least expensive as expected. It is encouraging to
%see that the more complex FMDV-H, FMDV-V
%and FMDV-VH are not much more expensive, 
%but can bring significant improvement over FMDV
%in terms of quality, making these complex FMDV variants
%practical solutions to data validation.

For the offline indexing step, we report that
the end-to-end latency of our job (on a cluster with
10 virtual-nodes) ranges from around 1 hour (with
$\tau = 8$), to around 3 hours (with $\tau = 13$).
We believe this shows that our algorithm is viable even
on small-scale clusters, despite using a large number of patterns.


\begin{figure}
  \includegraphics[width=0.45\textwidth]{figures/latency-all.png}
  \caption{Latency in milliseconds (per query column).}
  \label{fig:latency}
\end{figure}



\textbf{User study.}
To evaluate the human benefit of suggesting data-validation
patterns, we perform a user study by recruiting 5 
programmers (all with at least 5 years of 
programming experience),
to write data-validation patterns for 20 sampled test
columns in benchmark $\mathbf{B_E}$.  
This corresponds to the scenario of developers manually 
writing patterns without using the proposed algorithm. 


\begin{table}[t]
%\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c |} 
 \hline
  Programmer & avg-time (sec) & avg-precision & avg-recall  \\  \hline
   \#1 & 145 & 0.65 & 0.638  \\  \hline 
   \#2 & 123 & 0.45 & 0.431  \\  \hline
   \#3 & 84 & 0.3 & 0.266  \\  \hline
   FMDV-VH & \textbf{0.08} & \textbf{1.0}  & \textbf{0.978} \\  \hline
\end{tabular}
\caption{User study comparing 3 developers with 
FMDV-VH on 20 test columns,  by time spent and pattern quality.}
\label{tab:user-study}
\end{table}


We report that 2 out of the 5 users fail completely
on the task (their regex are either 
ill-formed or fail to match given examples). 
Table~\ref{tab:user-study} shows the results for the
remaining 3 users. We observe that on average, they
spend 117 seconds
to write a regex for one test column (for it often
requires many trials-and-errors). This is in sharp contrast to 
0.08 seconds required by our algorithm. Programmers' average 
precision is 0.47, also substantially
lower than the algorithm's precision of 1.0 on hold-out test data.



\textbf{Case studies using Kaggle.}
In order to use publicly available data sets 
to assess the benefits of data
validation against schema-drift,
we conduct a case study using 11 tasks sampled from
Kaggle~\cite{kaggle}, where each task
has at least 2 string-valued categorical attributes.
These 11 tasks include 7 for classification: 
\val{Titanic}, \val{AirBnb}, \val{BNPParibas}, \val{RedHat}, 
\val{SFCrime}, \val{WestNile}, \val{WalmartTrips};
and 4 for regression: \val{HousePrice}, \val{HomeDepot},
\val{Caterpillar}, and \val{WalmartSales}.

To simulate
schema-drift~\cite{breck2019data, polyzotis2017data, 
schelter2018automating}, for each Kaggle task,
we keep the training data unchanged, but swap 
the position of the categorical attributes in the testing data (e.g.,
if a data set has two attributes \val{date} and \val{time} at column-position
1 and 2, respectively, after simulated 
schema-drift the two attributes will be at column-position
2 and 1, respectively). This creates a small schema-mismatch between
training/testing data that is hard to detect but can be 
common in practice like explained in~\cite{breck2019data, polyzotis2017data}. 
%test data often arrive later in time and may be
%processed on a different platform (e.g., due to low-latency requirements), 
%using program-logic slightly different from the 
%logic used on training data (e.g., due to
%program evolution).


%We test two setups here.
%(1)  \val{Train-Orig-Test-SchemaDrift}: In this
%variant, schema-shift occurs only in the test data that arrives 
%later in time, but no the training data, 
%so that test data and training data have slightly different
%schema; and
%(2) \val{Train-SchemaDrift-Test-Orig}: In this variant, 
%schema-drift occurs
%in the last 50\% rows of the training data (because training data
%can often accumulate over a long period of 
%time, and schema-drift may happen during 
%the process).



\begin{figure*}
  \includegraphics[width=0.7\textwidth]{figures/Kaggle.png}
  \caption{Impact of schema-shift on Kaggle tasks, with and without
data-validation. FMDV detects schema-drift in 
8 out of 11 cases.}
  \label{fig:kaggle}
\end{figure*}

Figure~\ref{fig:kaggle} shows the quality results with
and without validation on these Kaggle
tasks. For all tasks, we use a popular GBDT method 
called XGBoost~\cite{xgboost} with default parameters.
We report R2 for regression tasks and 
average-precision for classification tasks.

The left (blue) bar of each task, labeled as \val{No-SchemaDrift},
shows the prediction-quality scores, on the original
datasets and without schema-drift. We normalize these scores as 100\%.
The middle (green)
bar, \val{SchemaDrift-without-Validation}, shows the quality scores
with schema-drift, measured 
relative to the original quality scores.
We observe a drop up to 78\% (\val{WalmartTrips}) in normalized 
scores. %\val{WestNile} and \val{HomeDepot} show
%no quality regression with schema-drift, because the default XGBoost
%produces a poor fit on these two hard tasks (which are not too different from random guesses).
Lastly, the right (red) bar, \val{SchemaDrift-with-Validation}
shows the quality when data-validation is used, 
which correctly detect schema-drift in 8 out of 11 tasks
(all except \val{WestNile}, \val{HomeDepot} and \val{WalmartTrips},
with no false-positives). Addressing 
such validation alerts would significantly boost the resulting quality scores.
s
While it is generally known that schema-drift
hurts ML quality~\cite{breck2019data, TFDV}, our analysis
quantifies its impact on publicly available data and
confirms the importance of data-validation.

\balance



==> paper - arxiv-full-version/introduction.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Introduction}

Complex data pipelines and data flows are increasingly common
in today's BI, ETL and ML systems
(e.g., in Tableau~\cite{tableau-flow}, 
Power BI~\cite{power-bi-flow}, Amazon Glue~\cite{amazon-workflow},
Informatica~\cite{Informatica}, Azure ML~\cite{azureml-pipelines}, etc.).
%Figure~\ref{fig:pipelines} shows example pipelines in
%Tableau (for BI), Informatica (for ETL), and AzureML (for ML), respectively.
These pipelines typically \textit{recur regularly} (e.g., daily), 
as BI reports need to be refreshed regularly~\cite{dayal2009data, schelter2018automating}, 
data warehouses need to be 
updated frequently~\cite{vassiliadis2009near}, and
ML models need to be retrained continuously (to
prevent model degradation)~\cite{breck2019data, polyzotis2017data}.


However, it is
widely recognized (e.g.,~\cite{breck2019data, hynes2017data, polyzotis2017data, schelter2018automating, 
schelter2019unit, schelter2019differential}) 
that in recurring production
data pipelines, over time upstream data feeds can often change in
unexpected ways. For instance, over time, data
columns can be added to or removed in upstream data,
creating \textit{schema-drift}~\cite{breck2019data, 
polyzotis2017data,  schelter2018automating}. 
Similarly, \textit{data-drift}~\cite{polyzotis2017data} is also
common, as the 
formatting standard of data values can change silently
(e.g., from ``\val{en-us}'' to ``\val{en-US}'', as reported in~\cite{polyzotis2017data}); and
invalid values
can also creep in (e.g., ``\val{en-99}'', for unknown locale).

Such schema-drift and data-drift can lead to quality issues
in downstream applications, which are both hard to detect 
(e.g., modest model degradation due to  
unseen data~\cite{polyzotis2017data}), and
hard to debug (finding root-causes in complex pipelines
can be difficult).
These silent failures require substantial human
efforts to resolve, 
increasing the cost of running production data pipelines
and decreasing the effectiveness of data-driven 
system~\cite{breck2019data, polyzotis2017data, 
schelter2018automating, schelter2019unit}.


\textbf{Data Validation by Declarative Constraints.}
Large tech companies operating large numbers of complex pipelines are the first to recognize the need to catch data quality issues
early in the pipelines. In response, they pioneered a number of 
``data validation'' tools, including Google's TensorFlow Data 
Validation (TFDV)~\cite{breck2019data, TFDV} and
Amazon's Deequ~\cite{Deequ, schelter2018automating}, etc.
%and LinkedIn's Data Sententiel~\cite{swami2020data},
These tools develop easy-to-use \textit{domain specific languages} (DSLs),
for developers and data engineers to write declarative
\textit{data constraints} that describe how ``normal'' data 
should look like in the pipelines, so that
any unexpected deviation introduced over time can be caught early
as they arise.


Figure~\ref{fig:deequ} shows an example code snippet\footnote{\url{https://aws.amazon.com/blogs/big-data/test-data-quality-at-scale-with-deequ/}}
from Amazon Deequ~\cite{schelter2018automating} to specify
data validation constraints on a table. 
In this case, it is declared
that values in the column ``\val{review\_id}'' need to be unique, column
``\val{marketplace}'' is complete (with no
\val{NULL}s), values in ``\val{marketplace}'' need to be
in a fixed dictionary 
\{``\val{US}'', ``\val{UK}'', ``\val{DE}'', ``\val{JP}'', ``\val{FR}''\}, etc.
Such constraints will be used to validate against data arriving
in the future, and raise alerts if violations are detected.
Google's TFDV uses a similar declarative approach 
with a different syntax.

These approaches allow users to
provide \textit{high-level specifications} of data
constraints, and is a significant improvement over 
 \textit{low-level} assertions used in ad-hoc validation scripts (which are
are hard to program and maintain)~\cite{breck2019data, TFDV,
Deequ, schelter2018automating, swami2020data}.

%We should also mention that data-validation is important 
%for \textit{any} data-driven enterprises (and not just large tech companies),
%as evidenced by data-validation features in
%enterprise-grade software
%such as Informatica Data Quality Rules~\cite{Informatica-DQ-rules}.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.45\textwidth]{figures/deequ-example-2.png}
\caption{Example code snippet to describe expected data-values, using declarative constraints in Amazon Deequ.}
\vspace{3mm}
\label{fig:deequ}
\end{figure}



\begin{comment}
\begin{figure*}
\vspace{-12mm}
\hspace{-0mm}\subfigure[Tableau (BI)] {
        \label{fig:wiki-spelling}
       \centering
        \includegraphics[width=0.32\textwidth]{figures/pipeline-tableau.png}} 
\hspace{-0mm}\subfigure[Informatica (ETL)] {
        \label{fig:wiki-uniqueness}
        \centering
        \includegraphics[width=0.3\textwidth]{figures/pipeline-informatica.png}}
%\hspace{-0mm}\subfigure[Alteryx (ETL)] {
 %       \label{fig:wiki-uniqueness}
 %       \centering
%        \includegraphics[width=0.32\textwidth]{figures/pipeline-alteryx.png}}
\hspace{-0mm}\subfigure[Azure ML (ML)] {
        \label{fig:wiki-uniqueness}
        \centering
        \includegraphics[width=0.32\textwidth]{figures/pipeline-azureml.png}}
\caption{Example data pipelines from BI tools (Tableau), ETL tools (Informatica), and ML tools (Azure ML). Complex data pipelines are very common in all types of data-driven
systems today.}\label{fig:pipelines}
\vspace{-3mm}
\end{figure*}
\end{comment}


\textbf{Automate Data Validation using Inferred Constraints.}
While declarative data validation clearly improves over 
ad-hoc scripts, and is beneficial as reported
by both Google and Amazon~\cite{breck2019data, schelter2018automating},
the need for data engineers to manually write
data constraints \textit{one-column-at-a-time} (e.g., 
in Figure~\ref{fig:deequ}) still makes it time-consuming 
and hard to scale. This is especially true for complex production data,
where a single data feed can have hundreds of
columns requiring substantial manual work.
As a result, experts today can only afford to write 
validation rules for
part of their data (e.g., important columns). 
Automating the generation of 
data validation constraints has 
become an important problem.

The main technical challenge here is that validation rules 
have to be inferred using data values 
\textit{currently observed} from a 
pipeline, but the inferred rules have to apply
to future data that \textit{cannot yet be observed}
(analogous to training-data/testing-data in ML settings where
test-data cannot be observed).
Ensuring that validation rules \textit{generalize} to unseen future data is thus
critical.


We should note that existing solutions already 
make efforts in this direction -- 
both Google TFDV and Amazon Deequ can scan 
an existing data feed, and automatically suggest validation
constraints for human engineers to inspect and approve.
Our analysis suggests that the capabilities of
these existing solutions are still rudimentary, especially
on \textit{string-valued data columns}.
For instance, for the example $C_1$
in Figure~\ref{fig:datetime-example}(a) with
date strings in \val{Mar 2019},
TFDV would infer a validation rule\footnote{This was initially tested on TFDV version 0.15.0, the latest version available in early 2020. We tested it again at the time of publication in March 2021 using the latest TFDV version 0.28.0, and observed the same
behavior for this test case.}  requiring all future values
in this column to come from a fixed dictionary 
with existing values in $C_1$:
\{`` \val{Mar 01 2019}'', \ldots `` \val{Mar 30 2019}'' \}.
This is too restrictive for data validation, 
as it can trigger false-alarms on future data
(e.g. values like ``\val{Apr 01 2019}'').
Accordingly, TFDV documentation does not recommend
suggested rules to be used directly, and
``\textit{strongly advised developers to review 
the inferred rule and refine it as needed}''\footnote{\url{https://www.tensorflow.org/tfx/data_validation/get_started}}.

When evaluated on production data (without human intervention), we
find TFDV produces false-alarms on over 90\%
string-valued columns.
%suggests that TFDV %\footnote{Tested on version 0.15.0, 
%%the latest version available as of Nov 2019.}
%almost always generate restrictive dictionaries
%as validation rules for string-valued data, producing a high
%false-positive rate. 
Amazon's Deequ considers distributions of values
but still falls short, triggering false-alarms on over 20\% columns.
Given that millions of data columns are processed daily
in production systems, these false-positive rates
can translate to millions of false-alarms,
which is not adequate for automated applications.


\begin{figure*}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/datetime-example.png}
\caption{Two example data columns $C_1$ and $C_2$. 
The top portion of each column
shows data in the current feed that can be observed, 
while the bottom portion shows
values that will arrive in the future.}
\label{fig:datetime-example}
\end{figure*}


%The upshot is that while automating data validation
%is an important direction, 
%current solutions are not yet
%sufficient (especially for \textit{string-valued  data}).

\textbf{Auto-Validate string-valued data using patterns.}
We in this work aim to infer
accurate data-validation rules for \textit{string-valued data},
using regex-like patterns. We perform an in-depth
 analysis of production data 
in real pipelines, from a large 
Map-Reduce-like system used 
at Microsoft~\cite{patel2019big, zhou2012scope},
which hosts over 100K production jobs each 
day, and powers popular products like Bing Search and Office.
We crawl a sample of 7M columns from the data lake hosting
these pipelines and find string-valued columns
to be prevalent, accounting for 75\% of 
columns sampled.% (data stored as strings but can be
%parsed as numbers are not included).


\begin{figure*}[t]
        \centering
        \includegraphics[width=1\textwidth]{figures/example-domain.png}
\caption{Example columns crawled from a production enterprise data lake.  Each
column has a distinctive data pattern in proprietary
formats, encoding specific meanings (the first column is
anonymized for review). 
These are all common patterns found in at least 5000 columns.}
\label{fig:domain-example}
\vspace{-3mm}
\end{figure*}


Figure~\ref{fig:domain-example} shows 7 example string-valued
columns from the crawl. A key characteristic common to
many such columns, is that these columns have \textit{homogeneous}
and \textit{machine-generated} data values, which exhibit
distinct ``patterns'' that encode specific semantic meanings. In our 
examples,  these include 
knowledge-base entity-id~\cite{BingEntity} (used by Bing Search), 
online-ads delivery status (used by search ads), 
time-stamps in proprietary formats  (used by search ads), etc.
We note that these are not one-off patterns occurring just
once or twice -- each pattern 
in Figure~\ref{fig:domain-example}
shows up in at least 5000 data columns in our crawl, suggesting
that these are widely-used concepts.
Similar data are likely common in other industries and
domains (e.g., for pharmaceutical or
financial companies~\cite{stonebraker2018data}).

In this work, we focus on these string-valued columns
that have homogeneous machine-generated data values.
Specifically, if we could infer suitable patterns to describe the
underlying ``domain'' of the data (defined as the space of 
all valid values),  we can use such patterns 
as validation rules against data in the future.
For instance, the pattern 
``{\small \texttt{<letter>\{3\} <digit>\{2\} <digit>\{4\}}}''
can be used to validate 
$C_1$ in Figure~\ref{fig:datetime-example}(a),
and ``{\small \texttt{<digit>+/<digit>\{2\}/<digit>\{4\} <digit>+:<digit>\{2\}:<digit>\{2\} <letter>\{2\}}}''
for $C_2$ in Figure~\ref{fig:datetime-example}(b).


Our analysis on a random sample of 1000 columns 
from our production data lake
suggests that around 67\% string-valued columns
have homogeneous machine-generated values
(like shown in Figure~\ref{fig:domain-example}), whose
underlying data-domains are amenable to pattern-based
representations (the focus of this work). 
The remaining 33\% columns have \textit{natural-language (NL) content}
(e.g., company names, department names, etc.),
for which pattern-based approaches would be less well-suited.
We should emphasize that for large data-lakes and production
data pipelines, machine-generated data will likely dominate (because 
machines are after all more productive at churning out large volumes of data
than humans producing NL data), making our proposed
technique widely applicable.
%or have complex structures beyond the expressiveness 
%of a regular language~\cite{rozenberg2012handbook}.



%revised
\iftoggle{fullversion}{
While on the surface this looks similar 
to prior work on \textit{pattern-profiling}
(e.g., Potter's Wheel~\cite{raman2001potter}
and PADS~\cite{fisher2005pads}), which
also learn patterns from values, 
we highlight the key differences in their objectives
that make the two entirely different problems.


\textbf{Data Profiling vs. Data Validation.}
In pattern-based data profiling, the main objective is to ``summarize''
a large number of values in a column $C$, 
so that users can quickly understand
content is in the column without needing to scroll/inspect every value.
As such, the key criterion is to select 
patterns that can succinctly 
describe given data values in $C$ \textit{only},
\textit{without needing to consider values not present in $C$}.

For example, existing pattern profiling
methods like Potter's Wheel~\cite{raman2001potter}
 would correctly
generate a desirable pattern 
``{\small \texttt{Mar <digit>\{2\} 2019}}'' for $C_1$ in 
Figure~\ref{fig:datetime-example}(a), which is valuable
from a pattern-profiling's perspective as it succinctly describes
values in  $C_1$.
However, this pattern is not suitable for 
data-validation, as it is overly-restrictive
and would trigger false-alarms for values
like ``{\small \texttt{Apr 01 2019}}'' arriving in the future. A more appropriate
data-validation pattern should instead be
``{\small \texttt{<letter>\{3\} <digit>\{2\} <digit>\{4\}}}''. 
Similarly, for $C_2$, Figure~\ref{fig:datetime-example}(b) shows
that a pattern ideal for profiling
is again very different from one suitable for data-validation.
}%iftoggle


\begin{figure}
        \centering
        \includegraphics[width=0.3\textwidth]{figures/hierarchy.png}
\caption{Example string generalization hierarchy.}
\label{fig:hierarchy}
\end{figure}

\begin{figure}
        \centering
        \includegraphics[width=0.5\textwidth]{figures/generalization-possibilities.png}
\caption{Possible ways to generalize a column of date-time strings, using the
hierarchy in Figure~\ref{fig:hierarchy}.}
\label{fig:generalization}
\end{figure}


Conceptually, there are many ways to ``generalize'' a column
of data into patterns. For a simple column of date-time strings
like in Figure~\ref{fig:generalization}, and using a standard generalization 
hierarchy (Figure~\ref{fig:hierarchy}), one could generate over 3 billion
patterns. For example, the first part
(digit ``\val{9}'' for month) alone can be generalized in 7 different
ways below, also shown in the top-right box of Figure~\ref{fig:generalization}.
\begin{small}
\begin{itemize}[leftmargin=*, ,topsep=0pt]
\item[](1) a constant ``{\small \texttt{9}}'' ({\small \texttt{Const(``9'')}}), 
\item[](2) one single digit ({\small \texttt{<digit>\{1\}}}), 
\item[](3) at least one digits ({\small \texttt{<digit>+}}), 
\item[](4) any number including floating-points ({\small \texttt{<num>}}), 
\item[](5) one alpha-numeric character ({\small \texttt{<alphanum>}}), 
\item[](6) at least one alpha-numeric characters ({\small \texttt{<alphanum>+}}), 
\item[](7) root of the hierarchy ({\small \texttt{<all>}})
\end{itemize}
\end{small}

The cross-product of these options at each position 
creates a large space of patterns (about 3.3 billion)  
  for this simple column.

The challenge for data-validation, is to select suitable
patterns from this large space given only
observed values in $C$, in
anticipation of valid values from the same ``domain''
that may arrive in the future.
The key is to not use
overly restrictive patterns (as in data-profiling),
which would yield many false-positive alerts.
Conversely overly general 
patterns (like the trivial ``\texttt{.*}'') should also
not be used, as they would 
fail to detect any data quality issues. 
In effect, we want to find
patterns that balance two conflicting goals: 
(1) reduce false-alarms 
(or improve detection precision); 
and (2) catch as many issues
as possible (or improve detection recall).

\textbf{A corpus-driven approach to pattern-inference.}
Intuitively, the pattern-inference problem is hard if we 
only look at one input column $C$ -- for the date-time examples in 
Figure~\ref{fig:datetime-example}, 
we as humans know what
patterns are suitable; 
but for the examples in Figure~\ref{fig:domain-example}
drawn from proprietary domains, even
humans may find it hard to determine suitable validation
patterns, and would need to seek
``additional evidence'', such as
other ``similar-looking columns''.  

Following this intuition, we in this work formulate
pattern-inference as optimization problems, by
leveraging a large corpus of related tables 
$\mathbf{T}$ (e.g. data produced by production pipelines and
dumped in
the same enterprise data lake). Our inference algorithms leverage 
columns ``similar'' to $C$ in $\mathbf{T}$, to 
reason about patterns that may be ideal for data-validation.
%Conceptually, for a given data column $C$, 
%we enumerate all possible candidate patterns for $C$
%and estimate their false-positive and 
%false-negative rates using $\mathbf{T}$.
%The pattern selection problem are then
%formulated as optimization problems.
%an application scenario that can tolerate a
%false-alarm rate of
%1\% would translate into 
%a precision level of 99\% -- i.e., for every 100 
%data-validation our patterns detect, 1 of which is a false-positive
%while 99 are true data quality issues.

%We further study two additional problem formulations
%to deal with challenges in real data: one with ``vertical-cuts''
%that can handle composite data columns; and the other with
%``horizontal-cuts'' that deals with ad-hoc ``dirty''
%values (e.g., ``null'', ``N.A.'', ``-'', etc.) in the same column. 

%We compare the proposed approach with alternative methods
%using real production data.
%Specifically, we take the
%first $p$\% of values from each real data column $C$ 
%as the ``training data'', for algorithms to 
%infer suitable validation pattern $h(C)$.
%The remaining ($1-p\%$) values in $C$ arriving in the future
%are used as ``test data'', which we know should not be incorrectly 
%detected as errors
%by validation rules $h(C)$ (this evaluates ``precision'').
%Furthermore, we sample values from other domains, 
%which we know should trigger validation errors using $h(C)$
%(this evaluates ``recall'').

\begin{comment}
It is worth noting that the proposed \sj{} can be seen as a unsupervised
method to infer \textit{single-column} data-quality constraints, 
which naturally complements with \textit{multi-column}
constraints (e.g. FDs).
Crucially, because \sj{} infers constraints 
from \textit{a large corpus of data in data lakes}, the resulting
constraints are reliable enough to be auto-applied at scale 
with a low false-positive rate. In comparison, typical multi-column
methods infer constraints (e.g., FDs) 
from \textit{one single table instance},
which often do not hold in a semantic sense~\cite{berti2018discovery, papenbrock2016hybrid} and require human
verification (thus cannot be applied directly to millions of tables
at scale).

%remove after revision
\rev{
We should also emphasize that our approach
infers constraints that describe the space
of all valid values in the underlying domain 
(enterprise-specific data-types), which can be considered
as a type of ``technical metadata''. In some cases
such data have more specific semantics  (e.g., only 
date-time in 2020 is allowed in this column),
which we feel are hard to infer in an unsupervised manner
and is best for humans to express in a declarative manner using
DSLs like~\cite{breck2019data, schelter2019unit}.
}

\end{comment}


Large-scale evaluations on 
production data suggest that \sj{} produces 
constraints that are substantially more accurate than existing 
methods. Part of this technology ships as an \textsc{Auto-Tag} feature 
in \textsc{Microsoft Azure Purview}~\cite{purview}.%\todo{link}








==> paper - arxiv-full-version/main.tex <==
%!TEX root = main.tex
\input{preamble}

\fancyhead{}

\begin{document}



\iftoggle{fullversion}{}{
% For squeezing
% For margin between figures and between figure and text
\setlength{\floatsep}{0pt}
\setlength{\textfloatsep}{0pt}
% For margin above (or below) figure caption
\setlength{\abovecaptionskip}{0pt}
% For margin around math environment
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
% For margin between itemize items
\setlength{\itemsep}{0pt}
% For first item and top
\setlength{\partopsep}{0pt}
}

%\pagenumbering{arabic}
\pagenumbering{gobble}

%\title{Auto-Regex: Automate Data Validation \\ Using By-Example Inference of Domain Patterns}
\title{Auto-Validate: Unsupervised Data Validation \\ Using Data-Domain Patterns Inferred from Data Lakes}

\author{Jie Song}
\authornote{Work done at Microsoft Research.}
\affiliation{\institution{University of Michigan}}
\email{jiesongk@umich.edu}

\author{Yeye He}
\affiliation{\institution{Microsoft Research}}
\email{yeyehe@microsoft.com}




\begin{abstract}
Complex data pipelines are increasingly common
in diverse applications such as BI reporting and
ML modeling. These pipelines 
often recur regularly (e.g., daily or weekly), 
as BI reports need to be refreshed, 
and ML models need to be retrained. However, it is
widely reported that in complex production
pipelines, upstream data feeds can change in 
unexpected ways, causing downstream applications 
to break silently that are expensive to resolve.

Data validation has thus become an important topic,
as evidenced by notable recent efforts from Google and Amazon,
where the objective is to catch data quality 
issues early as they arise in the pipelines.
Our experience on production data suggests, however, 
that on string-valued data, these existing approaches yield high
false-positive rates and frequently require human intervention.
In this work, we develop a corpus-driven approach to
auto-validate \emph{machine-generated data} by
inferring suitable data-validation ``patterns''
that accurately describe the underlying data-domain,
which minimizes false-positives while
maximizing data quality issues caught.
%to automate data validation, by leveraging a large corpus of data
%where the objective is to minimize false-positive 
%detection (on data from the same domain
%that will arrive in the future in the pipeline), while maximizing
%data quality issues that can be detected.
Evaluations using production
data from real data lakes
suggest that \sj{} is substantially more effective
than existing methods. Part of this 
technology ships as 
an \textsc{Auto-Tag} feature in \textsc{Microsoft Azure Purview}.
\end{abstract}

%\input{response-letter}
\maketitle

\input{introduction}
%\input{architecture}
%\input{pattern}
\input{auto-validate}
\input{auto-validate-vertical}
\input{auto-validate-horizontal}
\input{experiments}
\input{related}
\input{conclusions}

\clearpage

%\appendix 
%\input{appendix}

%\vspace{-2mm}

\balance
\bibliographystyle{abbrv}
{%\Large
\bibliography{auto-validate}
}

%\balancecolumns

%\iftoggle{fullversion}{\input{appendix}}{}
\end{document}


==> paper - arxiv-full-version/pattern.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Preliminary: Pattern Language}

TBD



==> paper - arxiv-full-version/related.tex <==
%!TEX root = main.tex
%\vspace{-3mm}
\section{Related Works}
\label{sec:related}

\hspace{3mm}\textbf{Data Validation.}
%Complex data pipelines are
%increasingly common. The dynamic nature of the 
%pipelines makes data validation important.
Notable recent efforts on data validation include
Google's TensorFlow Data 
Validation (TFDV)~\cite{breck2019data, TFDV} and
Amazon's Deequ~\cite{Deequ, schelter2018automating}.
These offerings allow developers to
write declarative data quality constraints to
describe how ``normal'' data should look like, which 
are described in detail in the introduction.
% so that
%any unexpected deviation can be caught 
%and addressed early. These efforts significantly improve
%over ad-hoc validation scripts and are shown to 
%be beneficial~\cite{breck2019data, 
%schelter2018automating}.

%We note that similar features are also found in enterprise software. For
%instance, Informatica allows users to program Data Quality 
%Rules~\cite{Informatica-DQ-rules} on data, 
%and raise alerts when the 
%rules are violated.
%}%iftoggle

\textbf{Error Detection.} There is an influential line of 
work on error-detection, including methods that focus on 
\textit{multi-column} dependencies, such as
FDs and denial constraints
(e.g.,~\cite{berti2018discovery, chiang2008discovering, chu2013,
dasu2002mining, golab2010data,  ilyas2004cords, kivinen1995approximate, yancoded}), where most techniques would require some amount
of human supervision (e.g., manually specified/verified constraints).
\sj{} is \textit{unsupervised}
and focuses on \textit{single-column} constraints, 
which naturally complements existing work.

Recent approaches propose learning-based error-detection
methods (e.g.,~\cite{heidari2019holodetect, huang2018auto, liu2020picket,
mahdavi2019raha, qahtan2019anmat, yan2020scoded, wang2019uni}), some of which are unsupervised~\cite{huang2018auto, liu2020picket, wang2019uni} and similar in spirit to \sj. 

%As pointed by prior work on data
% validation~\cite{breck2019data, Deequ, 
%schelter2018automating}, however, most of these algorithms 
%are not directly suited for data-validation, because they typically
%perform complex inference, which are difficult for developers to
%program and are often too costly to scale to 
%all production pipelines. \\

\textbf{Pattern Profiling.}
There is also a long line of work on pattern profiling,
including pioneering methods such as
Potter's wheel~\cite{raman2001potter} that leverages
the MDL principle, and other
related techniques~\cite{ilyas2018extracting, fisher2005pads, 
fisher2008dirt, naumann2014data}.  
%Variants of such profiling 
%methods are popular today, some of which 
%are implemented in Microsoft SQL 
%Server SSIS~\cite{ssis-profiling}, 
%Trifacta~\cite{trifacta-profiling}, 
%Ataccama~\cite{ataccama}, etc.
While both data validation 
and profiling produce patterns, data profiling
only aims to produce patterns
to ``cover'' given values in a column $C$, without
considering valid values from the same domain but not in 
$C$, and is thus prone to false-positives when used for 
data validation (for data that arrive in the future).
\nocite{chen2016metric, das2014clusterjoin}

\textbf{Other forms to validation.} 
While pattern-based validation is a natural fit for machine-generated data;
alternative forms of validation logic can be more suited for other 
types of data. For example, for natural-language data drawn from 
a fixed vocabulary (e.g., countries or airport-codes), 
dictionary-based validation learned from examples (e.g., set expansion~\cite{he2011seisa, pantel2009web, wang2007language}) 
is applicable. For complex types, semantic-type validation~\cite{hulsebos2019sherlock, 
yan2018synthesizing, zhang2019sato} is also a suitable choice.










==> paper - arxiv-full-version/response-letter.tex <==
%!TEX root = main.tex

\begin{center}
%\vspace{-12mm}
    {\LARGE Revision for SIGMOD'21: Auto-Validate: Validate Data Using Inferred Data Domain Patterns}
\end{center}

We would like to thank all reviewers for their constructive feedback. 
We believe addressing these comments indeed improves our paper.


%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Comments by Reviewer 1}}
%\vspace{-3mm}

\bigskip
\begin{tcolorbox}
\textbf{O1: Data homogeneity is assumed, which simplifies the detection problem, and focuses the domain on machine-generated data. This limits attributes to date/time, ids, status, etc. and would not cover more interesting data such as customer addresses, suffixes/prefixes in diseases, with much broader domains. How can the model be extended to cover these more interesting cases?}
\end{tcolorbox}


\stitle{Response.} 
This is a good point worth more discussion. The reviewer is
correct that the proposed approach
indeed focuses on machine-generated data, where homogeneity 
will likely hold (because in such cases values are 
generated by the same underling program). This 
approach we propose would indeed not
cover more difficult domains with natural-language-like data values,
such as customer addresses and disease names,
which may not have rigid patterns with strong regularity.

This raises an interesting questions like how often do
data homogeneity hold, and for
what fraction of real data in data lakes our
proposed approaches are applicable. 
To answer these questions, during
revision we have performed a quantitative analysis of real data
lakes under study. %(one from a large technology company referred
%to as ``Enterprise'', and
%one from a large government referred to as ``Government''). 
Specifically, we sampled 1000 data columns
from the data lake, and carefully classified each column 
as one of the following three cases: 

\begin{itemize}[leftmargin=*, ,topsep=0pt]
\item[](1) \textbf{\textit{Homogeneous-rigid-patterns}}: Data values in the same column are homogeneous (drawn from the same underlying domain). Furthermore these values are machine-generated, have strong regularity, and can be represented using ``rigid'' data patterns. 
\item[](2) \textbf{\textit{Homogeneous-NL-like}}: Data values in the same column are homogeneous (drawn from the same underlying domain), but 
they are natural-language-like (NL-like), which do not have 
strong regularity and cannot be (easily) represented using 
rigid data patterns. 
\item[](3) \textbf{\textit{Non-homogeneous}}: Data values in the same column are \textit{not} homogeneous because they are not 
from the same domain.
\end{itemize}

Concrete examples for each of these three classes 
can be found in the table below. 



\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_1 =$  \{ ``03/02/2015|OnBooking'', ``06/12/2015|OnBooking'', ``05/11/2015|OnImpressionDelivery'', \ldots \} & 0.676 & $[0.639, 0.711]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_2 =$  \{ ``Bristol Marriott Hotel City Centre'', ``Renaissance Schaumburg Convention Center Hotel'', ``The Ritz-Carlton, Dallas'', \ldots \} & 0.203 & $[0.174, 0.236]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_3 =$ \{ ``adobe reader updates for xp'', ``acrobat software deals'', ``download acrobat reader 8'', ``foxit pdf reader'', \ldots \} & 0.121 & $[0.098, 0.149]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Enterprise'' data lakes.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


\begin{comment}
\begin{table}[h!]
\vspace{-10mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_4 =$  \{ ``cabinetoffice.gov.uk/ndrC48zK'', ``cabinetoffice.gov.uk/j2tX8BmP'', ``cabinetoffice.gov.uk/ZUDH4uCx'', \ldots \} & 0.429 & $[0.391, 0.468]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_5 =$  \{ ``25a Eccleston Street'',  ``37 Liverpool Road South'', ``Centre for Enterprise Unit 2'', ``Unit E2 Southglade Business Park'', \ldots \} & 0.565 \todo{check} & $[0.526,0.603]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_6 =$  \{ ``british social attitudes survey'', ``vehicle license data'', ``social care survey england 2011 final'', \ldots \}  & 0.06 & $[0.002,0.016]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Government'' data lakes.}
\vspace{-2mm}
\label{tab:government-survey}
\end{table}
\end{comment}


$\bullet$ For (1) ``Homogeneous-rigid-patterns'', 
column $C_1$ %and $C_4$ 
in the table above shows a real example
column, which is machine-generated and homogeneous,
making it amenable to pattern-based representations.
(Many more such examples can be found in Figure~\ref{fig:domain-example}
of our paper).

Our analysis in the data lakes suggest that such machine-generated
data is the majority class in the Enterprise data lake -- out of 1000
sampled columns, 676 are in this class, which is 
a clear majority. We estimate that on the
7M column corpus, the relative frequency of
this class to be [0.639, 0.711] (with a 95\% 
confidence interval)\footnote{We
suspect that this fraction is likely to be higher in
other enterprise data lakes, because our 
data lake serves as the back-end for a commercial
search engine, which has to deal with large volumes of 
unstructured user queries that are not homogeneous.},
implying that there are at least 4M columns in this class,
for which our proposed Auto-Validate is applicable. 
We believe this is a significant number that underscores the prevalence of homogeneous data in data 
lakes, and the relevance of our
approach. (The prevalence of machine-generated
data can be attributed to the fact that machines are
much more productive at churning out 
large quantities of data than humans, 
which is perhaps not very surprising in retrospect).


\begin{comment}
In the case of the Government data lake, we see many more
manually edited CSVs from government agencies, and a smaller
fraction of data that are machine generated -- out of 1000 sampled
columns 429 are in this class, which nevertheless is still a significant
number.
\end{comment}

We added findings from this quantitative analysis in \rev{Section 2} of our paper to highlight the importance and generality of 
our method in the context of enterprise data lakes.


$\bullet$ For (2) ``Homogeneous-NL-like'', column $C_2$
% and $C_5$ 
shows a real example. These values are considered
as homogeneous, because they come from the
same underlying domain of
``hotel names''. (The reviewer's example of 
addresses and disease names would also fall in the same class). 
% for $C_2$, and ``street names'' for $C_5$). 
These values are natural-language-like, and thus
do not share a strong structural regularity -- 
e.g., while values in $C_2$ are all hotel names, ones
like ``The Ritz-Carlton, Dallas'' may not
mention the token ``hotel'',
and furthermore there are many lesser-known names that 
are difficult for even a human to tell whether they are 
really hotel names or not.

Given the ad-hoc nature of such natural-language-like data,
and the fact that even humans frequently cannot be
sure about whether a value $v$ should belong to a class $C$
(e.g., hotel names),
we suspect that it would be no easier for 
machines to reason about, 
especially in an automated and unsupervised manner
(no labeled examples or human intervention), as is
required by our at-scale data-lake settings.

Because of these considerations, and the fact that
pattern-based approaches are unlikely to be a good 
fit for NL-like content (drastically different approaches like
NLP-based methods may be required instead),
we emphasize from the start 
(in Abstract, Section 1 and Section 2) that 
the focus in this work 
is specifically on \textit{machine-generated data},
which accounts for a majority number of 
columns in enterprise data lakes.

Even though this class of ``Homogeneous-NL-like'' 
only accounts for around 20\% of enterprise columns,
this is nevertheless an interesting area of future work
that can complement nicely to
our approach, by addressing an orthogonal type of 
data columns. We added this interesting direction to the
future work section \rev{Section 7}.



$\bullet$ For (3) ``Non-homogeneous'': it is 
encouraging to see this class is 
not common in data lakes (the example in 
column $C_3$ shows heterogeneous 
user queries from a search engine),
confirming the prevalence of homogeneous
machine-generated data in enterprise data lakes.


\begin{tcolorbox}
\textbf{O2: What details can be provided on the ``in-house'' implementation to generate patterns based on a given hierarchy? This was rather unsatisfying given the complexity to generate a set of patterns, such details should be given}
\end{tcolorbox}



\stitle{Response.} 
Thank you for the suggestion. We added a sketch of 
the pattern-generation step in \rev{Section 2}. More
details including pseudo-code of this step is available
 in a full version of our paper~\cite{full}
(to be released on arXiv, and shared for reviewers to 
inspect~\footnote{\url{https://www.dropbox.com/sh/b2u39qha8o83zos/AACZPQ5jUDFwgCuFgGdc0oFsa?dl=0}}).


\begin{tcolorbox}
\textbf{O3: The ideas presented are relatively simple and the problem statement focuses on a constrained optimization problem. Tuning and setting the parameters r, and m is necessarily important given their significance in the problem statement. However, no guidelines are given in this direction.}
\end{tcolorbox}


\stitle{Response.} 
It would indeed be useful to discuss recommended 
settings for r and m,
and for that purpose we have a detailed sensitivity analysis in \rev{Figure~\ref{fig:sensitivity}} (a)(b). 
Our observation on various corpora 
is that the proposed FMDV-VH variant
(the blue lines) is not sensitive to
$r$ with $r \geq 0.02$, and not at all sensitive to different values 
of $m$. Our guideline is to use r=0.05 and m=100, which would be
safe choices in practice.

We have added these guidelines
in \rev{Section 5} of the revised paper.



\begin{tcolorbox}
\textbf{O4: The problem and proposed validation patterns appear to share strong similarity to recently proposed pattern functional dependencies. How are they different and why can't PFDs be used here?
\\ 
Qahtan et. al., Pattern Functional Dependencies for Data Cleaning
VLDB 2020.}
\end{tcolorbox}


\stitle{Response.} 
The reviewer is correct that PFD, which is an interesting
variant of FD, also leverages patterns. We have clarified in our paper
(\rev{Section 5 and Section 6}) the key differences between PFD and our
approach. These differences can be summarized as follows:

(1) A key difference between Auto-Validate 
and FD/PFD, 
is how the techniques are intended to be used. 
In Auto-Validate, the single-column domain constraints
are inferred from \textit{a large corpus of data in data lakes},
which as we showed conceptually and empirically,
are reliable enough to be applied in an 
unsupervised fashion at scale
(e.g., to millions of columns in data lakes), \textit{without 
requiring human intervention}.  In comparison, in the
FD discovery literature, it is known that because the
discovery is based on \textit{one single table 
instance}, discovered FDs are 
typically only ``candidates'' (with frequent false-positives)
that may not hold in a semantic sense 
(e.g., may not hold on data arriving in the 
future)~\cite{berti2018discovery, papenbrock2016hybrid}.

PFD is an extension to FD and is very similar in that 
regard -- it is explained in detail in Section 4.5 
of the PFD paper~\cite{qahtan13pattern} that discovered PFDs  
may not be semantically true, which require humans
to manually verify and select only true PFDs
from discovered candidates. This manual-filtering 
requirement is highlighted again 
in the experiments in Section 5.3 of the paper, which
explains that only
manually verified PFDs
are applied to test data for error-detection.

Because discovered FDs/PFDs require human 
verification and are not intended to be used in an unsupervised
manner, it is hard to scale them to millions of 
tables in data lakes, like AutoValidate does. This 
difference in intended use cases is the first and 
a crucial difference between the two methods.

(2) At a conceptual level, PFD is an extension to FD that 
leverages multi-column constraints, where dependency and
redundancy must exist across multiple columns in a table
for these multi-column approaches to work.
In comparison, Auto-Validate learns single-column constraints
based on the content of a single columns alone. It does not
rely on cross-column data dependency/redundancy, thus 
complementing to the multi-column approaches. 
(There are many scenarios where a 
column can be validated using single-column constraints but 
not multi-column ones, such as tables with only one or two columns, and tables with weak inter-column dependency, etc.).

We will discuss more on the complementary nature
of single- vs. multi-column constraints in our response to O5 below.

(3) Empirically, the fact that single-column constraints in 
Auto-Validate can nicely complement multi-column approaches like
FD/PFD has been validated in our experiments (\rev{Section 5}). 
Out of the 558 columns from the Enterprise benchmark 
that the proposed Auto-Validate can handle, only 247 
(or 44\%) are ``covered''
by PFD (involved in an PFD discovered from the original table instance).
Similarly, out of the 291 columns from the Government benchmark
handled by Auto-Validate, only 167 are involved in an PFD. We should
emphasize that these numbers (247 and 167) are only candidate
PFDs, which as we explained
in (1) above, may not hold in a semantic sense and require
additional human post-filtering,
and are thus likely over-estimates of PFD's true coverage
(we sampled PFDs from our results and indeed 
observed a large fraction of likely false-positives 
from the results).

(4) From a latency's perspective, we
should mention that PFDs can be fairly expensive to 
discover -- in our experiments it takes on average 
$>10$ minutes to process one column
in our enterprise benchmark (compared to 82ms 
per column for Auto-Validate), which can be another
obstacle to scale it to
millions of columns in large data lakes.

We added discussions of these conceptual
differences in the paper, and
we also added new experimental comparisons
with PFD in \rev{Section 5.3} now.

\begin{tcolorbox}
\textbf{O5: Auto-Validate appears to focus on a single column at a time, without considering multi-column correlations.}
\end{tcolorbox}


\stitle{Response.} 
The reviewer is correct that our approach focuses on learning 
and exploiting single-column
constraints, whereas existing work (such as dependency-driven 
data-cleaning) focuses on multi-column constraints (e.g.,
FDs and denial constraints). This highlights the uniqueness 
of our approach relative to the literature, and the fact
that it complements nicely with existing work, 
as we have now discussed in 
\rev{Section 5 and Section 6} of the paper. 

At a conceptual level, 
as our approach is among the first to automatically
learn and exploit single-column constraints, which is 
very different from multi-column constraints (e.g., FDs and denial constraints) used in existing work, it 
makes our approach uniquely positioned
in the context of the large body of existing work. We believe
that learning single-column
constraints is an under-explored area worth
more attention from the community. And we hope 
our work can serve as a springboard for future work
improving our methods in this under-studied space.

At an empirical level, we are also able to show that the single-column
constraints that our approach exploits
nicely complement with the multi-column constraints -- for example, on the enterprise benchmark data, our proposed single-column
approach works for 558 test columns; however, as we
explain in the experiments, out of the 558 columns,
at most 57 can be covered using FD-based 
methods (these columns are involved in an FD on the original table), 
and at most 247 can be covered using PFD-based methods.
We want to emphasize that we use an ``upper-bound'' analysis
for these baseline methods (which is why we say ``at most''), because  it is well known in the literature~\cite{berti2018discovery, papenbrock2016hybrid} that a 
significant fraction of FDs and PFDs
discovered from table instances are likely false-positives that may
not hold in a semantic sense. Nevertheless, this upper-bound
analysis highlights the complementary nature of 
single-column vs. multi-column constrains, and the 
value of exploiting single-column constraints 
studied in this work (which covers a significant fraction of data columns not ``covered'' by multi-column constraints like FDs).



\begin{tcolorbox}
\textbf{O6: The horizontal partitioning version uses a tolerance parameter to allow errors but still inherently assumes a level of homogeneity exists in the domain of C to identify patterns. Given the motivation of the work to address semantic and data drift, one can imagine that the beginnings of such drift would cause deviations from the norm/majority. Under this proposed horizontal partitioning, such values (which are not wrong nor dirty) would be removed, and never
identified.}
\end{tcolorbox}


\stitle{Response.} 
It is true that when data begins to drift, and when the drift is still
``minor'', our approach may not trigger,
because it consciously trades off recall for very high
precision. Recall that in our intended use case
high precision is crucial, because learned constraints are
applied at-scale to millions of columns without human
verification (a lower precision will likely overwhelm
human operators with false-alarms).

We should also mention that this 
desired level of sensitivity and the desired trade-off 
between precision/rcall is entirely 
customizable through the tolerance parameter.

We have added discussions in \rev{Section 4} to further 
clarify this design consideration.


\begin{tcolorbox}
\textbf{O7: In the evaluation, I found Figure~\ref{fig:sensitivity} to be difficult to read and to differentiate among the techniques and their parameter values when used as symbols. I would suggest separating the precision and recall graphs.}
\end{tcolorbox}


\stitle{Response.} 
We have separated precision and recall into two
separate graphs in \rev{Figure~\ref{fig:sensitivity}}, which should make the graphs more readable.


\begin{tcolorbox}
\textbf{O8: The related work was sparse, especially the error detection and pattern profiling sections.
I would recommend more technical discussion in each of these areas, and how this work is tied to the area of dependency driven data cleaning (where the
evaluation includes an FD based algorithm).}
\end{tcolorbox}


\stitle{Response.} 
As suggested, we have expanded our related work
section (\rev{Section 6}). Regarding dependency driven data cleaning --
in a nutshell, the large body of influential work on 
dependency/constraint-driven data cleaning
primarily focus on \textit{multi-column} dependency
(e.g., FDs or denial constraints),  whereas
our proposed \sj{}  infers \textit{single-column} constraints
from a table corpus, which is orthogonal and 
complements this line of work.
Furthermore, unlike existing dependency-driven methods 
that typically require humans verification
(for it is known that constraints discovered automatically 
from table instances may not always hold semantically~\cite{berti2018discovery, papenbrock2016hybrid}), 
our unsupervised approach infers accurate
single-column constraints that can be directly applied 
at scale (e.g., millions of columns) without requiring human validation.






\bigskip
{\huge \stitle{Response to Comments by Reviewer 2}}

\bigskip
\begin{tcolorbox}
\textbf{O1. More justifications could improve the technical depth. FMDV-H is considered NP-hard using a reduction from the independent set problem. A more detailed proof could be provided. Time complexity is O(T.P(D)) but P(D) is constrained by the choice of $\tau$, which is not explained/justified. This parameter limits the pattern enumeration in off-line indexing to columns of at most $\tau$ and it is critical. Statistical tests in Section 4 are chosen without a clear justification, whereas other tests of homogeneity (e.g., chi-square) could be used. Why?}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$  As suggested, we added a proof of NP-hardness in \rev{Section 4}.

$\bullet$ The parameter $\tau$ is indeed important as it motivates the Horizontal-cut algorithm (Section 3), and was described a few pages earlier in Section 2.4 (offline stage), and then in more detail Section 3. We realize that the ``time complexity'' section at the end of Section 4 (for the entire algorithm end-to-end with both Horizontal and Vertical cuts) also makes references to this $\tau$ that was introduced a few sections earlier, making it hard to refer back. We thank the reviewer for pointing this out, and have revised this part in \rev{Section 4} to explicitly 
reference relevant discussions of $\tau$ in earlier sections. (We tried to bring the time-complexity section closer to where $\tau$ is first described, which however turned out to be difficult, because the time-complexity is for the overall algorithm with both vertical-cuts and horizontal-cuts, which is only natural to come at the end of Section 4).  

We should also mention here that in addition to the analytical analysis, we have an encouraging sensitivity analysis on $\tau$ (Figure~\ref{fig:sensitivity_to_index_tau}) that shows a smaller
$\tau$ has little impact on result quality (the blue line for
FMDV-VH), thus allowing us to bound the complexity/cost
without sacrificing quality.

$\bullet$ Other tests of homogeneity can indeed be used, like the Chi-Squared test mentioned by the reviewer. We did already discuss this test, and experimentally compared with it in our paper (\rev{Section 4}), which showed no difference in result quality. We have highlighted it more in the paper to make it more visible.



\bigskip
\begin{tcolorbox}
\textbf{O2. The assumption that the data set contains homogeneous values drawn from the same underlying domain is a strong assumption (not so realistic) and the relaxation of this assumption claimed by the authors is not clear from the basic-version of Auto-Validate (section 2, Eq. (4)) to the more advanced variants (Section 4, Eq. (11)). Could the authors explain and demonstrate this effectiveness across domains? e.g. from Enterprise to Gov benchmarks for example ?}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$ We fully agree with the reviewer that the
kind of data we commonly encounter in our 
everyday life (e.g., csv and
spreadsheet files that humans manually create)
is indeed messy, and we as data researchers have
come to expect data to be messy/heterogeneous.
However, we want to highlight the perhaps counter-intuitive 
fact that because our setting is in
large enterprise data lakes with millions of 
tables, the vast majority of data in question
is \textit{machine-generated} (i.e., values in the same column
are generated by the same underlying program),
as opposed to manually created (which is indeed
more error-prone and less homogeneous).
%Given the scale of our data, this is perhaps not that 
%surprising in retrospect, because 
%machines are, after all, much productive in churning
%out data in volume than humans.

Given the context that data is typically ``machine generating''
in enterprise data lakes, it is then perhaps not 
entirely surprising that we find data in data lakes
to be more homogeneous than one may expected 
-- as we describe in detail
in our \rev{response to the O1 of Reviewer-1}, we have performed
an quantitative analysis of data in our data lakes, by sampling
1000 random columns and manually judging whether each is
homogeneous or not (we copy the result table below 
for ease of reference). Our analysis suggests that
879 columns out of the 1000 are deemed homogeneous, within
which 76.9\% (676 out of 879 columns) 
are clearly machine-generated as they have
rigid data-patterns \footnote{We
suspect that this fraction is likely to be higher in
other enterprise data lakes, because our 
data lake serves as the back-end for a commercial
search engine, which has to deal with large volumes of 
unstructured user queries that are likely ``non-homogeneous''.}. 


\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_1 =$  \{ ``03/02/2015|OnBooking'', ``06/12/2015|OnBooking'', ``05/11/2015|OnImpressionDelivery'', \ldots \} & 0.676 & $[0.639, 0.711]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_2 =$  \{ ``Bristol Marriott Hotel City Centre'', ``Renaissance Schaumburg Convention Center Hotel'', ``The Ritz-Carlton, Dallas'', \ldots \} & 0.203 & $[0.174, 0.236]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_3 =$ \{ ``adobe reader updates for xp'', ``acrobat software deals'', ``download acrobat reader 8'', ``foxit pdf reader'', \ldots \} & 0.121 & $[0.098, 0.149]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Enterprise'' data lakes.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


We believe
these are significant numbers and show the general applicability
of our technique, given that there are millions of columns at
stake in our data lake alone 
and our technique can apply to a majority of 
those cases. Since this technology is being released 
as a feature in a cloud-based enterprise data-lake product
in Jan 2021, and applied to many
other large enterprise data lakes, 
the potential impact will likely multiply.





$\bullet$ The reviewer is correct that homogeneity in
the basic-version of Auto-Validate (Section 2, Eq. (4)),
is indeed relaxed later in Section 4 for Horizontal-cut, as
explained in the paper. However, Eqn (11) pointed out 
in the comment is actually in Section 3 and
for a different variant called Vertical-cut, 
which as a result would not 
relax homogeneity, as the reviewer rightly
observed. We ask the reviewer to kindly
compare Eqn (5-7) in Section 2 with Eqn (12-16) in Section 4
instead, which should better show this relaxation (specifically 
in Eqn 16). We have clarified this more in \rev{Section 2
and Section 4} of the paper.

$\bullet$ Our experiments indeed try to demonstrate 
effectiveness across domains -- specifically, we used 
two benchmarks taken from two very different domains: 
one from a real Enterprise data lake, and one from a 
Government data repository. Our results show
that our proposed FMDV-VH algorithm 
is significantly better than both our own 
basic version (without Horizontal/Vertical-cuts), 
and all other baselines we experimented with. 

In the revision we added statistical tests 
in \rev{Section 5} to demonstrate
that these observed performance advantages are both
(1) statistically significant, and (2) the ``effect size'' of
the new algorithm is
``large'' in a statistical sense. These relate to D4 and D5
below, and we ask the reviewer to kindly refer to our
responses below for more information on the experimental
comparisons in different domains.


\bigskip
\begin{tcolorbox}
\textbf{O3. In terms of experiments, the setup is confusing. Some important details are omitted. Because of impractically large numbers of patterns, there are
omissions in the indexing and it is not clear whether these omissions are considered in the precision/recall measures (see other comments D4-D8).}
\end{tcolorbox}

\stitle{Response.} 
We have clarified  in \rev{Section 5} that the effect of omitting patterns is indeed already captured in our precision/recall evaluation – if for some column a suitable validation pattern is not generated 
by our algorithm (due to omissions in our 
indexing step), then we would either: (1) generate overly-generic
patterns that fail to catch quality issues tested, which would lead
to recall loss, or (2) generate overly-restrictive patterns
that produce false-alarms on correct data values, which
would lead to precision loss. Both of these two situations
are indeed already accounted for in our evaluation. 

(For other comments D4-D8 we will respond to them separately below).


\bigskip
\begin{tcolorbox}
\textbf{D1. Lemma 1 should be justified.}
\end{tcolorbox}

\stitle{Response.}  We have added a sketch of the proof 
to justify Lemma 1 in \rev{Section 2.3} as suggested.



\bigskip
\begin{tcolorbox}
\textbf{D2. Definition (3) is very simple and may not adapted for heterogeneous corpus.}
\end{tcolorbox}

\stitle{Response.} This relates to O1 and O2 above, which we 
have addressed in our responses above and 
in relevant sections of the paper. 

Briefly, we show in our response to O2
that we observe through a quantitative analysis that 
a majority of columns in large enterprise data lakes 
have machine-generated homogeneous values, making 
heterogeneity less of a problem in our setting.

For the minority of columns where
homogeneity does not apply, we should emphasize that:
(1) our technique will
pass on such columns (for no patterns can be generated), thus
not producing false-positives; and (2) more importantly, 
because no  patterns can be generated for the 
non-homogeneous columns even in the indexing step, 
they will not ``pollute'' our
signals for the homogeneous ones and would not 
affect our results on the majority cases where the 
technique does apply. 

Relating to our response to O1, the homogeneity
assumption in the basic version is also 
relaxed in our 
Horizontal-cut variant, which is shown to be 
effective (Figure~\ref{fig:accuracy}). 

We have added these discussions in our paper,
and we ask the reviewer
to kindly refer to our responses to O1 and O2 above 
for more detailed answers.


\bigskip
\begin{tcolorbox}
\textbf{D3. Figure 11 legend is incomplete (red diamond symbol has no name).}
\end{tcolorbox}

\stitle{Response.} The legend on this figure was 
made into a non-standard format with names first, followed
by symbols/markers, which made it appear as if the
last symbol (red diamond) has no name. We have fixed
the legend on \rev{Figure 11} to make it more standard using symbols first, followed by names, which should now avoid
this confusion.



\bigskip
\begin{tcolorbox}
\textbf{D4. The evaluation methodology in Section 5.1 does not detail the number of iterations (runs) of the randomized selection of the 1000 columns. As such,
this process should be re-iterated at least 10 times to account for randomization. It is not clear that the results in terms of precision, recall, F1 are averaged.
However, if this is the case, the results in Section 5.3 could mention the averages with their respective standard deviations (e.g., in Table 2 and Figure 10,
11, and 12). This would also tell us whether the main assumption made by the authors (i.e., values are homogeneous across columns in machine-generated
data) is realistic or not and if Eq. (4) is not too simplistic.}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$ Our precision and recall scores
are indeed averaged over 1000 randomly selected
columns from the corpus. We have clarified this
and added standard deviations to Table 2, and in relevant
discussions in \rev{Section 5}.\footnote{Figure 11 is a drill-down of Figure 10 
with a case-by-case analysis, where no separate 
standard deviations can be reported and the same from
Figure 10 applies.}

$\bullet$  Regarding the homogeneity assumption for 
machine-generated data, we have responded
to the related comment O2 above in more detail (using
a quantitative analysis of 1000 sampled 
columns). As a brief summary, homogeneity is observed 
to hold for a majority of columns in 
data lakes in practice, 
for which our technique provides clear value in 
terms of automated validation as shown in our
experiments. For the minority of columns where
homogeneity does not apply, we should emphasize that:
(1) our technique will
pass on such columns (for no patterns can be generated), thus
not producing false-positives; and (2) more importantly, 
because no  patterns can be generated for the 
non-homogeneous columns even in the indexing step, 
they will not ``pollute'' our
signals for the homogeneous ones and would not 
affect our results on the majority cases where the 
technique does apply.  We ask the reviewer
to kindly refer to our response to O2 for more details.


$\bullet$  Regarding the evaluation of our results, 
we added more details to \rev{Section 5} of our paper.
We treat the precision/recall/F-score result of an algorithm $A$ 
on a randomly selected column $C$ as a random variable, 
and we perform 1000 randomized trials that 
would sample from this underlying random
variable (using 1000 randomly selected columns).

Using these 1000 randomized trials, we can perform standard
statistical tests, where the null-hypothesis states that FMDV-VH
is no better when compared to an alternative 
baseline $A$, for each baseline we compare with. 
In the following we will report (1) statistical significance, and
(2) effect size, when comparing FMDV-VH with all baselines
using F-scores, which is the harmonic mean of precision and recall.



For statistical significance, as can be seen from the table below,
all $p$-values are in the range of 0.001 to 0.007,
much smaller than the standard threshold of
significance ($p<0.05$), indicating that we should reject the
null hypothesis, showing that
the quality benefit of using our proposed algorithm 
FMDV-VH is significant.



\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |} 
 \hline
 Compare FMDV-VH with:  & FMDV-basic & FMDV-V    & FMDV-H & Grok & XSystem & PWheel & SM-P-P & SM-P-M & SM-I-1 & SM-I-10 & FlashProfile & SSIS & Deequ & DeequDist & TFDV   \\  \hline \hline
Enterprise benchmark & 0.002 & 0.001 & 0.007 & 0 & 0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.001 & 0.001 & 0 & 0.001 & 0  \\ \hline
Government benchmark & 0.001 & 0.001 & 0.007 & 0 & 0.001 & 0 & 0 & 0 & 0 & 0.001 & 0.001 &  NA & NA & NA & NA \\ \hline
\end{tabular}
\caption*{$p$-value for statistical-significance on F-measures, between the proposed FMDV-VH, and all other baselines. We use $p<0.05$ to reject the null hypothesis that FMDV-VH is no better than a baseline. (All comparisons are statistical significant).}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


On top of statistical significance, we test for
``effect size'' using Cohen's d, which measures 
whether the F-score improvements are deemed as ``large''
in a statistical sense. (For Cohen's d, the convention is
to treat an effect-size of $d>0.8$ as large, and $d>1.2$ 
as very large\footnote{\url{https://en.wikipedia.org/wiki/Effect_size\#Cohen\'s_d}}). 
As can be seen from the table below,
most of these improvements over baselines are either ``large''
or ``very large'', showing a clear benefit of our algorithm
when using randomized trials a statistical interpretation.


\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |} 
 \hline
   & FMDV-basic & FMDV-V    & FMDV-H & Grok & XSystem & PWheel & SM-P-P & SM-P-M & SM-I-1 & SM-I-10 & FlashProfile & SSIS & Deequ & DeequDist & TFDV   \\  \hline \hline
Enterprise benchmark & 2.23 & 2.05 & 0.24 & 5.40 & 7.90 & 6.09 & 6.40 & 6.36 & 5.79 & 6.37 & 5.54 & 6.20 & 7.98 & 7.78 & 6.09  \\ \hline
Government benchmark & 1.928 & 1.838 & 0.154 & 2.913 & 4.395 & 4.075 & 4.210 & 4.294 & 4.233 & 4.109 & 2.085 & NA & NA & NA & NA  \\ \hline

\end{tabular}
\caption*{Cohen's $d$ for effect-size, between the proposed FMDV-VH, its different variants, and all other baselines. $d>0.8$ is regard as having large effects.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}

We have summarized our findings and the 
new statistical test results in \rev{Section 5} of the paper.


\bigskip
\begin{tcolorbox}
\textbf{D5. 1000 test cases have been used as ground truth (only for Enterprise data set), which may not be statistically significant as no detail is given on the
selection of these test cases and any potential selection bias in favor of the proposed method.}
\end{tcolorbox}

\stitle{Response.} 
We have clarified in \rev{Section 5} that the 1000 test columns 
are randomly selected from the data lake, 
which should be representative and
give no bias in favor of any method. 

Statistical significance results are discussed in detail
in our response to D4 above. 
We would like to confirm here that 
all comparisons in Figure~\ref{fig:accuracy}
are shown to be statistically significant, 
with $p$-values ranging from 0.001 to 0.007 (where $p<0.05$ 
is typically regarded as significant). We ask the reviewer to 
kindly refer to D4 above for more information.


\bigskip
\begin{tcolorbox}
\textbf{D6. The evaluation experiment consumes 1000 columns among 7.2 M and 628K respectively for Enterprise and Government data sets. The average
numbers of tuples and distinct values (with standard deviations) per data set are not given and it is difficult to have an idea of the heterogeneity of the data
sets.}
\end{tcolorbox}

\stitle{Response.} 
As suggested, we have added these statistics in \rev{Table 1 of Section 5} in our paper. We should clarify that the key homogeneity property our algorithm leverages is with respect to values in the same column (which is shown to hold in practice on a large fraction of data as detailed in our response to O1 of Reviewer-1).
Data tables may exhibit another layer of heterogeneity
in terms of number of rows and
distinct values, etc., which however do not 
pose challenges to the proposed method for pattern inference.


\bigskip
\begin{tcolorbox}
\textbf{D7. It is unclear how to set $\tau$ and the other parameters; the figures 12 (a-d) are difficult to read as they are on a very limited ranges for the parameters
and we suppose it is averaged over the two datasets but it is not specified.}
\end{tcolorbox}

\stitle{Response.} 
We have added discussion in \rev{Section 5.3} 
on recommended settings for these parameters
based on observations from the sensitivity analysis. 
It can be seen that the proposed FMDV-VH
(the blue line) is not particularly
sensitive to $m$, $\tau$, and $\theta$, and not
very sensitive to $r$ as long as it is set to a reasonably high
value (e.g., above 0.02).

We have completely redrawn \rev{Figures 12} to make it 
more readable, by separating precision and recall into two
sub-figures. We have also clarified in the figure caption 
that the sensitivity figures
only show results on the Enterprise benchmark
due to space constraints. We thank the reviewer
for these suggestions.


\bigskip
\begin{tcolorbox}
\textbf{D8. It is not clear how AD-UB and FD-UB are implemented and effectively tested as they may suffer from scalability issues.}
\end{tcolorbox}

\stitle{Response.} We have added clarification in \rev{Section 5.2}. For FD-UB, we implemented the
standard FD-discovery and run it on individual test tables. 
For AD-UB, we implemented what is reported in the AD paper~\cite{huang2018auto},
which is already designed for large corpora of tables.
Because both are known methods,
they do not pose significant scalability challenges for us.
We should note that unlike AutoValidate which is
required to run at an interactive speed, 
we are only comparing the two baselines
from a quality (precision/recall) perspective, which do not
require us to make the two run at an interactive speed.



\bigskip
\begin{tcolorbox}
\textbf{D9. Eq.(11) is too small}
\end{tcolorbox}

\stitle{Response.} 
We have separate \rev{Eq.(11)} into multiple lines, which should make it more readable now.



\bigskip
\begin{tcolorbox}
\textbf{D10. Non-conforming values like null values can actually be very informative of the heterogeneity for formatting missing values and should be indexed
whereas the authors propose a way to 'cut out' a fraction of the non-conforming values with $\theta$ parameter.}
\end{tcolorbox}

\stitle{Response.}
We thank the reviewer for the interesting suggestion. 
While our approach already shows good quality, 
this is definitely an interesting idea worth exploring in the future.
We added it in the future work \rev{Section 7}.


\bigskip
\begin{tcolorbox}
\textbf{D11. Balance of the paper structure. Please extend the conclusion and reduce the introduction to avoid redundant information.}
\end{tcolorbox}

\stitle{Response.} 
As suggested, we have rewritten parts of the introduction and conclusion sections to optimize the structure of  the paper.













\bigskip
{\huge \stitle{Response to Comments by Reviewer 3}}

\bigskip
\begin{tcolorbox}
\textbf{O1: In the ``Time Complexity'' subsection, it is explained that the offline step has a complexity that depends on the size of the full corpus (which is assumed
to be very large) multiplied by the number of patterns that can be generated for each column (exponential in the number of tokens contained by the column).
This is potentially an extremely large value.
Throughout the paper, little attention is paid to the cost of the required operations. Authors should clarify:
How was the corpus of patterns generated? How big was the cluster used to produce the index? What’s the effect of tau on the execution time? How often
does the index need to be updated?
Some examples of the number of patterns and segmentations encountered during the experimental section would help with having an idea of the cost of the
solution in a realistic situation. A study of the overall time required by the different algorithms would similarly be useful to provide additional context.
It is currently hard to understand how the system would perform in a small-scale environment that cannot rely on production-grade clusters.}
\end{tcolorbox}

\stitle{Response.} 
This is a great suggestions. We added discussions 
on the cost aspect in \rev{Section 5}
of our paper. Overall we are happy to report 
that our algorithms are expected to work fine on 
small-scale clusters. Specifically, although our jobs
were run on a production-scale cluster, 
our particular experiment reported in the paper with
7M columns finishes 
in under 3 hours end-to-end using only 10 “virtual nodes”.
Like other systems, our job scheduler 
dynamically assigns each job to an 
appropriate number of “virtual nodes” based on 
the job’s estimated cost, and 10 is estimated to
be (and indeed is) adequate for our indexing job.
Because each virtual-node in our system 
is wimpy (many virtual-nodes are packed into one
VM, with each node having a fraction of the resources in the VM),
we fully expect a job like ours to run without problem 
on small-scale clusters (less than 10 machines).

To provide additional details in response to the questions
raised: 

$\bullet$ The offline pattern generation step is indeed relevant,
for which we have added discussions in \rev{Section 2.1}
and \rev{Section 2.4} to better explain the steps involved.
The key insight is that while a brute-force enumeration
is indeed expensive, our approach 
avoids exhaustive enumeration in the offline
step by enumerating only patterns of length up to $\tau$
without affecting quality, 
because our Vertical-cut algorithm (Section 3) 
uses dynamic-programming that can piece together
sub-patterns into longer patterns at online query time.

$\bullet$ From a large table corpus, after pattern summarization
and aggregation ({Section 2.4}), our index is about 
900MB in size, with 6.2M entries (unique pattern candidates),
which is many orders of magnitude smaller than the raw
data. (More statistics on the patterns encountered/summarized
can be found in a full version of the paper~\cite{full}, which is
shared\footnote{\url{https://www.dropbox.com/sh/b2u39qha8o83zos/AACZPQ5jUDFwgCuFgGdc0oFsa?dl=0}} for the reviewer to inspect.).

$\bullet$ Changing $\tau$ from 8 to 13 increases the indexing job
from around 1 hour to 3 hours, which however produces no
significant increase in result quality. We recommend
to use $\tau = 8$ as a result. These are added to \rev{Section 5}.

$\bullet$ In one of our sensitivity study (not included
in the paper due to the space constraint), we use data corpus from
6 month ago as the ``training'' data for AutoValidate, 
and use ``test'' data
generated 6 months after as query columns. The result
quality is still high and we did not see significant 
drop in quality.
This we believe shows that the domain definitions 
of the underlying data 
do not change rapidly, making us to believe
that it is sufficient to re-run 
the indexing job once in a few months. 

\bigskip
\begin{tcolorbox}
\textbf{O2: AutoValidate works only on homogeneous columns (as they can be described through patterns), so free text columns must be excluded. The fact that AutoValidate cannot handle free text does not diminish the contribution, however this limitation should be clarified more from the start (abstract for sure -
even in the title?), while right now it is mentioned only briefly in the introduction and in a sentence in the experimental section (where initially it's claimed 1k
columns, but it's not the case).}
\end{tcolorbox}

\stitle{Response.} 
This is a great suggestion. We have now emphasized this 
point more in
the \rev{Abstract}, and re-iterated it in a few places in 
our introduction in 
\rev{Section 1}, so that readers can better understand 
that machine-generated homogeneous data is the 
focus of our work from the start.

\bigskip
\begin{tcolorbox}
\textbf{O3: The experimental study can be improved by reporting some results over the columns that are not handled by the proposed solution. Those are about
40\% and AutoValidate has 0 on those - what about the baselines? I am not suggesting this to raise an issue with the proposed system, but it would be fair to
give a feeling on what other do in a setting where this solution fails completely.
For example, users are asked to create regular expressions to describe a column taken from those that AutoValidate can handle. These regex are then
compared to what AutoValidate produces in its querying step. It is expected that a computer system would be many times faster at producing a result in
such conditions, but it is also true that the users may can up with much more expressive checks (see also O4).}
\end{tcolorbox}

\stitle{Response.} It is true that users can write more
expressive checks such as more specific regex based on 
their semantic understanding of the data expected in a column,
which is indeed not something that AutoValidate is intended
to support,
and is likely challenging for any unsupervised methods
(please kindly refer to O4 below for a more detailed response on this aspect).

We indeed performed an analysis of the 40\%
cases where AutoValidate does not handle.
The majority of the cases are the data columns that
our approach is not expected to handle, including
natural-language-like content 
(e.g., company-names, people-names), and
non-homogeneous columns 
(e.g., mixed search engine queries).  In both of these cases,
regex is likely not the right representation to capture the
underlying domain.  In our response to
\rev{O1 of Reviewer-1} we gave a detailed analysis of
the underlying data lake --  
we sampled 1000 columns and manually analyzed the characteristics of each column, and found that 32\% of the cases
are either homogeneous-but-natural-language-like, or
non-homogeneous, for which we would not expect any
pattern-based approach (including AutoValidate and other 
baselines compared in the paper) to handle. 
We ask the reviewer to kindly refer
to O1 of Reviewer-1 for more details of the analysis.

For the remaining cases (less than 10\%) 
where a ground-truth regex pattern
does exist and our approach fails to find the optimal pattern,
we found the main reason to be 
the lack of support for advanced pattern constructs, such as 
union of multiple patterns, and flexibly-formatted URLs, 
in our current profiler/pattern-language.

We have added this error analysis in \rev{Section 5.3} as
suggested.


\bigskip
\begin{tcolorbox}
\textbf{O4: If I understand correctly, given a query column that contains only data values starting on January 2020, the system will infer a date pattern. However,
the correct rule is the one with year equals to 2020 as those are covid 19 cases. Unfortunately, incorrect dates with 2018 are not detected by the pattern.
This issue does not seem to be captured by your experimental setting but would be a real issue in validation, as incorrect values are validated by the
patterns that you propose. I am not suggesting to improve the language of the patterns here, but to discuss and highlight this aspect (possibly measure it on
a sample of columns?) \\
\\
(From Q12 ``Response to Author Feedback''): Is missing business metadata leading to mistakes or affecting your method? how and how much?}
\end{tcolorbox}

\stitle{Response.}  These are excellent points. Our approach infers what is known as the ``technical metadata'', or the technical definition of all valid values in the underlying data domain (e.g., all valid date strings are considered acceptable for a column from a ``data-type/data-domain'' standpoint, which is a type of technical specification). This contrasts with what is known as the ``business metadata'', which may assign specific business meanings and semantics to each column (e.g., only dates in 2020 are acceptable in this column). The latter is indeed more expressive but is perhaps more difficult to infer from data-values alone, when an unsupervised method is used. This is because a column 
may have date-time values in Jan 2020, but from that alone, it is hard even for a human looking at the
data to know whether the data-owner's intent is
to only allow dates in Jan 2020, in Q1 of 2020, or all months of 2020. We feel that for such more expressive and semantic
checks, humans would need to be in the loop and existing
techniques such as declarative DSL for data-validation 
(e.g.,~\cite{breck2019data, schelter2019unit}) can
be used to complement auto-inferred technical 
data specification produced by our method.

We feel that the distinction on technical vs business metadata is indeed important, which we added in \rev{Section 1} of the paper. 

After reading the reviewer's response to
Q12 in the review (after author feedback), 
we feel that it should be clarified that while missing business
metadata may lead to missed opportunities in
catching certain quality issues, 
it does not lead to false-alarms or ``mistakes'' in a traditional sense (which would be a deal-breaker in our data lake settings).
This is because the technical-metadata is by definition 
broader and more tolerant than the more specific 
business-metadata (e.g., technical-metadata
specifies all valid date-time strings as acceptable,
while business-metadata accepts only date-time in 2020).
As such, without data-owners in-the-loop to provide
more fine-grained and specific metadata, we may miss on some
quality issues (loss of recall), but not trigger false-alarms
(precision is still very high).

The suggestion on 
sample-based human evaluation is also interesting.
However, since we are not data owners, 
it is sometimes a bit difficult
for us to judge in a reliable fashion, because 
by looking at the data-values alone, we may not know
the semantics behind them, or the intended constraints
on the column. We feel that ultimately it 
is up to the data owners
to tell us whether the suggested constraints are useful or not.


Along the line of what is suggested by the review, we
should report that we did
also interview real
data owners in our study, to get a sense of the
overall usefulness of our
algorithms (on top of the large-scale automated
evaluation reported in the paper, which we feel is an 
ideal and robust way for
checking compliance to ``technical metadata/data-types'',
which is the focus of the paper). We ran our
algorithms to infer constraints on real data, and then
use the constraints to catch real data quality issues 
in the data lake. From such issues, 
we sampled 10 cases,
identified the engineering teams that own the relevant datasets,
and interviewed these owners to check whether the suggested issues are indeed an issue, and whether the suggested
constraints make sense to them. (Because this is a fairly expensive
process as each case requires an 1:1 interview that is 
time-consuming for both us and the engineering teams
involved, it cannot scale to larger numbers,
which is why we chose to report the
automated evaluation in the paper).
All the teams surveyed
gave positive feedback, explaining the meanings of 
their data and telling us that 
identified issues are indeed
true data quality issues (though in some cases the data feeds are
stale copies in the lake that are no longer used, and would not
call for an immediate fix to be applied). In one case,
the data owner told us that the constraint is reasonable
but can be made more specific/restrictive given their
business context, which is very similar to what the
reviewer suggested. (Again, this may create
a loss of recall, but would not introduce false-alarms or
``mistakes'' in a traditional sense). Overall, we find such 
specific requirements to be 
difficult for algorithms to infer in an unsupervised
manner (because without a meeting with the data owner,
we as humans would not know). We feel that in such a situation, 
asking data owners to explicitly specify such constraints 
would seem like a more viable approach for now.





\bigskip
\begin{tcolorbox}
\textbf{R1: There are well-known patterns that should appear often in machine-generated data such as dates and IP addresses (this is touched upon in the
experimental section when testing Grok patterns). Is it possible to use these patterns during the pattern enumeration phase to prune bad patterns? Was
such a strategy considered?}
\end{tcolorbox}

\stitle{Response.} This is a very interesting idea. We feel that
using well-known patterns could be a useful 
optimization strategy to prune certain
parts of the search space, and yield additional efficiency
benefits. There may be a small cost to pay
in terms of quality though (e.g., we have seen version-numbers 
like ``1.0.0.1'', and if an IP-pattern is selected too hastily
without a proper search, the result quality may be reduced).
Since our latency for the online part is
already more than sufficient for most interactive uses (i.e. 86ms
per test column), we did not explore in the direction of
efficiency optimization further. Nevertheless this is 
a good suggestion that would at least reduce
offline indexing cost. We thank the reviewer for the
suggestion.



\bigskip
\begin{tcolorbox}
\textbf{R2: the matching approach seems the most promising baseline but it relies on a very simple matching method. I believe a better matching system, such as
those based on deep learning from relational data (e.g., Creating Embeddings of Heterogeneous Relational Datasets for Data Integration Tasks. SIGMOD20), improve the performance.}
\end{tcolorbox}

\stitle{Response.}  This is an excellent suggestion. We have
added discussions in this regard in \rev{Section 5} and also 
a reference to this related work.


==> pattern.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Preliminary: Pattern Language}

TBD



==> response-letter.tex <==
%!TEX root = main.tex

\begin{center}
%\vspace{-12mm}
    {\LARGE Revision for SIGMOD'21: Auto-Validate: Validate Data Using Inferred Data Domain Patterns}
\end{center}

We would like to thank all reviewers for their constructive feedback. 
We believe addressing these comments indeed improves our paper.


%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Comments by Reviewer 1}}
%\vspace{-3mm}

\bigskip
\begin{tcolorbox}
\textbf{O1: Data homogeneity is assumed, which simplifies the detection problem, and focuses the domain on machine-generated data. This limits attributes to date/time, ids, status, etc. and would not cover more interesting data such as customer addresses, suffixes/prefixes in diseases, with much broader domains. How can the model be extended to cover these more interesting cases?}
\end{tcolorbox}


\stitle{Response.} 
This is a good point worth more discussion. The reviewer is
correct that the proposed approach
indeed focuses on machine-generated data, where homogeneity 
will likely hold (because in such cases values are 
generated by the same underling program). This 
approach we propose would indeed not
cover more difficult domains with natural-language-like data values,
such as customer addresses and disease names,
which may not have rigid patterns with strong regularity.

This raises an interesting questions like how often do
data homogeneity hold, and for
what fraction of real data in data lakes our
proposed approaches are applicable. 
To answer these questions, during
revision we have performed a quantitative analysis of real data
lakes under study. %(one from a large technology company referred
%to as ``Enterprise'', and
%one from a large government referred to as ``Government''). 
Specifically, we sampled 1000 data columns
from the data lake, and carefully classified each column 
as one of the following three cases: 

\begin{itemize}[leftmargin=*, ,topsep=0pt]
\item[](1) \textbf{\textit{Homogeneous-rigid-patterns}}: Data values in the same column are homogeneous (drawn from the same underlying domain). Furthermore these values are machine-generated, have strong regularity, and can be represented using ``rigid'' data patterns. 
\item[](2) \textbf{\textit{Homogeneous-NL-like}}: Data values in the same column are homogeneous (drawn from the same underlying domain), but 
they are natural-language-like (NL-like), which do not have 
strong regularity and cannot be (easily) represented using 
rigid data patterns. 
\item[](3) \textbf{\textit{Non-homogeneous}}: Data values in the same column are \textit{not} homogeneous because they are not 
from the same domain.
\end{itemize}

Concrete examples for each of these three classes 
can be found in the table below. 



\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_1 =$  \{ ``03/02/2015|OnBooking'', ``06/12/2015|OnBooking'', ``05/11/2015|OnImpressionDelivery'', \ldots \} & 0.676 & $[0.639, 0.711]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_2 =$  \{ ``Bristol Marriott Hotel City Centre'', ``Renaissance Schaumburg Convention Center Hotel'', ``The Ritz-Carlton, Dallas'', \ldots \} & 0.203 & $[0.174, 0.236]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_3 =$ \{ ``adobe reader updates for xp'', ``acrobat software deals'', ``download acrobat reader 8'', ``foxit pdf reader'', \ldots \} & 0.121 & $[0.098, 0.149]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Enterprise'' data lakes.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


\begin{comment}
\begin{table}[h!]
\vspace{-10mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_4 =$  \{ ``cabinetoffice.gov.uk/ndrC48zK'', ``cabinetoffice.gov.uk/j2tX8BmP'', ``cabinetoffice.gov.uk/ZUDH4uCx'', \ldots \} & 0.429 & $[0.391, 0.468]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_5 =$  \{ ``25a Eccleston Street'',  ``37 Liverpool Road South'', ``Centre for Enterprise Unit 2'', ``Unit E2 Southglade Business Park'', \ldots \} & 0.565 \todo{check} & $[0.526,0.603]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_6 =$  \{ ``british social attitudes survey'', ``vehicle license data'', ``social care survey england 2011 final'', \ldots \}  & 0.06 & $[0.002,0.016]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Government'' data lakes.}
\vspace{-2mm}
\label{tab:government-survey}
\end{table}
\end{comment}


$\bullet$ For (1) ``Homogeneous-rigid-patterns'', 
column $C_1$ %and $C_4$ 
in the table above shows a real example
column, which is machine-generated and homogeneous,
making it amenable to pattern-based representations.
(Many more such examples can be found in Figure~\ref{fig:domain-example}
of our paper).

Our analysis in the data lakes suggest that such machine-generated
data is the majority class in the Enterprise data lake -- out of 1000
sampled columns, 676 are in this class, which is 
a clear majority. We estimate that on the
7M column corpus, the relative frequency of
this class to be [0.639, 0.711] (with a 95\% 
confidence interval)\footnote{We
suspect that this fraction is likely to be higher in
other enterprise data lakes, because our 
data lake serves as the back-end for a commercial
search engine, which has to deal with large volumes of 
unstructured user queries that are not homogeneous.},
implying that there are at least 4M columns in this class,
for which our proposed Auto-Validate is applicable. 
We believe this is a significant number that underscores the prevalence of homogeneous data in data 
lakes, and the relevance of our
approach. (The prevalence of machine-generated
data can be attributed to the fact that machines are
much more productive at churning out 
large quantities of data than humans, 
which is perhaps not very surprising in retrospect).


\begin{comment}
In the case of the Government data lake, we see many more
manually edited CSVs from government agencies, and a smaller
fraction of data that are machine generated -- out of 1000 sampled
columns 429 are in this class, which nevertheless is still a significant
number.
\end{comment}

We added findings from this quantitative analysis in \rev{Section 2} of our paper to highlight the importance and generality of 
our method in the context of enterprise data lakes.


$\bullet$ For (2) ``Homogeneous-NL-like'', column $C_2$
% and $C_5$ 
shows a real example. These values are considered
as homogeneous, because they come from the
same underlying domain of
``hotel names''. (The reviewer's example of 
addresses and disease names would also fall in the same class). 
% for $C_2$, and ``street names'' for $C_5$). 
These values are natural-language-like, and thus
do not share a strong structural regularity -- 
e.g., while values in $C_2$ are all hotel names, ones
like ``The Ritz-Carlton, Dallas'' may not
mention the token ``hotel'',
and furthermore there are many lesser-known names that 
are difficult for even a human to tell whether they are 
really hotel names or not.

Given the ad-hoc nature of such natural-language-like data,
and the fact that even humans frequently cannot be
sure about whether a value $v$ should belong to a class $C$
(e.g., hotel names),
we suspect that it would be no easier for 
machines to reason about, 
especially in an automated and unsupervised manner
(no labeled examples or human intervention), as is
required by our at-scale data-lake settings.

Because of these considerations, and the fact that
pattern-based approaches are unlikely to be a good 
fit for NL-like content (drastically different approaches like
NLP-based methods may be required instead),
we emphasize from the start 
(in Abstract, Section 1 and Section 2) that 
the focus in this work 
is specifically on \textit{machine-generated data},
which accounts for a majority number of 
columns in enterprise data lakes.

Even though this class of ``Homogeneous-NL-like'' 
only accounts for around 20\% of enterprise columns,
this is nevertheless an interesting area of future work
that can complement nicely to
our approach, by addressing an orthogonal type of 
data columns. We added this interesting direction to the
future work section \rev{Section 7}.



$\bullet$ For (3) ``Non-homogeneous'': it is 
encouraging to see this class is 
not common in data lakes (the example in 
column $C_3$ shows heterogeneous 
user queries from a search engine),
confirming the prevalence of homogeneous
machine-generated data in enterprise data lakes.


\begin{tcolorbox}
\textbf{O2: What details can be provided on the ``in-house'' implementation to generate patterns based on a given hierarchy? This was rather unsatisfying given the complexity to generate a set of patterns, such details should be given}
\end{tcolorbox}



\stitle{Response.} 
Thank you for the suggestion. We added a sketch of 
the pattern-generation step in \rev{Section 2}. More
details including pseudo-code of this step is available
 in a full version of our paper~\cite{full}
(to be released on arXiv, and shared for reviewers to 
inspect~\footnote{\url{https://www.dropbox.com/sh/b2u39qha8o83zos/AACZPQ5jUDFwgCuFgGdc0oFsa?dl=0}}).


\begin{tcolorbox}
\textbf{O3: The ideas presented are relatively simple and the problem statement focuses on a constrained optimization problem. Tuning and setting the parameters r, and m is necessarily important given their significance in the problem statement. However, no guidelines are given in this direction.}
\end{tcolorbox}


\stitle{Response.} 
It would indeed be useful to discuss recommended 
settings for r and m,
and for that purpose we have a detailed sensitivity analysis in \rev{Figure~\ref{fig:sensitivity}} (a)(b). 
Our observation on various corpora 
is that the proposed FMDV-VH variant
(the blue lines) is not sensitive to
$r$ with $r \geq 0.02$, and not at all sensitive to different values 
of $m$. Our guideline is to use r=0.05 and m=100, which would be
safe choices in practice.

We have added these guidelines
in \rev{Section 5} of the revised paper.



\begin{tcolorbox}
\textbf{O4: The problem and proposed validation patterns appear to share strong similarity to recently proposed pattern functional dependencies. How are they different and why can't PFDs be used here?
\\ 
Qahtan et. al., Pattern Functional Dependencies for Data Cleaning
VLDB 2020.}
\end{tcolorbox}


\stitle{Response.} 
The reviewer is correct that PFD, which is an interesting
variant of FD, also leverages patterns. We have clarified in our paper
(\rev{Section 5 and Section 6}) the key differences between PFD and our
approach. These differences can be summarized as follows:

(1) A key difference between Auto-Validate 
and FD/PFD, 
is how the techniques are intended to be used. 
In Auto-Validate, the single-column domain constraints
are inferred from \textit{a large corpus of data in data lakes},
which as we showed conceptually and empirically,
are reliable enough to be applied in an 
unsupervised fashion at scale
(e.g., to millions of columns in data lakes), \textit{without 
requiring human intervention}.  In comparison, in the
FD discovery literature, it is known that because the
discovery is based on \textit{one single table 
instance}, discovered FDs are 
typically only ``candidates'' (with frequent false-positives)
that may not hold in a semantic sense 
(e.g., may not hold on data arriving in the 
future)~\cite{berti2018discovery, papenbrock2016hybrid}.

PFD is an extension to FD and is very similar in that 
regard -- it is explained in detail in Section 4.5 
of the PFD paper~\cite{qahtan13pattern} that discovered PFDs  
may not be semantically true, which require humans
to manually verify and select only true PFDs
from discovered candidates. This manual-filtering 
requirement is highlighted again 
in the experiments in Section 5.3 of the paper, which
explains that only
manually verified PFDs
are applied to test data for error-detection.

Because discovered FDs/PFDs require human 
verification and are not intended to be used in an unsupervised
manner, it is hard to scale them to millions of 
tables in data lakes, like AutoValidate does. This 
difference in intended use cases is the first and 
a crucial difference between the two methods.

(2) At a conceptual level, PFD is an extension to FD that 
leverages multi-column constraints, where dependency and
redundancy must exist across multiple columns in a table
for these multi-column approaches to work.
In comparison, Auto-Validate learns single-column constraints
based on the content of a single columns alone. It does not
rely on cross-column data dependency/redundancy, thus 
complementing to the multi-column approaches. 
(There are many scenarios where a 
column can be validated using single-column constraints but 
not multi-column ones, such as tables with only one or two columns, and tables with weak inter-column dependency, etc.).

We will discuss more on the complementary nature
of single- vs. multi-column constraints in our response to O5 below.

(3) Empirically, the fact that single-column constraints in 
Auto-Validate can nicely complement multi-column approaches like
FD/PFD has been validated in our experiments (\rev{Section 5}). 
Out of the 558 columns from the Enterprise benchmark 
that the proposed Auto-Validate can handle, only 247 
(or 44\%) are ``covered''
by PFD (involved in an PFD discovered from the original table instance).
Similarly, out of the 291 columns from the Government benchmark
handled by Auto-Validate, only 167 are involved in an PFD. We should
emphasize that these numbers (247 and 167) are only candidate
PFDs, which as we explained
in (1) above, may not hold in a semantic sense and require
additional human post-filtering,
and are thus likely over-estimates of PFD's true coverage
(we sampled PFDs from our results and indeed 
observed a large fraction of likely false-positives 
from the results).

(4) From a latency's perspective, we
should mention that PFDs can be fairly expensive to 
discover -- in our experiments it takes on average 
$>10$ minutes to process one column
in our enterprise benchmark (compared to 82ms 
per column for Auto-Validate), which can be another
obstacle to scale it to
millions of columns in large data lakes.

We added discussions of these conceptual
differences in the paper, and
we also added new experimental comparisons
with PFD in \rev{Section 5.3} now.

\begin{tcolorbox}
\textbf{O5: Auto-Validate appears to focus on a single column at a time, without considering multi-column correlations.}
\end{tcolorbox}


\stitle{Response.} 
The reviewer is correct that our approach focuses on learning 
and exploiting single-column
constraints, whereas existing work (such as dependency-driven 
data-cleaning) focuses on multi-column constraints (e.g.,
FDs and denial constraints). This highlights the uniqueness 
of our approach relative to the literature, and the fact
that it complements nicely with existing work, 
as we have now discussed in 
\rev{Section 5 and Section 6} of the paper. 

At a conceptual level, 
as our approach is among the first to automatically
learn and exploit single-column constraints, which is 
very different from multi-column constraints (e.g., FDs and denial constraints) used in existing work, it 
makes our approach uniquely positioned
in the context of the large body of existing work. We believe
that learning single-column
constraints is an under-explored area worth
more attention from the community. And we hope 
our work can serve as a springboard for future work
improving our methods in this under-studied space.

At an empirical level, we are also able to show that the single-column
constraints that our approach exploits
nicely complement with the multi-column constraints -- for example, on the enterprise benchmark data, our proposed single-column
approach works for 558 test columns; however, as we
explain in the experiments, out of the 558 columns,
at most 57 can be covered using FD-based 
methods (these columns are involved in an FD on the original table), 
and at most 247 can be covered using PFD-based methods.
We want to emphasize that we use an ``upper-bound'' analysis
for these baseline methods (which is why we say ``at most''), because  it is well known in the literature~\cite{berti2018discovery, papenbrock2016hybrid} that a 
significant fraction of FDs and PFDs
discovered from table instances are likely false-positives that may
not hold in a semantic sense. Nevertheless, this upper-bound
analysis highlights the complementary nature of 
single-column vs. multi-column constrains, and the 
value of exploiting single-column constraints 
studied in this work (which covers a significant fraction of data columns not ``covered'' by multi-column constraints like FDs).



\begin{tcolorbox}
\textbf{O6: The horizontal partitioning version uses a tolerance parameter to allow errors but still inherently assumes a level of homogeneity exists in the domain of C to identify patterns. Given the motivation of the work to address semantic and data drift, one can imagine that the beginnings of such drift would cause deviations from the norm/majority. Under this proposed horizontal partitioning, such values (which are not wrong nor dirty) would be removed, and never
identified.}
\end{tcolorbox}


\stitle{Response.} 
It is true that when data begins to drift, and when the drift is still
``minor'', our approach may not trigger,
because it consciously trades off recall for very high
precision. Recall that in our intended use case
high precision is crucial, because learned constraints are
applied at-scale to millions of columns without human
verification (a lower precision will likely overwhelm
human operators with false-alarms).

We should also mention that this 
desired level of sensitivity and the desired trade-off 
between precision/rcall is entirely 
customizable through the tolerance parameter.

We have added discussions in \rev{Section 4} to further 
clarify this design consideration.


\begin{tcolorbox}
\textbf{O7: In the evaluation, I found Figure~\ref{fig:sensitivity} to be difficult to read and to differentiate among the techniques and their parameter values when used as symbols. I would suggest separating the precision and recall graphs.}
\end{tcolorbox}


\stitle{Response.} 
We have separated precision and recall into two
separate graphs in \rev{Figure~\ref{fig:sensitivity}}, which should make the graphs more readable.


\begin{tcolorbox}
\textbf{O8: The related work was sparse, especially the error detection and pattern profiling sections.
I would recommend more technical discussion in each of these areas, and how this work is tied to the area of dependency driven data cleaning (where the
evaluation includes an FD based algorithm).}
\end{tcolorbox}


\stitle{Response.} 
As suggested, we have expanded our related work
section (\rev{Section 6}). Regarding dependency driven data cleaning --
in a nutshell, the large body of influential work on 
dependency/constraint-driven data cleaning
primarily focus on \textit{multi-column} dependency
(e.g., FDs or denial constraints),  whereas
our proposed \sj{}  infers \textit{single-column} constraints
from a table corpus, which is orthogonal and 
complements this line of work.
Furthermore, unlike existing dependency-driven methods 
that typically require humans verification
(for it is known that constraints discovered automatically 
from table instances may not always hold semantically~\cite{berti2018discovery, papenbrock2016hybrid}), 
our unsupervised approach infers accurate
single-column constraints that can be directly applied 
at scale (e.g., millions of columns) without requiring human validation.






\bigskip
{\huge \stitle{Response to Comments by Reviewer 2}}

\bigskip
\begin{tcolorbox}
\textbf{O1. More justifications could improve the technical depth. FMDV-H is considered NP-hard using a reduction from the independent set problem. A more detailed proof could be provided. Time complexity is O(T.P(D)) but P(D) is constrained by the choice of $\tau$, which is not explained/justified. This parameter limits the pattern enumeration in off-line indexing to columns of at most $\tau$ and it is critical. Statistical tests in Section 4 are chosen without a clear justification, whereas other tests of homogeneity (e.g., chi-square) could be used. Why?}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$  As suggested, we added a proof of NP-hardness in \rev{Section 4}.

$\bullet$ The parameter $\tau$ is indeed important as it motivates the Horizontal-cut algorithm (Section 3), and was described a few pages earlier in Section 2.4 (offline stage), and then in more detail Section 3. We realize that the ``time complexity'' section at the end of Section 4 (for the entire algorithm end-to-end with both Horizontal and Vertical cuts) also makes references to this $\tau$ that was introduced a few sections earlier, making it hard to refer back. We thank the reviewer for pointing this out, and have revised this part in \rev{Section 4} to explicitly 
reference relevant discussions of $\tau$ in earlier sections. (We tried to bring the time-complexity section closer to where $\tau$ is first described, which however turned out to be difficult, because the time-complexity is for the overall algorithm with both vertical-cuts and horizontal-cuts, which is only natural to come at the end of Section 4).  

We should also mention here that in addition to the analytical analysis, we have an encouraging sensitivity analysis on $\tau$ (Figure~\ref{fig:sensitivity_to_index_tau}) that shows a smaller
$\tau$ has little impact on result quality (the blue line for
FMDV-VH), thus allowing us to bound the complexity/cost
without sacrificing quality.

$\bullet$ Other tests of homogeneity can indeed be used, like the Chi-Squared test mentioned by the reviewer. We did already discuss this test, and experimentally compared with it in our paper (\rev{Section 4}), which showed no difference in result quality. We have highlighted it more in the paper to make it more visible.



\bigskip
\begin{tcolorbox}
\textbf{O2. The assumption that the data set contains homogeneous values drawn from the same underlying domain is a strong assumption (not so realistic) and the relaxation of this assumption claimed by the authors is not clear from the basic-version of Auto-Validate (section 2, Eq. (4)) to the more advanced variants (Section 4, Eq. (11)). Could the authors explain and demonstrate this effectiveness across domains? e.g. from Enterprise to Gov benchmarks for example ?}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$ We fully agree with the reviewer that the
kind of data we commonly encounter in our 
everyday life (e.g., csv and
spreadsheet files that humans manually create)
is indeed messy, and we as data researchers have
come to expect data to be messy/heterogeneous.
However, we want to highlight the perhaps counter-intuitive 
fact that because our setting is in
large enterprise data lakes with millions of 
tables, the vast majority of data in question
is \textit{machine-generated} (i.e., values in the same column
are generated by the same underlying program),
as opposed to manually created (which is indeed
more error-prone and less homogeneous).
%Given the scale of our data, this is perhaps not that 
%surprising in retrospect, because 
%machines are, after all, much productive in churning
%out data in volume than humans.

Given the context that data is typically ``machine generating''
in enterprise data lakes, it is then perhaps not 
entirely surprising that we find data in data lakes
to be more homogeneous than one may expected 
-- as we describe in detail
in our \rev{response to the O1 of Reviewer-1}, we have performed
an quantitative analysis of data in our data lakes, by sampling
1000 random columns and manually judging whether each is
homogeneous or not (we copy the result table below 
for ease of reference). Our analysis suggests that
879 columns out of the 1000 are deemed homogeneous, within
which 76.9\% (676 out of 879 columns) 
are clearly machine-generated as they have
rigid data-patterns \footnote{We
suspect that this fraction is likely to be higher in
other enterprise data lakes, because our 
data lake serves as the back-end for a commercial
search engine, which has to deal with large volumes of 
unstructured user queries that are likely ``non-homogeneous''.}. 


\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|l | l | c | c |} 
 \hline
  Column type classification & Real example columns & \begin{tabular}{@{}c@{}}Fraction of columns \\ (in 1000 samples) \end{tabular}     & \begin{tabular}{@{}c@{}}95\% confidence  \\ intervals \end{tabular}   \\  \hline \hline
   \textbf{(1) Homogeneous-rigid-patterns} & $C_1 =$  \{ ``03/02/2015|OnBooking'', ``06/12/2015|OnBooking'', ``05/11/2015|OnImpressionDelivery'', \ldots \} & 0.676 & $[0.639, 0.711]$ \\  \hline 
   \textbf{(2) Homogeneous-NL-like} & $C_2 =$  \{ ``Bristol Marriott Hotel City Centre'', ``Renaissance Schaumburg Convention Center Hotel'', ``The Ritz-Carlton, Dallas'', \ldots \} & 0.203 & $[0.174, 0.236]$\\  \hline
   \textbf{(3) Non-homogeneous} & $C_3 =$ \{ ``adobe reader updates for xp'', ``acrobat software deals'', ``download acrobat reader 8'', ``foxit pdf reader'', \ldots \} & 0.121 & $[0.098, 0.149]$ \\  \hline
\end{tabular}
\caption*{Analysis of column homogeneity using 1000 columns from the ``Enterprise'' data lakes.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


We believe
these are significant numbers and show the general applicability
of our technique, given that there are millions of columns at
stake in our data lake alone 
and our technique can apply to a majority of 
those cases. Since this technology is being released 
as a feature in a cloud-based enterprise data-lake product
in Jan 2021, and applied to many
other large enterprise data lakes, 
the potential impact will likely multiply.





$\bullet$ The reviewer is correct that homogeneity in
the basic-version of Auto-Validate (Section 2, Eq. (4)),
is indeed relaxed later in Section 4 for Horizontal-cut, as
explained in the paper. However, Eqn (11) pointed out 
in the comment is actually in Section 3 and
for a different variant called Vertical-cut, 
which as a result would not 
relax homogeneity, as the reviewer rightly
observed. We ask the reviewer to kindly
compare Eqn (5-7) in Section 2 with Eqn (12-16) in Section 4
instead, which should better show this relaxation (specifically 
in Eqn 16). We have clarified this more in \rev{Section 2
and Section 4} of the paper.

$\bullet$ Our experiments indeed try to demonstrate 
effectiveness across domains -- specifically, we used 
two benchmarks taken from two very different domains: 
one from a real Enterprise data lake, and one from a 
Government data repository. Our results show
that our proposed FMDV-VH algorithm 
is significantly better than both our own 
basic version (without Horizontal/Vertical-cuts), 
and all other baselines we experimented with. 

In the revision we added statistical tests 
in \rev{Section 5} to demonstrate
that these observed performance advantages are both
(1) statistically significant, and (2) the ``effect size'' of
the new algorithm is
``large'' in a statistical sense. These relate to D4 and D5
below, and we ask the reviewer to kindly refer to our
responses below for more information on the experimental
comparisons in different domains.


\bigskip
\begin{tcolorbox}
\textbf{O3. In terms of experiments, the setup is confusing. Some important details are omitted. Because of impractically large numbers of patterns, there are
omissions in the indexing and it is not clear whether these omissions are considered in the precision/recall measures (see other comments D4-D8).}
\end{tcolorbox}

\stitle{Response.} 
We have clarified  in \rev{Section 5} that the effect of omitting patterns is indeed already captured in our precision/recall evaluation – if for some column a suitable validation pattern is not generated 
by our algorithm (due to omissions in our 
indexing step), then we would either: (1) generate overly-generic
patterns that fail to catch quality issues tested, which would lead
to recall loss, or (2) generate overly-restrictive patterns
that produce false-alarms on correct data values, which
would lead to precision loss. Both of these two situations
are indeed already accounted for in our evaluation. 

(For other comments D4-D8 we will respond to them separately below).


\bigskip
\begin{tcolorbox}
\textbf{D1. Lemma 1 should be justified.}
\end{tcolorbox}

\stitle{Response.}  We have added a sketch of the proof 
to justify Lemma 1 in \rev{Section 2.3} as suggested.



\bigskip
\begin{tcolorbox}
\textbf{D2. Definition (3) is very simple and may not adapted for heterogeneous corpus.}
\end{tcolorbox}

\stitle{Response.} This relates to O1 and O2 above, which we 
have addressed in our responses above and 
in relevant sections of the paper. 

Briefly, we show in our response to O2
that we observe through a quantitative analysis that 
a majority of columns in large enterprise data lakes 
have machine-generated homogeneous values, making 
heterogeneity less of a problem in our setting.

For the minority of columns where
homogeneity does not apply, we should emphasize that:
(1) our technique will
pass on such columns (for no patterns can be generated), thus
not producing false-positives; and (2) more importantly, 
because no  patterns can be generated for the 
non-homogeneous columns even in the indexing step, 
they will not ``pollute'' our
signals for the homogeneous ones and would not 
affect our results on the majority cases where the 
technique does apply. 

Relating to our response to O1, the homogeneity
assumption in the basic version is also 
relaxed in our 
Horizontal-cut variant, which is shown to be 
effective (Figure~\ref{fig:accuracy}). 

We have added these discussions in our paper,
and we ask the reviewer
to kindly refer to our responses to O1 and O2 above 
for more detailed answers.


\bigskip
\begin{tcolorbox}
\textbf{D3. Figure 11 legend is incomplete (red diamond symbol has no name).}
\end{tcolorbox}

\stitle{Response.} The legend on this figure was 
made into a non-standard format with names first, followed
by symbols/markers, which made it appear as if the
last symbol (red diamond) has no name. We have fixed
the legend on \rev{Figure 11} to make it more standard using symbols first, followed by names, which should now avoid
this confusion.



\bigskip
\begin{tcolorbox}
\textbf{D4. The evaluation methodology in Section 5.1 does not detail the number of iterations (runs) of the randomized selection of the 1000 columns. As such,
this process should be re-iterated at least 10 times to account for randomization. It is not clear that the results in terms of precision, recall, F1 are averaged.
However, if this is the case, the results in Section 5.3 could mention the averages with their respective standard deviations (e.g., in Table 2 and Figure 10,
11, and 12). This would also tell us whether the main assumption made by the authors (i.e., values are homogeneous across columns in machine-generated
data) is realistic or not and if Eq. (4) is not too simplistic.}
\end{tcolorbox}

\stitle{Response.} 

$\bullet$ Our precision and recall scores
are indeed averaged over 1000 randomly selected
columns from the corpus. We have clarified this
and added standard deviations to Table 2, and in relevant
discussions in \rev{Section 5}.\footnote{Figure 11 is a drill-down of Figure 10 
with a case-by-case analysis, where no separate 
standard deviations can be reported and the same from
Figure 10 applies.}

$\bullet$  Regarding the homogeneity assumption for 
machine-generated data, we have responded
to the related comment O2 above in more detail (using
a quantitative analysis of 1000 sampled 
columns). As a brief summary, homogeneity is observed 
to hold for a majority of columns in 
data lakes in practice, 
for which our technique provides clear value in 
terms of automated validation as shown in our
experiments. For the minority of columns where
homogeneity does not apply, we should emphasize that:
(1) our technique will
pass on such columns (for no patterns can be generated), thus
not producing false-positives; and (2) more importantly, 
because no  patterns can be generated for the 
non-homogeneous columns even in the indexing step, 
they will not ``pollute'' our
signals for the homogeneous ones and would not 
affect our results on the majority cases where the 
technique does apply.  We ask the reviewer
to kindly refer to our response to O2 for more details.


$\bullet$  Regarding the evaluation of our results, 
we added more details to \rev{Section 5} of our paper.
We treat the precision/recall/F-score result of an algorithm $A$ 
on a randomly selected column $C$ as a random variable, 
and we perform 1000 randomized trials that 
would sample from this underlying random
variable (using 1000 randomly selected columns).

Using these 1000 randomized trials, we can perform standard
statistical tests, where the null-hypothesis states that FMDV-VH
is no better when compared to an alternative 
baseline $A$, for each baseline we compare with. 
In the following we will report (1) statistical significance, and
(2) effect size, when comparing FMDV-VH with all baselines
using F-scores, which is the harmonic mean of precision and recall.



For statistical significance, as can be seen from the table below,
all $p$-values are in the range of 0.001 to 0.007,
much smaller than the standard threshold of
significance ($p<0.05$), indicating that we should reject the
null hypothesis, showing that
the quality benefit of using our proposed algorithm 
FMDV-VH is significant.



\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |} 
 \hline
 Compare FMDV-VH with:  & FMDV-basic & FMDV-V    & FMDV-H & Grok & XSystem & PWheel & SM-P-P & SM-P-M & SM-I-1 & SM-I-10 & FlashProfile & SSIS & Deequ & DeequDist & TFDV   \\  \hline \hline
Enterprise benchmark & 0.002 & 0.001 & 0.007 & 0 & 0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.001 & 0.001 & 0 & 0.001 & 0  \\ \hline
Government benchmark & 0.001 & 0.001 & 0.007 & 0 & 0.001 & 0 & 0 & 0 & 0 & 0.001 & 0.001 &  NA & NA & NA & NA \\ \hline
\end{tabular}
\caption*{$p$-value for statistical-significance on F-measures, between the proposed FMDV-VH, and all other baselines. We use $p<0.05$ to reject the null hypothesis that FMDV-VH is no better than a baseline. (All comparisons are statistical significant).}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}


On top of statistical significance, we test for
``effect size'' using Cohen's d, which measures 
whether the F-score improvements are deemed as ``large''
in a statistical sense. (For Cohen's d, the convention is
to treat an effect-size of $d>0.8$ as large, and $d>1.2$ 
as very large\footnote{\url{https://en.wikipedia.org/wiki/Effect_size\#Cohen\'s_d}}). 
As can be seen from the table below,
most of these improvements over baselines are either ``large''
or ``very large'', showing a clear benefit of our algorithm
when using randomized trials a statistical interpretation.


\begin{table}[h!]
\vspace{-2mm}
\centering
\scriptsize
\begin{tabular}{|c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |} 
 \hline
   & FMDV-basic & FMDV-V    & FMDV-H & Grok & XSystem & PWheel & SM-P-P & SM-P-M & SM-I-1 & SM-I-10 & FlashProfile & SSIS & Deequ & DeequDist & TFDV   \\  \hline \hline
Enterprise benchmark & 2.23 & 2.05 & 0.24 & 5.40 & 7.90 & 6.09 & 6.40 & 6.36 & 5.79 & 6.37 & 5.54 & 6.20 & 7.98 & 7.78 & 6.09  \\ \hline
Government benchmark & 1.928 & 1.838 & 0.154 & 2.913 & 4.395 & 4.075 & 4.210 & 4.294 & 4.233 & 4.109 & 2.085 & NA & NA & NA & NA  \\ \hline

\end{tabular}
\caption*{Cohen's $d$ for effect-size, between the proposed FMDV-VH, its different variants, and all other baselines. $d>0.8$ is regard as having large effects.}
\vspace{-2mm}
\label{tab:enterprise-survey}
\end{table}

We have summarized our findings and the 
new statistical test results in \rev{Section 5} of the paper.


\bigskip
\begin{tcolorbox}
\textbf{D5. 1000 test cases have been used as ground truth (only for Enterprise data set), which may not be statistically significant as no detail is given on the
selection of these test cases and any potential selection bias in favor of the proposed method.}
\end{tcolorbox}

\stitle{Response.} 
We have clarified in \rev{Section 5} that the 1000 test columns 
are randomly selected from the data lake, 
which should be representative and
give no bias in favor of any method. 

Statistical significance results are discussed in detail
in our response to D4 above. 
We would like to confirm here that 
all comparisons in Figure~\ref{fig:accuracy}
are shown to be statistically significant, 
with $p$-values ranging from 0.001 to 0.007 (where $p<0.05$ 
is typically regarded as significant). We ask the reviewer to 
kindly refer to D4 above for more information.


\bigskip
\begin{tcolorbox}
\textbf{D6. The evaluation experiment consumes 1000 columns among 7.2 M and 628K respectively for Enterprise and Government data sets. The average
numbers of tuples and distinct values (with standard deviations) per data set are not given and it is difficult to have an idea of the heterogeneity of the data
sets.}
\end{tcolorbox}

\stitle{Response.} 
As suggested, we have added these statistics in \rev{Table 1 of Section 5} in our paper. We should clarify that the key homogeneity property our algorithm leverages is with respect to values in the same column (which is shown to hold in practice on a large fraction of data as detailed in our response to O1 of Reviewer-1).
Data tables may exhibit another layer of heterogeneity
in terms of number of rows and
distinct values, etc., which however do not 
pose challenges to the proposed method for pattern inference.


\bigskip
\begin{tcolorbox}
\textbf{D7. It is unclear how to set $\tau$ and the other parameters; the figures 12 (a-d) are difficult to read as they are on a very limited ranges for the parameters
and we suppose it is averaged over the two datasets but it is not specified.}
\end{tcolorbox}

\stitle{Response.} 
We have added discussion in \rev{Section 5.3} 
on recommended settings for these parameters
based on observations from the sensitivity analysis. 
It can be seen that the proposed FMDV-VH
(the blue line) is not particularly
sensitive to $m$, $\tau$, and $\theta$, and not
very sensitive to $r$ as long as it is set to a reasonably high
value (e.g., above 0.02).

We have completely redrawn \rev{Figures 12} to make it 
more readable, by separating precision and recall into two
sub-figures. We have also clarified in the figure caption 
that the sensitivity figures
only show results on the Enterprise benchmark
due to space constraints. We thank the reviewer
for these suggestions.


\bigskip
\begin{tcolorbox}
\textbf{D8. It is not clear how AD-UB and FD-UB are implemented and effectively tested as they may suffer from scalability issues.}
\end{tcolorbox}

\stitle{Response.} We have added clarification in \rev{Section 5.2}. For FD-UB, we implemented the
standard FD-discovery and run it on individual test tables. 
For AD-UB, we implemented what is reported in the AD paper~\cite{huang2018auto},
which is already designed for large corpora of tables.
Because both are known methods,
they do not pose significant scalability challenges for us.
We should note that unlike AutoValidate which is
required to run at an interactive speed, 
we are only comparing the two baselines
from a quality (precision/recall) perspective, which do not
require us to make the two run at an interactive speed.



\bigskip
\begin{tcolorbox}
\textbf{D9. Eq.(11) is too small}
\end{tcolorbox}

\stitle{Response.} 
We have separate \rev{Eq.(11)} into multiple lines, which should make it more readable now.



\bigskip
\begin{tcolorbox}
\textbf{D10. Non-conforming values like null values can actually be very informative of the heterogeneity for formatting missing values and should be indexed
whereas the authors propose a way to 'cut out' a fraction of the non-conforming values with $\theta$ parameter.}
\end{tcolorbox}

\stitle{Response.}
We thank the reviewer for the interesting suggestion. 
While our approach already shows good quality, 
this is definitely an interesting idea worth exploring in the future.
We added it in the future work \rev{Section 7}.


\bigskip
\begin{tcolorbox}
\textbf{D11. Balance of the paper structure. Please extend the conclusion and reduce the introduction to avoid redundant information.}
\end{tcolorbox}

\stitle{Response.} 
As suggested, we have rewritten parts of the introduction and conclusion sections to optimize the structure of  the paper.













\bigskip
{\huge \stitle{Response to Comments by Reviewer 3}}

\bigskip
\begin{tcolorbox}
\textbf{O1: In the ``Time Complexity'' subsection, it is explained that the offline step has a complexity that depends on the size of the full corpus (which is assumed
to be very large) multiplied by the number of patterns that can be generated for each column (exponential in the number of tokens contained by the column).
This is potentially an extremely large value.
Throughout the paper, little attention is paid to the cost of the required operations. Authors should clarify:
How was the corpus of patterns generated? How big was the cluster used to produce the index? What’s the effect of tau on the execution time? How often
does the index need to be updated?
Some examples of the number of patterns and segmentations encountered during the experimental section would help with having an idea of the cost of the
solution in a realistic situation. A study of the overall time required by the different algorithms would similarly be useful to provide additional context.
It is currently hard to understand how the system would perform in a small-scale environment that cannot rely on production-grade clusters.}
\end{tcolorbox}

\stitle{Response.} 
This is a great suggestions. We added discussions 
on the cost aspect in \rev{Section 5}
of our paper. Overall we are happy to report 
that our algorithms are expected to work fine on 
small-scale clusters. Specifically, although our jobs
were run on a production-scale cluster, 
our particular experiment reported in the paper with
7M columns finishes 
in under 3 hours end-to-end using only 10 “virtual nodes”.
Like other systems, our job scheduler 
dynamically assigns each job to an 
appropriate number of “virtual nodes” based on 
the job’s estimated cost, and 10 is estimated to
be (and indeed is) adequate for our indexing job.
Because each virtual-node in our system 
is wimpy (many virtual-nodes are packed into one
VM, with each node having a fraction of the resources in the VM),
we fully expect a job like ours to run without problem 
on small-scale clusters (less than 10 machines).

To provide additional details in response to the questions
raised: 

$\bullet$ The offline pattern generation step is indeed relevant,
for which we have added discussions in \rev{Section 2.1}
and \rev{Section 2.4} to better explain the steps involved.
The key insight is that while a brute-force enumeration
is indeed expensive, our approach 
avoids exhaustive enumeration in the offline
step by enumerating only patterns of length up to $\tau$
without affecting quality, 
because our Vertical-cut algorithm (Section 3) 
uses dynamic-programming that can piece together
sub-patterns into longer patterns at online query time.

$\bullet$ From a large table corpus, after pattern summarization
and aggregation ({Section 2.4}), our index is about 
900MB in size, with 6.2M entries (unique pattern candidates),
which is many orders of magnitude smaller than the raw
data. (More statistics on the patterns encountered/summarized
can be found in a full version of the paper~\cite{full}, which is
shared\footnote{\url{https://www.dropbox.com/sh/b2u39qha8o83zos/AACZPQ5jUDFwgCuFgGdc0oFsa?dl=0}} for the reviewer to inspect.).

$\bullet$ Changing $\tau$ from 8 to 13 increases the indexing job
from around 1 hour to 3 hours, which however produces no
significant increase in result quality. We recommend
to use $\tau = 8$ as a result. These are added to \rev{Section 5}.

$\bullet$ In one of our sensitivity study (not included
in the paper due to the space constraint), we use data corpus from
6 month ago as the ``training'' data for AutoValidate, 
and use ``test'' data
generated 6 months after as query columns. The result
quality is still high and we did not see significant 
drop in quality.
This we believe shows that the domain definitions 
of the underlying data 
do not change rapidly, making us to believe
that it is sufficient to re-run 
the indexing job once in a few months. 

\bigskip
\begin{tcolorbox}
\textbf{O2: AutoValidate works only on homogeneous columns (as they can be described through patterns), so free text columns must be excluded. The fact that AutoValidate cannot handle free text does not diminish the contribution, however this limitation should be clarified more from the start (abstract for sure -
even in the title?), while right now it is mentioned only briefly in the introduction and in a sentence in the experimental section (where initially it's claimed 1k
columns, but it's not the case).}
\end{tcolorbox}

\stitle{Response.} 
This is a great suggestion. We have now emphasized this 
point more in
the \rev{Abstract}, and re-iterated it in a few places in 
our introduction in 
\rev{Section 1}, so that readers can better understand 
that machine-generated homogeneous data is the 
focus of our work from the start.

\bigskip
\begin{tcolorbox}
\textbf{O3: The experimental study can be improved by reporting some results over the columns that are not handled by the proposed solution. Those are about
40\% and AutoValidate has 0 on those - what about the baselines? I am not suggesting this to raise an issue with the proposed system, but it would be fair to
give a feeling on what other do in a setting where this solution fails completely.
For example, users are asked to create regular expressions to describe a column taken from those that AutoValidate can handle. These regex are then
compared to what AutoValidate produces in its querying step. It is expected that a computer system would be many times faster at producing a result in
such conditions, but it is also true that the users may can up with much more expressive checks (see also O4).}
\end{tcolorbox}

\stitle{Response.} It is true that users can write more
expressive checks such as more specific regex based on 
their semantic understanding of the data expected in a column,
which is indeed not something that AutoValidate is intended
to support,
and is likely challenging for any unsupervised methods
(please kindly refer to O4 below for a more detailed response on this aspect).

We indeed performed an analysis of the 40\%
cases where AutoValidate does not handle.
The majority of the cases are the data columns that
our approach is not expected to handle, including
natural-language-like content 
(e.g., company-names, people-names), and
non-homogeneous columns 
(e.g., mixed search engine queries).  In both of these cases,
regex is likely not the right representation to capture the
underlying domain.  In our response to
\rev{O1 of Reviewer-1} we gave a detailed analysis of
the underlying data lake --  
we sampled 1000 columns and manually analyzed the characteristics of each column, and found that 32\% of the cases
are either homogeneous-but-natural-language-like, or
non-homogeneous, for which we would not expect any
pattern-based approach (including AutoValidate and other 
baselines compared in the paper) to handle. 
We ask the reviewer to kindly refer
to O1 of Reviewer-1 for more details of the analysis.

For the remaining cases (less than 10\%) 
where a ground-truth regex pattern
does exist and our approach fails to find the optimal pattern,
we found the main reason to be 
the lack of support for advanced pattern constructs, such as 
union of multiple patterns, and flexibly-formatted URLs, 
in our current profiler/pattern-language.

We have added this error analysis in \rev{Section 5.3} as
suggested.


\bigskip
\begin{tcolorbox}
\textbf{O4: If I understand correctly, given a query column that contains only data values starting on January 2020, the system will infer a date pattern. However,
the correct rule is the one with year equals to 2020 as those are covid 19 cases. Unfortunately, incorrect dates with 2018 are not detected by the pattern.
This issue does not seem to be captured by your experimental setting but would be a real issue in validation, as incorrect values are validated by the
patterns that you propose. I am not suggesting to improve the language of the patterns here, but to discuss and highlight this aspect (possibly measure it on
a sample of columns?) \\
\\
(From Q12 ``Response to Author Feedback''): Is missing business metadata leading to mistakes or affecting your method? how and how much?}
\end{tcolorbox}

\stitle{Response.}  These are excellent points. Our approach infers what is known as the ``technical metadata'', or the technical definition of all valid values in the underlying data domain (e.g., all valid date strings are considered acceptable for a column from a ``data-type/data-domain'' standpoint, which is a type of technical specification). This contrasts with what is known as the ``business metadata'', which may assign specific business meanings and semantics to each column (e.g., only dates in 2020 are acceptable in this column). The latter is indeed more expressive but is perhaps more difficult to infer from data-values alone, when an unsupervised method is used. This is because a column 
may have date-time values in Jan 2020, but from that alone, it is hard even for a human looking at the
data to know whether the data-owner's intent is
to only allow dates in Jan 2020, in Q1 of 2020, or all months of 2020. We feel that for such more expressive and semantic
checks, humans would need to be in the loop and existing
techniques such as declarative DSL for data-validation 
(e.g.,~\cite{breck2019data, schelter2019unit}) can
be used to complement auto-inferred technical 
data specification produced by our method.

We feel that the distinction on technical vs business metadata is indeed important, which we added in \rev{Section 1} of the paper. 

After reading the reviewer's response to
Q12 in the review (after author feedback), 
we feel that it should be clarified that while missing business
metadata may lead to missed opportunities in
catching certain quality issues, 
it does not lead to false-alarms or ``mistakes'' in a traditional sense (which would be a deal-breaker in our data lake settings).
This is because the technical-metadata is by definition 
broader and more tolerant than the more specific 
business-metadata (e.g., technical-metadata
specifies all valid date-time strings as acceptable,
while business-metadata accepts only date-time in 2020).
As such, without data-owners in-the-loop to provide
more fine-grained and specific metadata, we may miss on some
quality issues (loss of recall), but not trigger false-alarms
(precision is still very high).

The suggestion on 
sample-based human evaluation is also interesting.
However, since we are not data owners, 
it is sometimes a bit difficult
for us to judge in a reliable fashion, because 
by looking at the data-values alone, we may not know
the semantics behind them, or the intended constraints
on the column. We feel that ultimately it 
is up to the data owners
to tell us whether the suggested constraints are useful or not.


Along the line of what is suggested by the review, we
should report that we did
also interview real
data owners in our study, to get a sense of the
overall usefulness of our
algorithms (on top of the large-scale automated
evaluation reported in the paper, which we feel is an 
ideal and robust way for
checking compliance to ``technical metadata/data-types'',
which is the focus of the paper). We ran our
algorithms to infer constraints on real data, and then
use the constraints to catch real data quality issues 
in the data lake. From such issues, 
we sampled 10 cases,
identified the engineering teams that own the relevant datasets,
and interviewed these owners to check whether the suggested issues are indeed an issue, and whether the suggested
constraints make sense to them. (Because this is a fairly expensive
process as each case requires an 1:1 interview that is 
time-consuming for both us and the engineering teams
involved, it cannot scale to larger numbers,
which is why we chose to report the
automated evaluation in the paper).
All the teams surveyed
gave positive feedback, explaining the meanings of 
their data and telling us that 
identified issues are indeed
true data quality issues (though in some cases the data feeds are
stale copies in the lake that are no longer used, and would not
call for an immediate fix to be applied). In one case,
the data owner told us that the constraint is reasonable
but can be made more specific/restrictive given their
business context, which is very similar to what the
reviewer suggested. (Again, this may create
a loss of recall, but would not introduce false-alarms or
``mistakes'' in a traditional sense). Overall, we find such 
specific requirements to be 
difficult for algorithms to infer in an unsupervised
manner (because without a meeting with the data owner,
we as humans would not know). We feel that in such a situation, 
asking data owners to explicitly specify such constraints 
would seem like a more viable approach for now.





\bigskip
\begin{tcolorbox}
\textbf{R1: There are well-known patterns that should appear often in machine-generated data such as dates and IP addresses (this is touched upon in the
experimental section when testing Grok patterns). Is it possible to use these patterns during the pattern enumeration phase to prune bad patterns? Was
such a strategy considered?}
\end{tcolorbox}

\stitle{Response.} This is a very interesting idea. We feel that
using well-known patterns could be a useful 
optimization strategy to prune certain
parts of the search space, and yield additional efficiency
benefits. There may be a small cost to pay
in terms of quality though (e.g., we have seen version-numbers 
like ``1.0.0.1'', and if an IP-pattern is selected too hastily
without a proper search, the result quality may be reduced).
Since our latency for the online part is
already more than sufficient for most interactive uses (i.e. 86ms
per test column), we did not explore in the direction of
efficiency optimization further. Nevertheless this is 
a good suggestion that would at least reduce
offline indexing cost. We thank the reviewer for the
suggestion.



\bigskip
\begin{tcolorbox}
\textbf{R2: the matching approach seems the most promising baseline but it relies on a very simple matching method. I believe a better matching system, such as
those based on deep learning from relational data (e.g., Creating Embeddings of Heterogeneous Relational Datasets for Data Integration Tasks. SIGMOD20), improve the performance.}
\end{tcolorbox}

\stitle{Response.}  This is an excellent suggestion. We have
added discussions in this regard in \rev{Section 5} and also 
a reference to this related work.

